Scalable Testing of Context-Dependent Policies over Stateful Data Planes with Armstrong

Network operators today spend significant manual effort in ensuring and checking that the network meets their intended policies. While recent work in network verification has made giant strides to reduce this effort, they focus on simple reachability properties and cannot handle context-dependent policies (e.g., how many connections has a host spawned) that operators realize using stateful network functions (NFs). Together, these introduce new expressiveness and scalability challenges that fall outside the scope of existing network verification mechanisms. To address these challenges, we present Armstrong, a system that enables operators to test if network with stateful data plane elements correctly implements a given context-dependent policy. Our design makes three key contributions to address expressiveness and scalability: (1) An abstract I/O unit for modeling network I/O that encodes policy-relevant context information; (2) A practical representation of complex NFs via an ensemble of finite state machines abstraction; and (3) A scalable application of symbolic execution to tackle state space explosion. We demonstrate that Armstrong is several orders of magnitude faster than existing mechanisms.

==> ack.tex <==
\section*{Acknowledgments}
We thank Rodrigo Fonseca and Shriram Krishnamurthy for their
 feedback.  This work was supported in part by the Intel Lab's
University Research Office. Seyed Kaveh Fayazbakhsh was supported in 
part by a Renaissance Technologies Fellowship.


==> concerns.tex <==
\section{Concerns}
\begin{itemize}

 \item just found non-interesting errors, e.g., ip v6 gets dropped
 
 \item what is the  guarantee? what is covered/non covered? should we worry about non-covered parts?
 should i be happy if you tell things are fine based on some sampling/statistical testing?
  
 \item what setting can we accommodate (enterprise, data center, cloud, interdomain, etc)? 
 are the principles  generalizable? 
 
 \item what do we envision as the end product? an open flow app? a new architecture? a set of
 apis like flowtags?\dots
 

 
\end{itemize}


\comment{

\section{Macro Concerns}
\begin{itemize}

\item  why are prior testing abstractions like propositional logic, frenetic
formalism, hsa formalism not sufficient?

e.g., why is this not LTL/CTL or whatever from frenetic not enough -- we need to get some formal person to 
 look at this? 

%\item scalability?


%\item what is the criteria for a good test script? min time to run? 
%min number of entries? exploring the leaves in a certain order?

%\item interference from background?

\end{itemize}

\comment{
\section{Micro concerns}

\begin{itemize}

\item the test traffic generation logic runs at the controller. but how to tell a host to run certain traffic?

\item don't like to repeat the nsdi examples.

\item we can assume all mboxes are in state0 that allows everything. then static config takes it to state1.
this way even a packet filter will have a state machine.

\item the dpg is pictorially too high-level. where is the detailed policy represented?
e.g., block H2$\rightarrow$xyz.com rather that just FW H2?

\item what is the test guarantee/coverage? a simple example: suppose
a FW is suppose to drop packets destined to $ip_1$ and allow everything 
else. how do we test this? suppose the five tuple has $N$ bits. to ensure
there are no false pos/neg we need to test $2^N$ possibilities?

\item need to clearly define the traditional black hole, loop, and 
reachability in the presence of mboxes. e.g., is it considered a black 
hole when an ips drops packets?
is it a loop when an http response goes back from a cache to the host?
suppose there is a NAT between A and B; does this mean A can "reach" B?

\item (not a concern!) ATPG can be still orthogonally useful for exploring paths purely 
involving switches and routers.


\end{itemize} 
}
}

==> deprecated/concerns.tex <==
\section{Concerns}
\begin{packeditemize}
\item \seyed{The example does not involve any ``bump-in-the-wire'' deployment. Does that matter\
in terms of the generality of the solution?}
%% Drop

\item \seyed{Raised by vyas: what should be the tagging scheme in case of cryptography?}
%% cant say anything


\item \vyas{why encode in headers, why not do reactive?}

%% this should be clear already

\item \vyas{question from brown: do we need active tagging or would a more minimal
capability that the middlebox simply passes on the tags be sufficient?}

%% address using proxy setting?

\end{packeditemize}


==> deprecated/design.tex <==


\section{\Name Overview}
\label{sec:design}
%\seyed{i think we should generalize the ``test manifest" 
%to include elements like mbox config instruction (e.g., the 
%"clear cache" instruction for a proxy), not just pure traffic to inject?}

%\seyed{to decide: moving this high-level design to intro}

 Figure~\ref{fig:overview} shows a high-level overview of the \Name framework
  with key  logical components: 

\begin{packedenumerate}

\item {\em Test traffic planner}, which generates a 
 test traffic plan  or {\em manifest}  and coordinates
the actions of the {\em injectors} to generate  traffic traces that 
 test desired properties. 

\item {\em\Injectors} are regular hosts or servers running 
 test traffic generators or trace injection software 
 and run the commands issued by the planner. 

\item The {\em monitoring and validation engines} passively monitors the status
of the SDN controller and the  data plane.  This serves two purposes.  First,
the current state can inform the actions of the planner; e.g., which are the
reachable prefixes.  Second, monitoring reports help us check if a test
succeeded or  help diagnose why a test may have failed; e.g., is it a
legitimate failure or caused by interference from background traffic?
(See~\S\ref{sec:discussion}.)

\end{packedenumerate}

\begin{figure}[t]
  \centering \includegraphics[width=230pt]{./figs/overview.pdf}
  \tightcaption{High-level architecture of \Name.}
\label{fig:overview}
 \end{figure}

Our focus in this paper is on designing  the {\em test traffic
 planner}, and we plan to integrate  tools from prior 
 work for the other components. For example,
 we can use existing injection tools (e.g., bittwist, pytbull) or 
 request generators (e.g., Harpoon~\cite{harpoon}).
Similarly, for the monitoring engine, we can use a combination of controller
checkpoints and data plane logging~\cite{netsight}.


Figure~\ref{fig:planner_arch} shows the modules within the 
  test traffic planner.  The output of the planner is a
 {\em test manifest} for  the various 
 injectors,  indicating the
 sequence of test packets to inject, time to inject, and injection locations.
The main inputs to the test traffic planner are:

\begin{figure}[t]
  \centering \includegraphics[width=220pt]{./figs/planner_arch.pdf}
  \tightcaption{Design of the test traffic planner in \Name.}
\label{fig:planner_arch}
 \end{figure}

\begin{packeditemize}
\item {\em Models of data plane elements:} 
  First, we need abstract models to capture different \DPFs. 
  While stateless \DPFs (i.e., switches 
 and routers) can be modeled using {\em transfer 
 functions}~\cite{hsa}, we 
 need new models for stateful \DPFs such as proxies and stateful 
 firewalls. 

\item {\em Network model:}  We need to model the network topology (i.e., 
  how the \DPFs  are connected) and the forwarding 
 strategy. This is essential to test service
 chaining policies and dynamic data flows.

\item {\em Policy requirements:}  In addition to traditional network
reachability properties (e.g., loop-freeness or black holes), the power of
advanced  data planes coupled with new SDN control planes will  likely lead to
more complex policies. We already saw some examples with the service chaining
policy in Figure~\ref{fig:proxy} and the dynamic data flow in
Figure~\ref{fig:lips-hips}.  We may  also want to verify other consistency
properties; e.g., does a NAT maps all packets in a flow consistently; does a
stateful firewall block reverse-direction traffic for unestablished
connections; and does a rate limiter honor the configured thresholds?

\end{packeditemize}

Given these inputs, we envision
 a {\em  trace planner algorithm} that generates a ``high-level'' 
 test plan; e.g., \emph{``inject
flow $f$ into the network from host/server $I$ at time $t$"}. 
 Essentially, this involves some mechanism to systematically
 explore  different states of the data plane and test its 
  behavior in these states. 
%That is,  we need a ``plan"  or 
% a sequence of ``actions" to transition from the ``current state" to 
% some ``goal state'' in which we want to test the policy. 
 For instance, in the example of Figure~\ref{fig:lips-hips}, to ensure that the 
L-IPS triggers a suspicious flag, our plan will be to have a host 
 have three consecutive failed connections.


The  test manifest generator  translates the output of the planner into a
concrete traffic trace.  The test manifest generator chooses a subset of
traffic traces from a repository of test traffic traces.  We decouple the trace 
 planning step  from the  manifest generation for  reasons 
 of modularity; e.g.,  to  try different algorithms for trace plan generation.
%\vyas{need better names or macros for each of these components}


==> deprecated/detailed_approach.tex <==
\section{Generating test plans}
\label{sec:details}

%As we discussed in the earlier sections, to test a stateful data plane, we need
%to be able to verify the data plane's behavior against the intended policies in  
%different states. 
%At a high level, this test approach requires a way of making 
%the desired transitions of data plane state via injecting test manifests. 
In this section, we discuss our initial approach in designing the test traffic planner.
We begin by discussing how we model \DPFs as state machines.\footnote{While the set of states could 
 be infinite w.r.t. future traffic patterns (e.g., all HTTP objects), at any given instant
 we have a finite set of states.} Then, we show how we can compose  \DPFs 
 to build a model of the entire network. Finally, we show how we can cast 
 test trace generation in the language of {\em planning} tools from 
 the AI literature.

  

%the data plane can be modeled as a finite state machine w.r.t. the observed
%traffic at any given time.}

%Since a stateful data planes is composed of individual stateful elements, we 
%need a model of stateful behavior of network elements and need to combine 
%these individual models together to build a model of the network data plane. 

\subsection{\DPFs as State Machines}

 Figure~\ref{fig:sm} highlights how the different \DPFs from the 
 previous sections can be naturally modeled as state machines. 
\begin{figure}[t]
\centering 
\subfloat[Example in Figure~\ref{fig:proxy}]
{
\includegraphics[width=220pt]{./figs/ex1_FSM.pdf}
\label{fig:sm:fwproxy}
} \\ \vspace{-0.3cm} 
\subfloat[Example in Figure~\ref{fig:lips-hips}]
{
\includegraphics[width=220pt]{./figs/ex2_FSM.pdf}
\label{fig:sm:lipships}
}
\tightcaption{Modeling \DPFs as state machines and service chaining or composition 
 as special conditional transitions between individual state machines. }
\label{fig:sm}
 \end{figure}


\begin{packedenumerate}
\item{\em Stateful firewall:}  Each observed packet belongs to 
a connection that is in one of the four shown states: \texttt{NULL}, \texttt{NEW}, 
\texttt{ESTABLISHED}, or \texttt{INVALID}. Each connection starts in the \texttt{NULL} 
state. Receiving a packet that corresponds to an outgoing edge of the 
current state takes the connection to the next state.


\item {\em Proxy:} The state of a  proxy is expressed w.r.t. the HTTP object \emph{X} (e.g., an HTML web page), showing 
whether it is cached. 

%In this example the functional semantics of the proxy 
%mandates that parameter \texttt{x} refer to an HTTP session.
 
\item {\em Light IPS:} The light IPS maintains a counter for each 
 source host, tracking the number of recent failed connections. It increases 
 the counter when failed connections recur and periodically decrements 
 the counter to avoid false positives. 

\item {\em Heavy IPS:}  The heavy IPS  just maintains two 
 states: is a host  sending malicious traffic or not.
\end{packedenumerate}
 
%\begin{figure}[t]
% \end{figure}
 
 
We currently assume that the \DPF vendor or domain expert can generate these models. 
 Synthesizing  models from the source code or black-box behaviors is 
 an interesting direction for future work  (\S\ref{sec:discussion}).


 
 \subsection{Modeling the network} % Data Plane as a State Machine}
 Having modeled individual \DPFs,  we need to put them together to create  a
network-wide model of the data plane (the ``network model module" in
Figure~\ref{fig:planner_arch}). Suppose our chaining policy is to ensure that
\DPF  A processes the traffic before \DPF B. Then, we embed the prerequisite of
traffic being processed by A as a precondition to enter  the state machine model of B (shown 
 by dashed arrows in Figure~\ref{fig:sm}). Note that not all 
 transitions across the state machines of individual \DPFs may be meaningful; 
 e.g., a proxy may not respond unless the connection is already established. 

%We show an example of this in  the next section, where  the light IPS and the
%heavy IPS are chained together to implement the dynamic dataflow.

%\seyed{check this pls- i mean to say you need flow tags or something to
%implement policies, otherwise might raise question for the reader how you would
%do this in the first place, leave alone testing it...}
 Since some \DPFs may modify packet headers, setting up forwarding 
 entries to compose \DPFs might be challenging 
 as observed in prior work~\cite{simplesigcomm,flowtags_nsdi}. 
Our goal in this paper is not to mandate a specific 
 data plane realization for service chaining and we can use a combination of 
 existing approaches~\cite{simplesigcomm,flowtags_nsdi,stratos}. Rather, our goal in \Name 
 is to {\em test} that such implementations are correct, and the design of \Name 
 is agnostic to this implementation.

% \seyed{this para is meant to say that in the eventual system we need to
% include stateless elements too} 
We also envision including models of stateless \DPFs (i.e., switches and
routers) as part of this network-wide model. Here, we believe existing work on
reachability testing~\cite{hsa, atpg} can be integrated into \Name.

\subsection{State-space exploration}
 Given the \DPF and network state models and  some ``initial'' network
state, we can formulate our testing requirement 
 in terms of  creating a sequence of events/transitions to move the
network to some intended ``goal'' state. For instance, to check that the 
  H-IPS does indeed block hosts sending three failed connections 
 with  a botnet payload, we need to ensure that the network transitions 
 to the H-IPS Alarm state.  

Based on this intuition, we believe that AI planning tools offer a ``natural
language'' in which to express this problem and thus  we formulate this as a
planning problem~\cite{russel}.  That said, we do not claim that planning is an
optimal or the only possible approach, it is a ``natural language'' in which to
express our desired properties. We are also exploring other  traditional
software testing approaches (see~\S\ref{sec:discussion}).  

%We explain  this in more detail next.

%We start from a known \emph{initial state} (e.g., when no traffic has traversed
%the network yet). In each state we can use certain operators to
%\emph{transition} to a next state. We want to find a sequence of actions that
%if taken bring the data plane to a \emph{goal state}. We show an example of
%this in the next section. 

 We make two other observations here. 
 First, not all states  may be relevant or important to explore;
 e.g., if the alarm count threshold of L-IPS=3, we may not care about 
 100 failed connections, but focus instead on values close to threshold. 
Second, there might be  multiple candidate  plans to reach our target state; 
 we defer  the issue of coverage to future work (see~\S\ref{sec:discussion}).


==> deprecated/discussions.tex <==
\section{Discussion}
\label{sec:discussion}
%We conclude  with open issues and directions for future work.
%\subsection{Data Plane}
\myparatight{Other approaches}
 We do not claim that the planning-based approach is necessary or optimal. 
 Our choice was pragmatic---we tried a range of \DPF models using datalog, 
  proposition logic, and first order logic, but could not model \DPFs as compactly 
 as the language of planning. 
As an alternative to planning, we also tried bounded model checkers
to generate test plans. Here, we write  the \DPF 
 state machine model as simple C code and use CBMC~\cite{cbmc} to generate 
counterexamples.  This counter example indicates the values of variables that lead to 
 a violation of a specific policy and use it as the input to the trace generator. 


%. We can utilize this as follow: we assert that the goal state is not 
%reachable (while in fact it is) to make the tool show why this is not true, indicating 
%the preceding state and the action. Going backward from the goal state one step 
%at a time we eventually get a complete path from the initial state to the goal state.
 Intuitively, we can also use symbolic execution approaches for test plan 
 generation. That is,  
we can think of state graph exploration as the symbolic execution of a program that 
encodes this graph. The leaves of the symbolic execution tree are reachable states 
from the initial state and each edge indicates a state transition. The counter example-based 
approach above in effect helps us explore the desired leaves of the tree. As ongoing work,
  we are evaluating the  expressivity and efficiency of different approaches.


\myparatight{Synthesizing middlebox models} We currently model the \DPF state
machines manually based on our domain knowledge.  A natural research direction
is to automatically extract such models given the implementation of various
middleboxes, either from source code (e.g.,~\cite{cegar}) or even from blackbox
traces (e.g.,~\cite{netcheck}). One interesting question is balancing model
tractability vs.\ fidelity; e.g., we can trivially take all variables in the
code as a high-fidelity model, but it may needlessly increase model complexity. 

% its code is accurate 
%but far from useful due to the huge space of possible assignments.).



%\myparatight{Non-deterministic behavior of the data plane} Some network
%elements such as load balancers may behave randomly (e.g., choosing a random
%server from the server pool), making testing challenging. In other words, we
%may not be able to control state transitions deterministically by injecting
%test manifests. One possible approach to (perhaps partially) overcome this
%problem is providing new APIs (also mentioned in~\ref{subsec:realnets}) to
%enable querying the current state of middleboxes (e.g., the current
%request-to-server mappings in a load balancer), at a minimum, we know what have
%tested despite we did not control how this mapping occurred.

%\subsection{Test Methodology}
\myparatight{Coverage and efficiency} 
  In general, we want to exhaustively test the policy in all possible network
states. However, this may be inefficient in very large \DPF state machines and
large networks. Thus, we need  mechanisms to make this state space exploration
more efficient; e.g., identify ``equivalence'' classes of states where the
behaviors might be identical.  There might also be many possible
 test plans that essentially reach the same goal state, in which case we prefer 
 more ``efficient'' plans. On a related note, we may prefer highly overlapping 
 action plans while trying to reach multiple goals. Here, we can also explore 
 opportunities to improve test efficiency by explicitly forcing \DPFs into particular 
 configurations; e.g., choosing a different rate limit or failed connection threshold.  

    
 
 %The number of states and the combinations of then can be large. We need a
 %mechanism to cover all or most of the relevant cases based on the policy
 %goals.  \myparatight{Test efficiency}

% There are typically multiple ways to reach a goal in planning problem (e.g., a
%cache object can be evicted by cache time-out or running an instruction to
%clear the cache). A test manifest should be fast to compute and run and cause
%minimal traffic. Efficient test manifest generation requires accounting for
%semantics of different protocols (e.g., the fact that HTTP runs on top of TCP
%may be useful in generating a test script containing only HTTP traffic to test
%both a proxy and a stateful firewall in one run) among other things.
 %\myparatight{Beyond test traffic}
% While we have focused on injecting test traffic into the network as the
%mechanism to trigger data plane state transitions, modifying data plane
%configurations can act as extra degrees of freedom in state transitions.  For
%example, a cached object in a proxy can be evicted either by a new object
%(i.e., traffic-based state transition) or by a proxy configuration instruction
%to clear the cache (i.e., configuration-based state transition). This extra
%degree of freedom may enable exploring the state space of the data plane more
%efficiently.

%\subsection{Testing Real Networks}
%\label{subsec:realnets}

\myparatight{Interference and diagnosis} One natural concern is that our
testing may interfere with background/non-test traffic.  There are two main
concerns here. First,  since the normal network traffic changes the state of
the data plane, it may impact the correctness of our test scenario and our
observations. Second, we need to make sure the test traffic does not change the
network state such that adversely affects  regular traffic (e.g., an IPS counter
might be increased beyond the alarm threshold).  To tackle these challenge, we
plan to use new  middlebox APIs such as FlowTags~\cite{flowtags_nsdi} or
OpenNF~\cite{openmb} to query the \DPF state and use new SDN capabilities for
ubiquitous control/data plane logging~\cite{netsight}. This helps in two ways. First,
knowledge of the current network state can minimize interference during test
generation.  Second, given that interference is unavoidable, we can use these
status reports to determine the root cause of a test failure.

% e.g.,  
%middenables 
%querying the current state of middleboxes (e.g., the current request-to-server 
%mappings in a load balancer), analogous to today's controller's capability to
%query switch statistics.

  
%to conduct a test, the controller 
%needs to be able to efficiently query the current data plane state before 
%computing and injecting the test manifest. Conversely, 
%One approach to tackle this challenge is to extend of the
%\myparatight{Diagnosis} 
%While the capability of determining whether the data plane 
%satisfies the policy goals is useful, it is not sufficient: if the test fails, we want to 
%determine the root cause(s) behind it (e.g., middlebox mis-config, middlebox bug, 
%broken link, or router bug) to tackle the problem. At a minimum, incorporating a  
%traceroute-like capability into \Name may help locate the problematic network 
%element. 


%\myparatight{Integration of existing device-specific test tools}
%There are many tools for penetration tests (e.g., Metaspoilt~\cite{metasploit},
%pytbull~\cite{pytbull}) 
%and other types of device-specific tests that focus on individual network elements 
%o%r policies and cannot serve the goal of testing network-wide policies involving 
%v%arious stateful elements. Integrating them into the \Name framework is a direction
%o%f future work.

%\subsection{Alternative Approaches to Planning}
%\label{subsec:alternative}




==> deprecated/earlyresults.tex <==
\section{Implementation and Early Evaluation}
\label{sec:promise}

Next, we describe the preliminary promise of implementing the 
 test traffic planner using  GraphPlan~\cite{graph plan}, an open source AI planning tool.

 
%to generate a \emph{high-level test plan}. 
  \begin{figure*}[t]
	\subfloat[L-IPS-H-IPS example]
	{
	\includegraphics[width=240pt]{./figs/ex2-entire-code.pdf}
	\label{fig:code:example2}
	}
	\subfloat[Firewall-Proxy example]
	{
	\includegraphics[width=240pt]{./figs/ex1-entire-code.pdf}
	\label{fig:code:example1}
	}
  \tightcaption{Code snippets for the two example scenarios in the GraphPlan language. Keywords are shown in Uppercase while  predicates are italicized.
  Each network input (i.e., a packet or a flow) is a parameter. 
  Each state  is captured by a  predicate with (possibly empty) parameters.   
 Each ``operator'' models  a state transition with (possibly empty) parameters.  We  input the initial states and the desired goal state.} 
 \end{figure*}


% using AI planning tools.  To make the 
%discussion concrete, we walk through the example in 
% Figure~\ref{fig:lips-hips}, and focus on starting  from the initial
% state where the network has observed no traffic to a ``goal'' of
%  taking the network to  the state where the heavy IPS is triggered.

\subsection{Implementation in GraphPlan}

GraphPlan provides a natural way to encode the state machines 
 and \DPF composition we saw earlier in \S\ref{sec:details}.
Figure~\ref{fig:code:example2} shows the corresponding 
GraphPlan code snippet for the state machines.

Here, we have a logical universe of possible traffic events, which are modeled
as {\tt parameters} within the GraphPlan language. In \Name, parameters are
network packets or flows with specific attributes; e.g., a port-80 HTTP
connection.  Each logical state in a \DPF state machine is represented as a
specific  {\em predicate}.  Some predicates may be additionally associated with
a given parameter; e.g., for a stateful firewall $\mathit{new}\langle x
\rangle$ indicates that the flow $\langle x \rangle$ is logically in state
$\mathit{new}$, whereas for a L-IPS the counting state is not parameterized by
a specific flow $\langle x \rangle$.  
 Each ``transition'' in the state machine is
represented as an ``operator'' in the GraphPlan language.  Each operator takes
as input one or more ``parameters, and gets triggered if its associated {\em
preconditions} hold true.  Once  the operator has completed its execution
(i.e., a state transition occurs), it has some {\em effects}, wherein
assertions involving \texttt{x} either become true or false.  As discussed in
the previous section, composition of \DPFs can be modeled as logical
preconditions that carry over from one \DPF model to the next.\footnote{We also 
 have models to capture  network-level state such as
  flow creation; we do not show these for brevity.}


To make this concrete, let us walk through the L-IPS--H-IPS example in Figure~\ref{fig:code:example2}.
  For brevity, we only show a subset of the possible transitions here. 
 Here, the states for the L-IPS are of the form {\tt count-*}.  The code shows that 
 in the state count-2, the  L-IPS will transition to the state count-3 if it sees a new failed connection.  
 It marks  this flow as seen using an auxiliary predicate
  as shown.  It also triggers another predicate {\em caused-lips-alarm} which is used 
 in the composition. The H-IPS is much simpler and the only states 
 are HIPS-OK and HIPS-ALARM; its precondition is that the processing is triggered 
 only if the {\em caused-lips-alarm} is true and it transitions to the HIPS-Alarm 
 state if it observes bot signatures in the flow $\langle x \rangle$. 
% \vyas{what does parameter mean for us?} 
Similarly, Figure~\ref{fig:code:example1} shows the code snippet for the
FW-proxy example.   While not shown here for brevity, we can also refine the
evict operator to distinguish different eviction reasons; timeout vs.\ cache
full. 



 % Figure~\ref{fig:lips-snippet-operators} 
%shows some GraphPlan code snippets to define the operators. The operators
%define \emph{network-level actions} (e.g., operators to create/finish a connection's traffic)
%as well as  \emph{middlebox-level actions} that express the intended network
%policies in terms of middlebox capabilities (e.g., operators to capture the counting 
%behavior of the light IPS). F

 In addition to the \DPF and composition models, we also  specify (a)
initialization conditions and (b) our intended {\em goal}.
Figure~\ref{fig:code:example2} also shows these initial conditions as
\emph{facts} describing our ``world'' where both L-IPS and H-IPS start in their
default states. Our  target goal state is to see 
 whether the H-IPS will raise an
alarm, if we have a sequence of three failed connections followed by a 
 specific payload value.   


We use  GraphPlan's in-built solver to generate a {\em plan} that will take us
from the initial state to the target goal state.
Figure~\ref{fig:lips-code-script} shows the solution generated by GraphPlan
showing the actions to take to reach the goal state for the L-IPS--H-IPS
example.  Given this high-level sequence of operators, we use a {\em
translation script} that uses  a
test traffic library to produce the {\em test manifest}. We currently manually 
populate this traffic library with different template traces; e.g., 
failed connections, web requests etc.

% as 
%generated by the test manifest generator component is shown in 
%Figure~\ref{fig:lips-code-script} ($server_1$ and $server_2$ shown in the Figure 
%are TCP servers running in our test bed).

\begin{figure}[t]
  \centering \includegraphics[width=220pt]{./figs/ips-code-script.pdf}
  \tightcaption{The test manifest to take the network of Figure~\ref{fig:lips-hips}
  to the goal state that the heavy IPS generates an alarm. The three rows in the
  figure correspond to $flow1$, $flow3$,  and $flow2$ of 
  Figure~\ref{fig:code:example2}, respectively.}
\label{fig:lips-code-script}
 \end{figure}

\subsection{Preliminary results}
\myparatight{Validation} To validate our test manifest,  we instantiate the network
topology using MiniNet.  We use Snort with different configurations to realize
the L-IPS and H-IPS functions, suitably  extended to support
FlowTags, so that we can route traffic depending on the L-IPS output~\cite{flowtags_nsdi}. 
 We use a custom version of  \texttt{POX} to set up forwarding
rules. 

%upport FlowTags 
%tagging operations), and Snort as both of the IPSes.\footnote{We use the 
%FlowTags-enhanced version of Snort for the light IPS, as the data plane forwarding 
%decisions depends on the outcome of the processing by this IPS~\cite{flowtags_nsdi}.}

We examined two scenarios. In the first scenario, we set up the network
elements correctly and ran the test manifest of
Figure~\ref{fig:lips-code-script}. The heavy IPS alarmed as expected and
blocked the malicious payload. In the second scenario, we
(mis-)configured the light IPS such that it alarms upon seeing the fourth
connection attempt (not the third one as mandated by the policy goal).  In this
case, we observed that injecting the test manifest does not trigger an alarm at
the heavy IPS and the flow  (i.e., the last row of
Figure~\ref{fig:lips-code-script}) passed through, violating the intended
policy.

\myparatight{Scalability} The examples of Figures~\ref{fig:proxy} and
~\ref{fig:lips-hips} each take about 3~ms to solve using GraphPlan. To
evaluate the scalability, we setup synthetic larger ``chains'' with 6 \DPFs
and 100 concurrent flows, where each \DPF can be in one of four states similar
to the stateful firewall. In this case, the solver takes around 1 minute, which
is manageable as we do not intend \Name to be a real-time system.   
 We found that the time to generate a plan grows roughly linearly as a
function of the number of operators in the model (not shown).

  
  
%measured the planner's run time in different scenarios running the planner on a
%commodity host.  The planner takes less than 1 minutes to find the solution in
%an adversary model, where the action traffic needs to be processed by a chain
%of middleboxes whose network-wide model involves 300 operators and over 1000
%propositions (this  is roughly equivalent of having 100 concurrent flows
%processed by a chain of six middleboxes, where each middlebox can be in one of
%the four possible states w.r.t. each flow, similar to the stateful firewall
%discussed in the previous section). Moreover, the runtime of planning grows
%linearly as a function of the number of operators in the model.

%\seyed{TODO 2: tie the stuff in this section more clearly to elements of section 3.}

%\seyed{TODO 3: highlight any unclear or important code snippet elements.}





==> deprecated/flowkeys.tex <==
A set of FlowTags (a \emph{TagSet}) can be associated with any
flow; however, the TagSet is not represented explicitly in the
packet headers.  Instead, the controller maintains a mapping
between TagSets and SDN flow-matching patterns, as well as a
mapping between TagSets and actions.   When anSDN switch
sees a packet for which it has no matching rule,
it sends (as is typical for OpenFlow) a packet-in message
to the controller, which responds with the appropriate
flow-table rule.  Likewise, when a middlebox sees such
a packet, it sends an analogous message to the controller
\jeff{this should be described in the southbound API!},
which responds with a new match-table rule, using the
actions defined in Sec.~\ref{southboundapi}.  Note that
the actions that the controller sends to a middlebox will
generally be quite different from those that it sends to
a switch.

With the current OpenFlow specification, the controller
needs to identify tagged flows implicitly, via standard
header fields (e.g., the IP/TCP 5-tuple).  However, it
might be more efficient (in terms of flow-table space and
control-message traffic) to use an explicit, opaque,
flow label in the packet headers.  The controller's match
rules could then match on flow labels, possibly covering
many TCP connections with one label.  With the current
OpenFlow spec, the only IPv4 field that could be used for
an explicit flow label is the 6-bit ToS field, although
perhaps the 16-bit IP-ID field could be handled with an
OpenFlow protocol modification.  For IPv6, the most recent
OpenFlow specification allows matching on the 20-bit flow-label
field.  (FlowTags might be a good resolution of the question
``how should we use the flow-label field?''~\cite{AmanteEtAl2012}.)
% AmanteEtAl2012 = 
% http://rmv6tf.org/wp-content/uploads/2012/11/rmv6tf-flow-label11.pdf
Our proof-of-concept experiments (Sec.~\ref{earlyresults}) use
the 6-bit ToS field.

\jeff{another issue: in the case where a proxy is muxing
requests from many sources onto one TCP connection, without
explicit flow labels, it would have to communicate with the
controller each time it changed the TagSet on a connection,
which would be really inefficient -- and might lead to races
with the rules in downstream network elements.  Do we have
a solution to this, beyond using the IP ToS bits as a way
to create a small flow-label namespace that is ``local'' to a
given 5-tuple?}


==> deprecated/intro.tex <==
\section{Introduction}
\label{sec:intro}
 
%% verification, bunch of work already done
Software-defined networking (SDN) has been instrumental in enabling new  {\em
testing and verification} capabilities. Specifically, we have seen many frameworks
to ensure that the network meets specific reachability properties (e.g.,  no 
black holes, no permanent loops, no access control violations).  These  include
work on   {\em static and runtime checking} of network configurations  (e.g.,
HSA~\cite{hsa}, VeriFlow~\cite{veriflow}),  {\em programming languages} for
 control applications (e.g., Frenetic~\cite{frenetic}), {\em test packet
generation}  tools  (e.g., ATPG~\cite{atpg}), and tools to  test control 
programs (e.g., NICE~\cite{nice}, VeriCon~\cite{vericon}).

% and techniques to improve the scalability of these methods (e.g.,
%NetPlumber~\cite{netplumber}, Libra~\cite{libra}).

%% real networks are unfortunately much more complex -- many more types of entities, 
 %%  more fancy policies,   %% stateful/dynamic actions 
 While the aforementioned efforts have taken significant strides,
  they still fall short of capturing {\em
realistic} network settings  on two key dimensions. (We elaborate on these in
\S\ref{sec:motivation}.)

\begin{packeditemize}

\item {\bf Complex data plane elements:} Studies have shown that there  are a range of advanced
 data plane functions (\DPF)\footnote{We use the  term \DPF   
  to encompass both physical hardware middleboxes and  virtualized instances.}
 including firewalls, load balancers, NATs, proxies,
intrusion detection and prevention systems, and application-level
gateways~\cite{aplomb,comb,mtcp_imc}. 
Unlike routers and switches,  such \DPFs are {\em stateful}. This  stateful 
 behavior manifests in different forms: (1)   \DPFs maintain {\em
connection- and application-level} context; e.g., a stateful firewall  allows
responses on connections established from inside a secure network; (2) 
  \DPFs track {\em state across connections} depending on the history
of observed traffic; e.g., a rate limiter may count the number of
active sessions, or  an IDS may keep track of recent failed
connections~\cite{trw}, or a proxy may store responses in its
  cache. 


% \seyed{this para might leave the reader with the impression that we are trying to
% solve the challenge of hidden states?}

\item {\bf Complex policy requirements:} While reachability is  
  necessary, it does  not capture  the full spectrum of 
 requirements that network administrators may want to verify. 
Administrators may want to ensure that  {\em service chaining} 
policies are implemented correctly~\cite{ietfnsc}.  
Other kinds of policies may focus on {\em dynamic dataflow} properties in
that the intended policy depends on the specific ``states'' of the  network. 
 For example,  we may want to ensure that traffic from suspicious hosts be routed through 
deep inspection proxies~\cite{prolexic}.

% Again, this falls outside the scope of 
%existing test and verification tools in the SDN literature.

\end{packeditemize}

%% our vision 
Such complex \DPF behaviors unfortunately fall outside the scope of existing
test and verification tools in the SDN literature.  For instance, while
verification tools can account for simple ``waypointing'' policies, they cannot
capture hidden actions of non-L2/3 data plane elements; e.g., a proxy sending
a cached response or a NAT rewriting headers.
 Our overarching vision  in this work is to bridge this gap between the promise of ``CAD for
networks'' vision~\cite{mckeowntalk}  and the 
capabilities offered by SDN tools today (\S\ref{sec:motivation}).  
 

 
%% why data plane testing
 In this paper, we focus on developing a practical {\em data plane testing}
framework called \Name to systematically test such stateful behaviors and policy
requirements.  We believe   data plane testing is a  more practical approach
compared to configuration testing or static verification approach on three
fronts. First, stateful behaviors of proprietary \DPFs may be  {\em hidden} and
{\em non-deterministic}.  For instance, we may not know the state of the object
cache in a proprietary proxy. Similarly, with load balancers or NATs, we may
not know the internal mappings between the incoming/outgoing connections.
Second, these behaviors may have subtle temporal effects; e.g., the
``counting'' behavior of a  rate limiter or the ``eviction'' behavior of a
cache may depend on internal timers.  Third, it might be difficult to precisely
model the  complex control logic that administrators want atop \DPFs; e.g.,
distributed middlebox load balancing~\cite{simplesigcomm} or elastic middlebox
scaling or migration~\cite{stratos,openmb,splitmerge}, or how they react to
network dynamics (e.g., link congestion or server load.

%\seyed{fourth reason?}




%Our goal is a {\em holistic test traffic
%generation} \seyed{how about ``test script?" b/c that may involve mbox config instructions etc besides pure traffic} 
%framework that can capture the types of complex data plane effects and new policy requirements outlined above.
%\seyed{i think we need to make it very clear why we need data plane test by giving
%root causes that cannot be captures otherwise like broken link, mbox bug, mbox
%misconfig, etc.}


%% insight
%Our goal is a {\em holistic test traffic generation} framework that can capture
%the types of complex data plane effects and new policy requirements outlined
%^above.  

 In conjunction, these stateful and dynamic effects require us to think beyond
 individual packets in designing test traffic~\cite{atpg}.
  Rather, what we need is a {\em trace} or a specifically
interleaved sequence of packets that logically {\em triggers} a chain of
specific state transitions in the data plane.  To this end, 
  \Name  models  \DPFs as
{\em state machines} where each state represents a state of the \DPF
(e.g.,  per-connection state for each session or the objects in the proxy
cache).  Given these models,  test trace generation can be formulated 
 as a problem of identifying
a sequence of transition events or a {\em plan}, that  move  the data plane
(i.e., the set of \DPFs) from the ``current state'' to a desired {\em goal}
state.  


 Specifically, we cast the trace generation
problem  within the framework of {\em planning} tools from the AI
literature~\cite{russel} and demonstrate the preliminary promise of using 
 existing planning tools like GraphPlan~\cite{graphplan} to generate test scenarios. 
 That said, however,  we do not claim that this is 
necessary or optimal---it gives us a
natural ``language'' in which to express our requirements. We are also 
exploring techniques from  software testing  including
fuzzing~\cite{fuzzing} and symbolic checking~\cite{symbex}.

% as natural enablers as well.

% we cast this here  
%we have a specific goal state and our objective is to take a sequence 
%of ``actions'' to reach the goal state~\cite{}.

In the rest of the paper, we begin by motivating the problem of stateful data
plane testing in \S\ref{sec:motivation}. We give an overview of  \Name 
 in \S\ref{sec:design} and show how planning tools can help generate a test
traffic sequence in \S\ref{sec:details} and \S\ref{sec:promise}. We
conclude with a discussion of open questions and challenges in
\S\ref{sec:discussion}. We discuss  related work inline throughout the paper.




==> deprecated/motivation.tex <==
\section{Motivation}
\label{sec:motivation}

We use two simple examples to highlight the challenges of 
 verifying complex policies with stateful \DPFs.
 Both examples highlight the need to (1)
use testing rather than static verification, (2) look beyond generating
individual test packets, and (3) be cognizant of the state semantics of \DPFs.
Table~\ref{tab:examples} summarizes the key aspects of these examples.
%to test why testing the data plane requires considering connection flows or
%sessions as the of test unit (as opposed to individual packets) and awareness
%of state semantics of middleboxes. Then we briefly discuss why existing work
%is not sufficient and motivate the need for {\em stateful data plane testing}
%that involves a systematic exploration of different states of the data plane,
%which is the foundation of \Name.


%\seyed{i replaced NAT with proxy as i think proxy creates the same challenge of
%NAT, plus i am giving the proxy model in section~\ref{sec:details}}
\subsection{Example Scenarios}

%\seyed{by now the reader must be clear why we need to test the data plane (as 
%opposed to static analysis such as hsa, nice).}

\myparatight{Example 1}
In  Figure~\ref{fig:proxy},  our policy goal is 
 to (a) always block unsolicited connections from the Internet
 and (b) block a subset of users from accessing specific sites. 
 The firewall and the proxy are stateful, operating above L2/3.
The stateful firewall operates based on a model of TCP connections and
maintains a state per connection (e.g., SYN observed, established, or invalid).
The proxy operates at the session level and  responds to  HTTP requests
directly if it has the object cached; otherwise, it retrieves the object from
the remote server. 
 Note that the proxy's state (i.e., the current cache contents) and firewall's
state (i.e., current connections status) at any given time might be hidden if
these are proprietary \DPFs (either hardware or virtual appliances), and depends
on the recent history.  

In this network, we may  want to test that the firewall is
correctly implementing the stateful semantics; i.e., it 
 only allows  reverse traffic for previously established connections. 
  Similarly, we want to systematically
explore different possible behaviors; e.g., do cached responses violate 
 the ``chaining'' policies?

%Thus, we cannot capture their behaviors using simple
%``transfer'' functions~\cite{}.  Similarly, while existing  test packet
%generation frameworks are sufficient to explore {\em stateless}
%\DPFs~\cite{atpg};  e.g., the forwarding/ACL actions of OpenFlow switches, they
%fall short in our scenario. 

\begin{figure}[t]
  \centering \includegraphics[width=180pt]{./figs/ex1_proxy_sdn14.pdf}
  \tightcaption{The stateful firewall maintains a state per TCP connection. The proxy's 
  state (i.e., cache contents) is determined by the history of observed traffic.}
\label{fig:proxy}
 \end{figure}

\myparatight{Example 2}
In Figure~\ref{fig:lips-hips}, we want to use the ``light'' IPS (L-IPS) to flag
hosts as suspicious and then subject traffic from the suspicious hosts to
deeper inspection at the ``heavy'' IPS (H-IPS).  For instance, L-IPS may check
if a host has $k$  consecutive failed connections~\cite{trw} and H-IPS may then
apply known botnet payload signatures.
%the light IPS raises an alarm, the heavy IPS, whose processing is more
%computationally costly, must perform deep packet inspection (DPI). In
%particular, the light IPS needs to raise an alarm if any host makes three or
%more TCP connection attempts made to the server, and the heavy IPS is expected
%to drop the packet if it includes an HTTP GET method.

 Now, testing that the configuration behaves as expected will 
require a systematic way to explore different 
 data plane states; e.g.,  (1) having less than $k$ 
 TCP connections established; (2) 
 $k$  TCP connections failed and a botnet payload was observed; and 
 (3)  $k$ TCP connections failed 
 but no botnet payloads were observed. 
 Exploring these different states requires 
taking into account the state semantics and configurations 
  of the L- and H-IPS.
 Again,  the count state of the L-IPS may be hidden and determined by internal
timeouts.

% thus, simple static checking may be insufficient.  Packet-level
%testing is insufficient, as our  intended policy here is an example of a
%dynamic data flow---traffic is routed to H-IPS only when L-IPS flags a host as
%suspicious. 
 

\begin{figure}[t]
  \centering \includegraphics[width=190pt]{./figs/ex2_IPS_sdn14.pdf}
  \tightcaption{The test scheme needs to be cognizant of both IPSes states and their event-driven logical connection.}
\label{fig:lips-hips}
 \end{figure}

\begin{table}[t]
\begin{small}
\begin{tabular}{l|l|p{2cm}|p{2cm}}
		&  & Example1 & Example2 \\ \hline 
	
\multirow{2}{*}{Dataplane}  & Stateful  & Firewall only allows valid connections &   Light IPS counts number of connections\\  
	  		   & Hidden  &  Proxy cache state & Counters/timers  \\  \hline 
\multirow{2}{*}{Policy}  & Chaining  & Per-user class service chains & Only suspicious hosts routed through heavy IPS \\  
	                 & Dynamic  &  Proxy cached responses &  Triggered action when connection count exceeds threshold   
\end{tabular}
\end{small}
\tightcaption{Summary of the motivating examples.}
\label{tab:examples}
\end{table}


\subsection{Current Solutions}
\label{subsec:related_limitations}

 At a high-level, prior work in the SDN testing/verification space has largely
focused on stateless reachability properties, and testing such stateful \DPFs or
dynamic data flow behaviors falls outside their scope.\footnote{To be fair,
they do explicitly mention that such stateful \DPFs are outside their intended
scope.}

%Testing network-wide policies in realistic stateful and dynamic middleboxes 
%falls outside the purvey of the prior work. The related work can be classified
%as follows:

\myparatight{Static verification} These methods (e.g., HSA~\cite{hsa})  take the data plane configuration 
and infer whether certain properties holds. However, they cannot be used to 
capture runtime data plane issues; e.g., they cannot capture the  hidden and 
dynamic states of \DPFs.
%NetPlumber~\cite{net plumber} and 
%Veriflow~\cite{veriflow} are run-time static verification methods that aim 
%to ensure at run time that modifying network configuration will not break 
%the desired properties. They are unable to capture stateful semantics of 
%the data plane as well is run time data plane faults.

\myparatight{Test packet generation} ATPG~\cite{atpg} generates test packets to
efficiently explore data plane reachability.  However, it cannot be used to
test stateful data planes; e.g., it doesn't capture the semantics of TCP
sessions or track history of previous packets to trigger cache evictions. 

\myparatight{Controller tools} NICE~\cite{nice} and VeriCon~\cite{vericon}
model SDN control applications  as state machines and use model checking to
find hidden logic bugs; they do not  capture data plane effects. Other language
frameworks (e.g., Pyretic~\cite{pyretic}) simplify SDN programming, but do not
 capture semantics of stateful \DPFs. 

\myparatight{Middlebox orchestration} Prior work  provides mechanisms 
 to ensure correct forwarding even in the presence of hidden \DPF actions. 
FlowTags requires  new APIs for \DPFs to expose information to SDN
controllers~\cite{flowtags_nsdi} while 
  Stratos explicitly replicates virtual middleboxes to avoid 
 such issues~\cite{stratos}.
  While these provide concrete  realizations,
 they cannot guarantee correctness; e.g., in the presence of failures.  In fact,
this paper is motivated by the inability to systematically test the
implementations in this previous work!


==> deprecated/newtagging.tex <==
\section{\Name Architecture}
\label{sec:tagging}


\begin{figure}[tbf]
  \centering \includegraphics[width=220pt]{./figs/flowtags_architecture.pdf}
  \tightcaption{{\bf The \Name architecture:} We highlight the extensions we introduce 
 as part of \Name.   We avoid explicit changes to switches or the need for 
  direct interfaces between  switches and middleboxes.}
%so that the corresponding  vendors  can innovate   independently.}
\label{fig:vision}
\end{figure}

The examples presented in the previous section show that the lack of visibility 
into middlebox actions hinders policy enforcement
and verification. Motivated by this observation, we propose \Name, an extended SDN 
 architecture that incorporates the necessary  visibility into middlebox actions
 in order to systematically  enforce and verify policies.

 In designing \Name, we impose three pragmatic constraints: (1) 
Require minimal
modifications to middleboxes, in order to spur adoption among middlebox vendors;
(2) Preserve existing switches as well as the switch-controller interface
(e.g., OpenFlow), to retain compatibility with switch vendors; (3) Avoid 
direct interactions between middleboxes and switches, to decouple the
evolutionary paths of these different classes of devices. 
 

The key idea in  \Name is to \textit{tag} packets with the necessary middlebox
context.\footnote{Context refers to middlebox-specific internal information that is
critical for policy enforcement, e.g., cache hit/miss in the case of a proxy or
the public-private mappings in the case of a NAT.} Thus, the packet processing
actions of a \Name-enhanced middlebox will now entail adding the relevant \Tags
into the packet header. The SDN controller configures the actions on switches
and middleboxes  to use these  \Tags (added by other middleboxes) as part of
their data plane operations,
in order to correctly enforce network-wide policies.


\subsection{Overview}
\label{sec:archoverview}
 SDN today provides an interface between the controller and switches to control
forwarding behavior. \Name extends this architecture 
along three key dimensions highlighted in Figure~\ref{fig:vision}: 

% (Jeff) I reordered these to place the most important dimension first.
\begin{packedenumerate} 

\item \Name-enhanced middleboxes that account for an incoming packet's
existing \Tags while processing it, and that may also add new \Tags based on 
the context. Switches use \Tags to steer packets. These data plane \Name-related
behaviors are discussed in \Section\ref{sec:dataplane}.


\item  New  \Name APIs
between the controller and \Name-enhanced middleboxes
% (i.e., middleboxes that are minimally extended to support tagging actions).
We highlight
these new APIs  in \Section\ref{sec:apis}. 

\item  New control applications that configure the tagging behavior of the middleboxes and switches,
and that also leverage \Tags to support policy enforcement and verification (\Section\ref{sec:apps}).

\end{packedenumerate}

Note that \Name neither imposes new capabilities on SDN switches nor requires direct signaling between middleboxes and switches; 
switches continue to use traditional SDN APIs.  The only interaction between switches
and middleboxes is (indirectly) via \Tags.  As discussed earlier, we take
this approach  to allow switch and middlebox designs to innovate independently
and to retain compatibility with existing SDN standards (e.g., OpenFlow). 


% (Jeff) I reordered the sentences somewhat, to improve the flow.
% I also cut some text that didn't seem to add much clarification.
Conceptually, each packet is associated with a set of \Tags. Given packet header space limitations,
packets only carry a compact encoding of the set, rather than the actual set of \Tags.
% with some suitable decoding logic.
(For clarity, we describe the design in terms of \Tags rather than their encodings.)
%versions with the assumption that these \Tags can be embedded
%within the ToS/DSCP field.  
%Our choice of 
Embedding this contextual information in the packets avoids the need for each  switch and
middlebox to communicate with the controller on a per-packet basis when making their 
forwarding/processing decisions.

With the current OpenFlow specification,  the only IPv4 field that we could use in
our current implementation (\Section\ref{sec:earlyresults}) to carry \Tags is the 6-bit
ToS/DSCP field.
% and we use this in our experiments
Newer standards could allow us to use additional header fields (\Section\ref{sec:apis_encoding}).


In the simplest case, when a switch sees a packet with a \Tag for which it has no 
matching rule, it sends (as is typical in OpenFlow) a packet-in message to the controller, 
which in turn responds with the appropriate \emph{FlowTable} rule.  Likewise, when a middlebox sees
such a packet, it sends an analogous message to the controller to learn the correct 
\Name-related action, using the functions described below.  In general, the actions that
the controller sends to a middlebox will be different from those that it sends
to a switch. To improve efficiency, in terms of table space and
control-message traffic, we can also install  \Name-related actions proactively.

\subsection{Southbound API}
\label{sec:apis}

We define an interface between the  enhanced SDN controller and \Name-enhanced
middleboxes in order to control the \Name-related behavior.  Note that
middleboxes are both \emph{producers}  (e.g., the NAT needs to expose
host-public IP mappings) as well as \emph{consumers} (e.g., the IDS scan
detector must use \Tags to attribute traffic to hosts)  of \Tags.  Corresponding
 to these two roles, we envision two configuration tables: (1)  Analogous to
the FlowTable rules in OpenFlow, each middlebox has a {\em \NameFlowTable} 
 to match flow patterns to \Tags; and (2) A {\em \NameActionTable} that maps 
 a packet with specific \Tags into (middlebox-specific) 
actions. 


\myparatight{\Tag addition} When a middlebox receives a packet that does not
match in \NameFlowTable, it queries the controller via
\requestTagAction(\PacketArg,\MboxSpecificContextArg) to obtain the relevant
rule.  The response from the  controller is a two-tuple of the form \mbox{$\langle$\FlowMatchArg,\TagArgNoSpace$\rangle$}.\footnote{\FlowMatchArg is 
analogous to {\tt struct ofp\_match} and can support wildcard entries.} The 
middlebox will add these specific \TagArg to packets matching the pattern \FlowMatchArg when the
context is \MboxSpecificContextArg.  Note that the controller may need context to
determine \TagArg; e.g., a proxy needs to declare if the packet was the result
of a cache hit/miss. We also envision other functions such as  \copyTag() (to
preserve  \Tags)  and \deleteTag() (reset after a \Tag has served its
purpose).  For brevity, we skip their details.\footnote{It might
seem that \copyTag is sufficient; i.e., a packet is tagged  when it enters the
network, and middleboxes simply preserve \Tags. However, there are scenarios
where \Tags need to reflect internal middlebox decisions; e.g., the proxy needs
to indicate if the response was the result of a cache hit or miss.}

\myparatight{\Tag consumption} We also need corresponding APIs to control how \Tags
affect a middlebox's packet processing actions. When a middlebox receives a
packet with  \Tags that do not have an action specified in the
\NameActionTable, it queries the controller via
\requestAction(\PacketArg,\TagArg)\footnote{We show \PacketArg and \TagArg
separately for clarity---physically, \TagArg is embedded in \PacketArg.} to
request the necessary packet processing action from the controller. The
controller responds with an appropriate \mbAction, in the form of a tuple 
of the form \mbox{$\langle$\FlowMatchArg,\mbActionNoSpace$\rangle$}, that is specific to the
middlebox; e.g.,   configuring how a NIDS should count packets for scan
detection.

% (This is sent only if the 
%middlebox does not already know what action to take on packet \PacketArg that
%includes \TagArg.)


\subsection{\Name Data Plane}
\label{sec:dataplane}

\myparatight{Middleboxes}  Adopting the \Name API entails two extensions to
middlebox software.  First,  vendors must support \Tag-writing functions. Our
experience suggests that many middleboxes (e.g., Squid, Bro) follow a
\emph{session-oriented} architecture, where each incoming connection is
associated with its attendant state~\cite{comb,SKGR:10short}.  Thus, we can add
the \Tags to this connection record structure and ensure that this information
is added to outgoing packets.  Second, and perhaps  more involved, middleboxes
need to incorporate \Tags  added by other middleboxes into their logic; e.g.,
when a NIDS or an ACRL attributes a packet to the principal.  Again, we can leverage
the  session-oriented model, to implement this logic. 


\myparatight{Switch extensions} Switches continue to match on  packet header fields
as defined by OpenFlow (or its descendants). They are agnostic to the semantics
of \Tags; these semantics are maintained at the controller.

\subsection{Control Applications}
\label{sec:apps}

We envision three new roles for  control applications:
 
\begin{packedenumerate} 

\item Analogous to today's SDN control applications for access control and routing,
we  need new control applications to translate a given set of network
policies into  (1)  \Tag addition/consumption at middleboxes, and (2) \Tag-based
packet forwarding rules at SDN switches. 

\item We will also need to develop a suite of verification applications to check whether 
  the set of desired policies  have been successfully enforced.
As we saw in the motivating examples, policy verification can be  difficult in the presence 
of dynamic middlebox actions, as we do not know how  a packet 
 is modified while traversing the network. By exposing \Tags, 
  \Name can even enable us to extend existing policy verification techniques
 (e.g.,~\cite{hsa})
 by treating \Tags as additional header fields.

\item Finally, we need a \Tag encoding layer  to support suitable 
 mechanisms to encode  \Tags given the available  packet header fields. 

\end{packedenumerate}


\subsection{End-to-End Example}

To make the above discussion concrete, we revisit  the proxy example
(Figure~\ref{fig:ratelimit}) extended with \Name as shown in
Figure~\ref{fig:tagsintuition}. As in traditional SDN, the controller maintains
a global view of the network state, including switch FIBs.  Additionally, the
controller maintains a copy the  \NameFlowTable and \NameActionTable
for each middlebox.  In this example, we need \Tags to both distinguish the
hosts and determine whether the request results in a cache hit. Corresponding
to these scenarios,   the proxy adds suitable {\Tag}s to outgoing packets as
shown; the FlowTables of the switches incorporate {\Tag}s in making forwarding
decisions.


\begin{figure}[t]
  \centering \includegraphics[width=220pt]{./figs/e2e_example.pdf}
  \tightcaption{ {\bf An example of using \Name:}  Each
packet carries the contextual information necessary for 
 correct  policy enforcement (e.g., which source? is this cached or not?)
 Only the forwarding rules affected by tagging are shown for brevity.}
\label{fig:tagsintuition}
\end{figure}

To see how using \Tags enables policy enforcement, suppose the content for
website xyz is in the proxy cache when H2 tries to access it for the first
time.  Upon receiving this request, the proxy sets $\Tag=4$ in  the  response
packet as it learns from the controller using the
\requestTagAction(\PacketArg,{\tt \{H2,HIT\}}) API call, where \PacketArg is
H2's HTTP request packet to get xyz. The proxy adds this $\Tag=4$ to the
(cached) response packet and sends it to S1. S1 forwards the packet to S2 and S2 forwards
it to the ACRL device. The ACRL device uses the \requestAction(\PacketArg,$4$)
API to learn the packet processing action for this packet, which in this
case is blocking the packet. (The API calls are not shown in the figure, for
clarity.)


As this example shows, \Name enables us to implement the intended access
control policy correctly even in the presence of dynamic and traffic-dependent
middlebox actions. In addition to policy enforcement, \Tags can also provide
new policy verification capabilities. For instance,  we can collect  packet-level logs at the switches and
middleboxes and correlate them using \Tags,  to create an end-to-end view of
a packet as it traverses the network.


==> deprecated/outline.tex <==
\section{Introduction}

\begin{packeditemize}

\item Networks' complexity makes them error prone. network operators (a.k.a. masters 
of complexity) need to make sure policies are enforced despite all this complexity. 
this is difficult today and the process is mostly ad hoc, manual, and error-prone.

\item While static verification is useful and has recently observed significant progress (e.g.,
~\cite{hsa, anteater}), it is not sufficient. many things can go wrong in specific realizations of 
the network (see~\S\ref{sec:motivation}). To verify successful enforcement of network policies 
given a real network, it is necessary to conduct verification as close to the wire as possible. 
To test the network in a live manner, we need to inject carefully selected test traffic into the 
data plane and verify the observed behavior of the data plane against the expected behavior 
mandated by the policies.a

\item Today's realistic network testing scenarios, unfortunately, fall outside the purvey 
of the existing work in that both policy requirement and data plane elements are 
\emph{stateful and dynamic}: 
(1) service chaining policies~\cite{ietfnsc} are by structure stateful and dynamic (e.g., send traffic
to the heavy IPS only if it has triggered an alarm on the light IPS) \seyed{this policy dimension
needs a more inclusive name/description given new scenarios beyond DPGs}, (2) many 
middleboxes that are widely used expose stateful and dynamic behavior
(e.g., stateful firewall, providing cached response by a proxy). These two dimensions
mandate test requirements that go beyond what existing solutions offer.

\item We take a step towards the overarching vision of CAD for 
networks~\cite{mckeown-sigcomm12} by developing \Name, a framework to efficiently test 
realistic data planes despite the above challenges. Given a set of network policy 
requirements, first, \Name helps model the data plane as a finite state machine to 
facilitate formulating the test goals and make the test process intuitive. 
Then \Name generates test traffic that is carefully chosen as to efficiently explore 
the ``state space'' of data plane. It then monitors network-wide behavior and validates 
it against the policies.

\item We make three contributions:

\begin{packeditemize}

\item \mypara{Modeling the data plane} We provide a framework to model individual data 
plane elements (e.g., firewalls, proxies) such that they can be composed with each other, 
yielding a \emph{data plane model} in form of a finite state-machine. This model, while being
intuitive to the human operator, is used to encode the intended policies and plan test
traffic.

\item \mypara{Planning test traffic} Given a set of intended network-wide policies as well 
as the data plane model, we identify and implement a ``network test planner". This involves 
formulating a test plan (i.e., what traffic/where/when to inject into the network) that 
strikes a balance between the \emph{efficiency} and \emph{coverage} of the test activity 
in realistic scenarios.

\item \mypara{Test validation} After injecting test traffic, \Name monitors the behavior 
of the data plane and infers whether it complies with our intended policies. In so doing, 
we have overcome the challenge of mutual \emph{interference} between regular network traffic 
(e.g., from users, departments) and test traffic, w.r.t. both performance and correctness.

\end{packeditemize}

\end{packeditemize}

This paper is organized as follows\dots

\section{Motivation}

\subsection{Motivating Scenarios}

\begin{packeditemize}

\item To bring a conceptual framework to motivation, maybe put a symbolic 2D plane figure 
here. the X-axis is policy space (i.e., things we want to enforce) and the Y-axis is data 
plane state space (i.e., what possible states the entire data plane can be in at any given 
time). on each axis there are a set of regions that we "care" about. the intersection(s) of 
them give(s) the region(s) that we need to focus on. give an example of how this region is
identified. then we can discuss there is no framework that helps us systematically these 
regions of concern.

\item {\bf Example 1---Reachability analysis} Lots of prior work on this, but they focus
on static analysis. This example shows how dynamic/static aspects of data planes/policies
can make existing work insufficient in reachability analysis.

\item {\bf Example 2---Dynamic policy graphs (DPGs)} One of the hotsdn examples?

\item {\bf Example 3---Security/Penetration test} 

\item {\bf Example 4---Fault tolerance} password attempts counting or firewall launching 
scenarios from toby?

\item {\bf Example 5---Cascaded NATs} \seyed{what example to present here?}

\subsection{Strawman Solutions}
Here we discuss the underlying reasons behind inadequacy of existing solutions to address
the above scenarios.\seyed{the goal here is no characterize why existing work fall short.
we'll probably keep the relwork as the final section.}

\begin{packeditemize}

\item Static verification~\cite{hsa, veriflow, netplumber}

\item Test packet generation~\cite{atpg}

\item Existing firewall/IPS testing tools~\cite{pytbull}

\item Testing control plane~\cite{nice,tshoot_sigcomm14}

\item Policy steering tools~\cite{simplesigcomm, flowtags_nsdilong}

\end{packeditemize}

\item We refute each of them in (a subset of) these four dimensions: 

\begin{packeditemize}

\item Failing to capture stateful/dynamic policies

\item Failing to capture stateful/dynamic data plane elements

\item Failing to capture data plane-level problems

\item Lack of network-wide testing

\end{packeditemize}

\end{packeditemize}


\section{\Name Overview}

\subsection{System architecture}

\begin{packeditemize}

\item describe the overall scenario.

\item make it clear that we are not verifying data plane implementation's correctness 
(as opposed to epfl14). we are testing whether the policies are enforced correctly.

\item walk through the solution components:

\begin{packeditemize}

\item data-plane modeler

\item test traffic planner

\item monitoring and validation engines

\end{packeditemize}

\end{packeditemize}

\subsection{End-to-end example}

\begin{packeditemize}

\item highlight why doing something trivial in each stage is not enough.

\end{packeditemize}


\section{Modeling Data Plane}

\subsection{Motivation}

\emph{Question:} Why do we model the data plane? 

Existing state of affairs w.r.t. real data planes is too complex. E.g., a real 
middlebox code base is too big and too complex. Modeling the data plane 
serves two goals:

\begin{packeditemize}

\item  Taming this complexity to enable systematic testing of the data plane

\item Help network operators understand the relevant stateful and dynamic behavior 
of the data plane

\end{packeditemize}

\subsection{Challenges and Strawman Solutions}

\begin{packeditemize}

\item \emph{Strawman solution 1}: Do not model the data plane altogether. E.g.,
just use the policy spec (e.g., the \DPG) to test the network. 

\item \emph{Rebuttal of strawman solution 1}: This is not sufficient: without accounting 
for the stateful nature of the data plane, we face two problems: (1) How to generate test 
traffic?, (2) Given test traffic, how to make sense of the test (e.g., what we have (not) tested)?

\item \emph{Strawman solution 2}: Just use located packet/transfer function as the model
of the data plane (e.g., HSA~\cite{hsa}). 

\item \emph{Rebuttal of strawman solution 2}: This approach cannot capture two important 
aspects of real data planes:

\begin{enumerate}

\item Stateful elements: HSA assumes a transfer function is just a function of input packet, 
not the possible \DPF's state.

\item HSA assumes the unit of processing is the same all through the data path (e.g., functions 
$f_1$, $f_2$, $f_3$,\dots each process input packet $X$ and throw out $f_3(f_2(f_1(X)))$). The 
reality is $f_1$ (a router) and $f_2$ (a packet filter) may act on a per-packet basis, but $f_3$ 
(a proxy) may process HTTP sessions. In other words, the \emph{operational semantics} and 
\emph{multiplicity}\footnote{For example, an HTTP GET packet as in input to a proxy can 
trigger a sequence of packets being sent by different network elements (e.g., a request from 
the proxy to the remote server, the response from the server to the proxy, and the response 
from the proxy to the client.)} of different functions may be different, which makes their 
composition non-trivial. 

\end{enumerate}

\subsection{Our Solution}
There are many ways of modeling a system. What are the \emph{data plane model requirements}?

\begin{packeditemize}

\item \emph{Model fidelity}: Each \DPF model must be loyal to the behavior of the actual \DPF. In
particular, it should capture the stateful and dynamic aspects of the data plane that affect 
policy correctness

\item \emph{Composabilty}: A network data plane is a naturally composed of individual elements. Can 
our model be composable as well? This is desirable since we can glue together individual element 
models according to the topology and create a network-wide data plane model.

\item \emph{Intuitiveness}: The model should be easy to understand by human operators.

\end{packeditemize}

\item Modeling assumptions:

\begin{packeditemize}

\item The middlebox implementation is ``correct'' (i.e., no crashed, unintended 
infinite loops, memory leaks). \seyed{we don't really need to assume this. if the 
middlebox is buggy it should show up in the test results.}

\item Access to middlebox code: ``whitebox modeling'' vs. ``blackbox modeling''

\item Model generation: hand-written vs. synthesized

\end{packeditemize}

\seyed{one tricky case is non-deterministic behavior of NATs etc. maybe we can use NFAs in this case 
with $\epsilon$ transitions. at least it can show us what kind of things can go wrong in the data plane.}

\item Our modeling approach:

\begin{packeditemize}

\item Model each \DPF as a Mealy finite state machine that takes as input a located packet and 
outputs a located packet. This approach makes the individual models naturally composable and also
makes it easy to state policy in terms of located packets (\seyed{back these up with examples}). 
We have developed such models for 
common stateful and dynamic \DPFs such as proxies, firewalls, IPSes, load balancers, and 
NATs.\footnote{Note that passive \DPFs such as passive monitoring and asset detection devices do not 
need to be modeled, as they do not affect networks' traffic.} 

\end{packeditemize}

\end{packeditemize}

\section{Test Traffic Planning}

\subsection{Motivation}

\begin{packeditemize}

\item Input: topology, data plane model, policies

\item Output: test plan which specifies what test packet to inject from where and when

\end{packeditemize}

\subsection{Challenges and Strawman Solutions}

\begin{packeditemize}

\item \emph{Strawman solution 1}: Manual test case generation

\item \emph{Rebuttal of strawman solution 1}: Ad hoc, difficult, and unscalable.

\item \emph{Strawman solution 2}: Use firewall/IPS test tools or fuzzers.

\item \emph{Rebuttal of strawman solution 2}: They can't tell us anything
beyond the behavior of a specific \DPF.

\end{packeditemize}

\subsection{Our Solution}

What are the \emph{test traffic requirements}?

\begin{packeditemize}

\item \emph{A way of expressing intended policies} \seyed{\DPGs may not be enough
given all the motivating examples. and the fact that time plays a role in certain policies}

\item \emph{Performance} of test traffic planning/generation

\item \emph{Overhead} of test traffic on the network

\item \emph{Coverage} of test. E.g., what ``states" our test traffic can cover?
Given a cap for test traffic volume, what states are more important to cover?


\item \emph{Coping with practical constraints}:  How to accommodate practical 
network constraints (e.g., i can use only a subset of hosts to inject test traffic; or, 
my test traffic should not be of a protocol that a firewall will drop)

\end{packeditemize}

Our test traffic generation approach based on symbolic execution:\footnote{
While our results using model checking and AI planning are similar to those
using symbolic execution w.r.t. test correctness, we faced performance limitations.}

\begin{enumerate}

\item Provide a clear way of defining policies 

\item Conduct static analysis based on data plane models and policies to find 
possible violations.\seyed{we need device configurations/ACL files here too.}

\item The preprocessing stage using topology and policies to determine
symbolic variables.

\item Generate a test traffic plane using symbolic execution.

\item Post process the test traffic plan to generate test traffic (i.e.,
concrete packets to inject into the network along with injection locations
and times).

\end{enumerate}


\section{Test Validation}
\subsection{Monitoring}

\begin{packeditemize}

\item show strawman solutions don't solve what this section achieves.

\item Input: test plan

\item Output: what can i infer wrt to policies? with what confidence?

\item Goal: capture enough traffic to make inference possible

\item challenges: 

\begin{packeditemize}

\item traffic log size. should sample in a meaningful way.

\item choice of monitoring nodes can be limited

\end{packeditemize}

\end{packeditemize}

\subsection{Validation}
\begin{packeditemize}

\item Input: policies, topology, captured monitored traffic, models

\item Output: what can i infer wrt to policies? with what confidence?

\item challenges: 

\begin{packeditemize}

\item ``performance interference'' with regular traffic: don't want to congest the network with test traffic

\item ``correctness interference'' with regular traffic: dint want to let the test traffic semantically make thing 
wrong for the regular traffic or vice versa (e.g., a counting up IPS)

\item diagnostics

\end{packeditemize}

\end{packeditemize}


\section{Related Work}

\Name encompasses several areas of related work. In what follows we briefly
characterize related work.

\subsection{Correctness assumptions}

\begin{packeditemize}

\item Correct by structure: This class of prior work assume the data plane
behaves as instructed by the control plane. They also do not consider middleboxes.
(e.g., Vericon~\cite{vericon}, Pyretic~\cite{pyretic}).

\item Static verification: The goal here is to analyze network's behavior given
data plane configuration. The two underlying assumptions are: (1) the control plane 
is manifested as configuration files, (2) the data plane behaves as instructed by
the control plane. Further, traffic modification and dynamic actions are not considered.

\item Live test: This category makes minimal assumptions about the correctness of
the data plane. The key idea is to verify network policies we need to inject traffic into 
the data plane and observe how it is treated in practice (e.g., ATPG~\cite{atpg}).

\end{packeditemize}

\subsection{Policies} Reachability, isolation, and loop-freeness have been widely considered
as the basic set of network properties or invariants. Policy chains and dynamic policy graphs
(\DPGs) specify more elaborate traffic processing aspects of the data plane.

\subsection{What to test}

\begin{packeditemize}

\item control plane

\item data plane

\end{packeditemize}

\subsection{Techniques}

\begin{packeditemize}

\item MC

\item Symbolic execution

\item Model-based testing?

\item \dots

\end{packeditemize}

\section{Evaluations}

\subsection{Evaluation Questions}

\begin{packeditemize}

\item Q1---Can we model the data plane correctly?

\begin{packeditemize}

\item element model validation---have we modeled each data plane element correctly?

\begin{packeditemize}

\item introduce bugs (w.r.t. policies) into code and see if that is captured in the model

\item use test traces and compare the output of the code and the model on test trace

\end{packeditemize}

\item data plane model validation---have we modeled the entire data plane correctly?

\begin{packeditemize}

\item in a given network test trace, is there any discrepancy between the data plane and the model w.r.t. policies?

\end{packeditemize}

\end{packeditemize}


\item Q2---Can we model the data plane efficiently?

\begin{packeditemize}

\item how long does it take to synthesize data plane model? is it a function of LoC?

\item we need to somehow show the trade-off between model's size and usability. maybe belongs
to the following questions.

\end{packeditemize}

\item Q3---What kind of bugs can \Name capture? ---the 
metrics here is coverage (i.e., what fraction of bugs \Name find.)

\begin{packeditemize}

\item known correctness bugs

\item new correctness bugs

\item synthesized correctness bugs

\item performance bugs

\end{packeditemize}

\item Q4---Can \Name effectively cope with interference?

\begin{packeditemize}

\item correctness interference

\item performance interference

\end{packeditemize}

\item Q5---What is the performance of \Name?

\begin{packeditemize}

\item how long does it take to test the policies? 

\begin{packeditemize}

\item break it down to its states: (1) planning, (2) injection and monitoring, (3) validation

\end{packeditemize}

\item memory and bandwidth overhead

\end{packeditemize}

\item Q6---Does \Name scale?

\begin{packeditemize}

\item run time as a function of policy complexity, and as a function of network topology

\end{packeditemize}

\end{packeditemize}

\subsection{Practical Insights}
Anything cool we learned or found (bugs, roadmap insight, practical challenge).

\input{concerns}



==> deprecated/relwork.tex <==
\section{Related Work}

 
{\bf Static Checking:} Checking the network configuration in order to detect bugs after they have occurred
has been explored in ~\cite{anteater} and ~\cite{hsa}. Possibility of violating network invariants (e.g.,
reachability constraints and routing loops) is modeled as a SAT problem in Anteater~\cite{anteater}. The 
corresponding tool provides a counterexample of packet headers that violate the invariants. The main idea 
in Header Space Analysis (HSA)~\cite{hsa} is to model network topology and forwarding behavior as transformations
on packet headers. This enables us to reason about configuration invariants independent of specific protocols.
Static checking is not sufficient for the cases where we would like to prevent violations from happening.

{\bf Dynamic Checking:} Veriflow~\cite{veriflow} is a framework for detecting violations in real-time. All
possible flow paths of the network are modeled as forwarding graphs, where each forwarding graph is associated
with a an equivalence class of traffic (i.e., packets that experience the same set of forwarding actions). By
maintaining forwarding graphs updated, violation against invariants can be queried and prevented upon insertion
of a new rule or deletion of an existing rule. NetPlumber~\cite{netplumber} is a verification tool based on the 
principles of HSA~\cite{hsa}. NetPlumber, however, runs much faster than HSA due to running checks in an
incremental fashion: only the parts of the forwarding behavior that are affected by a change are updated.

The above static and dynamic techniques for configuration verification are unable to accommodate the case 
that `dynamic boxes' are present in the network: if a switch or middlebox change packet content, or its 
forwarding behavior follows a randomized algorithm, the above techniques cannot be applied.


\mypara{New middlebox extensions} It might appear that if all middlebox functionalities required for each traffic
can be applied at a single location rather than at different individual middleboxes,
the problem can be solved. CoMb~\cite{comb} is an example of consolidating various
middlebox functionalities, possibly within an individual machine. A policy shim steers 
traffic to and from various modules, each corresponding to a middlebox. While being 
partly helpful, the shim needs to determine the correct order of traversing middlbebox
modules such that the polices are enforced consistently. This approach reduces to the
previously described attempt of rearranging middleboxes, and therefore, is insufficient.

Add jeff's ref.

{\bf Monitoring:} Automatically testing network configuration is explored in~\cite{atpg}. A minimal
set of test packets are generated to exhaustively verify each forwarding rule across the network.


==> deprecated/tagging.tex <==
\section{\Name Architecture}
\label{sec:tagging}



To address this lack of visibility, we need middleboxes to export some contextual
 information  between incoming and outgoing traffic. One option is for middleboxes
 to provide a logical ``query-response'' interface wherein the SDN controller
 can reactively query the middlebox for the required information.  The second approach 
 is to enable middleboxes to  logically mark packets 
 with the relevant contextual information. The 
 problem with the former  approach is that the controller  needs to be  
 involved at a per-packet granularity at every network hop increasing both 
 network and controller overhead. In contrast, the packet marking approach 
 lends itself to an architecture where the controller can even \emph{proactively} 
 setup the necessary forwarding and packet processing rules.  Thus, 
 we choose a packet marking based approach in our \Name architecture. 
 
\begin{figure}[tbf]
  \centering \includegraphics[width=220pt]{./figs/flowtags_architecture.pdf}
  \tightcaption{{\bf The \Name architecture:} We highlight the extensions we introduce 
 as part of \Name.   We avoid explicit changes to switches or the need for 
  explicit interfaces between  switches and middleboxes.}
\label{fig:vision}
\end{figure}




\Name  requires (minimal) extensions to middleboxes to add
logical {\em \Tags}  to provide the relevant context  between incoming
and outgoing traffic; e.g., which source caused this packet to be sent, or
whether this response was cached.  Other switches (and middleboxes) use the
\Tags in conjunction with traditional network-layer information to perform
their data plane actions.   

\subsection{Overview} 

SDN controllers configure the tagging actions on middleboxes using the  new
\Name API (Figure~\ref{fig:vision}).  It is important to 
note  \Name does not impose new capabilities
on SDN switches and does not  require explicit signaling between middleboxes
and switches. Switches continue to use
traditional SDN APIs such as OpenFlow. 
 The only signaling between switches and middleboxes is through
the \Tags.  We take this stance for two practical reasons: (1) to allow switch
and middlebox designs to innovate independently and (2) to retain compatibility
with existing SDN standards such as OpenFlow. 


Conceptually, each packet is associated with a set of logical \Tags. The \Tags
need not be explicitly specified in the packet headers due to header space
limitations.  Packets carry a compact encoding or a \TagEnc that
indexes into a \Tags mapping table. This mapping table is maintained at the
controller; middleboxes and switches  receive the mappings relevant to their
actions.  With the current OpenFlow specifications,  the
only IPv4 field that could be used is the 6-bit ToS/DSCP
field and we use this in our experiments
(\Section\ref{sec:earlyresults}); newer standards could allow us to use  additional fields 
\Section\ref{sec:discussion}).



In the simplest case, when a
switch sees a packet with a \TagEnc for which it has no matching rule, it sends
(as is typical for OpenFlow) a packet-in message to the controller, which
responds with the appropriate flow-table rule.  Likewise, when a middlebox sees
such a packet, it sends an analogous message to the controller which responds
with a new rule, using the actions defined below.  In general, the actions that
the controller sends to a middlebox will be different from those that it sends
to a switch. To improve efficiency, in terms of flow-table space and
control-message traffic, we can also install  \Tag-related actions proactively.
 



\subsection{The \Name ``southbound'' API}

%\vyas{either say whats new or shrink this to avoid increasing expectation} -- DONE

We define an interface between the  enhanced SDN controller and
modified middleboxes in order to control the tagging-related behavior.  Analogous to
the \emph{FlowTable} rules in OpenFlow, we envision a {\em \NameTable} on each
\Name-enhanced middlebox that maps packet descriptors into
corresponding tagging actions. 


%\begin{packeditemize}

%\item {\bf \Tag modifications:} 
\mypara{\Tag addition} 
  A basic function is \requestTagAction(\Packet,\TagEnc), which 
 the middlebox uses to obtain the relevant tagging actions 
 from the SDN controller for a new packet that does not match any previous 
 tag addition rule.  
 The \appendTag(\Packet,\MboxSpecificContext,\TagEnc) function 
 signals the middlebox to add specific \TagEnc to packets matching
the \Packet description.  Note that this action may need 
 middlebox-specific context; e.g.,  proxy needs to  identify if the packet
was the result of a cache hit/miss. We also envision other 
 basic functions such as  \copyTag (to preserve 
 \Tags)  and \deleteTag (reset after the \Tag has served its purpose).

\vyas{im not sure i like the defn of these functions . .what is input, what is output, who 
 is the sender, recipient etc, why do some  have tagenc in argument while others dont etc}

\vyas{one option is to make it vague and not show any params}


%%\vyas{Address concenr about preserve vs add tags} DONE

 At first glance, it might seem that the \copyTag capability is sufficient;
i.e., a packet is tagged with the necessary information when it enters
the network and middleboxes simply preserve these \Tags. Note, however, that
there are scenarios where we need \Tags to reflect internal middlebox
decisions; e.g., the proxy needs to indicate if the response was a cache hit or
miss. Thus, we make a conscious choice to add \Tags at middleboxes  rather than
at hosts or switches because they are the only network elements with sufficient
context.

% to add \Tags.
\mypara{\Tag consumption} Middleboxes are both  producers as well as consumers
of the \Tags. Thus, we  need corresponding mechanisms to control how 
 the \Tag information is used. 
  From our motivating scenarios, we see
that \Tags help in \emph{attributing} traffic to some
network-level \emph{principal} (e.g.,  source or flow).  
%To this end,  we
%envision  API calls to specify the attribution logic.  
 The
\requestAttribute(\Packet,\TagEnc) function is used by a middlebox to request
the controller to provide the necessary attribution logic.  Correspondingly, the
\getPrincipal(\Packet) call maps  the header and \TagEnc
information to a suitable principal; i.e., conceptually decoding the \TagEnc.

%\seyed{
%two things: 1) how about changing MapAttr->ReplyAttr? 2) TagEnc is a field of the packet
%(as used in MapAttr(Pkt.TagHdr, Pkt.TagEnc). So the notation RqstAttr(Pkt,TagEnc) in which they 
%look separate might be confusing.}

%	\end{packedenumerate}

%For
%instance, in our example,  \Tag=1 identifies H1 and \Tag=2 identifies H2;  the
%IDS is simply given rules for the mapping function \getPrincipal(*,1) = H1 and
%\getPrincipal(*,2) = H2 so that it can attribute the connection request to the
%exact source.

%\end{packeditemize}

%Can we retrofit this into existing middleboxes?
%Are there natural chokepoints?




\subsection{\Name data plane}


\mypara{Middleboxes}   Adopting the \Name API entails two extensions to
middlebox software.  First,  vendors must support \Tag-writing functions. Our
experience suggests that many middleboxes (e.g., Squid, Bro) follow a
\emph{session-oriented} architecture, where each incoming connection is
associated with its attendant state~\cite{comb,SKGR:10short}.  Thus, we can add
the \Tags to this connection record structure and ensure that this information
is added to outgoing packets.  Second, and perhaps  more involved, middleboxes
need to use \Tags  for attributing traffic to a network-level principal.  Again,
given a session-oriented model, we can create a lightweight translation layer
that interposes the \getPrincipal~call on  accesses to connection record
fields.


\mypara{Switch extensions} Switches continue to match on  packet header fields
as defined by OpenFlow (or its descendants). They are agnostic to the semantics
of the {\TagEnc}s; this mapping is maintained at the controller. That said, we
can improve the efficiency and avoid  controller overhead if the switches can
 match more header fields to reduce the number of \TagEnc
dereferences.

\subsection{Implications for policy verification}
Policy verification is very difficult in the presence of dynamic middlebox
actions. The underlying reason is that if we do not know how exactly a packet
is processed by a middlebox, we cannot determine whether the desired policies
are successfully applied. 

\Name demystifies middlebox actions by exposing (only relevant parts of) their 
actions, and so doing, enables us to apply policy verification techniques that 
rely on visibility of middlebox actions (e.g.,~\cite{hsa}).

\vyas{this is a bit vague and not technically interesting .. not sure it belongs here}

\subsection{An End-to-end example}

To make the above discussion concrete, we revisit  the proxy example extended
with suitable \Tags and actions as shown in Figure~\ref{fig:tagsintuition}. As
in traditional SDN, the controller maintains a global view of the network state
including the FIBs at each switch. Moreover, the controller maintains
the necessary \NameTable state for each middlebox in the network.  
In this example, we need \Tags to distinguish both the host and whether the
the request results in a cache hit/miss. Corresponding to these scenarios,   the proxy appends
suitable {\TagEnc}s to the outgoing packets as shown; 
 the FlowTables of the switches incorporate the {\TagEnc}s in making forwarding decisions.


\begin{figure}[t]
  \centering \includegraphics[width=220pt]{./figs/e2e_example.pdf}
  \tightcaption{{\bf Example using \Name:}  Each
packet carries the contextual information necessary for 
 correct  policy enforcement (e.g., which source? is this cached or not?).
 Only the forwarding rules affected by tagging are shown for brevity.}
\label{fig:tagsintuition}
\end{figure}

To see how using \Tags enable policy enforcement, suppose the content for website xyz 
is in the proxy cache when H2 tries to access
it.  Upon receiving this request, the proxy sets \TagEnc=4 in  the  response
packets using the API \appendTag(\Packet,\{H2,HIT\},4), where \Packet is a HTTP
request packet to get xyz. 
As a result, S1 will forward the HTTP response to S2 and S2 will forward
this to the ACRL device. The ACRL device uses the {\getPrincipal(\Packet)} API calls 
to decode the respective {\TagEnc}s, which in this example means identifying the host
and the requested content (all encoded in \TagEnc=4), and can correctly block the request.

%\vyas{say something abt benefits of tags} -- DONE

As the above example shows, \Name enables us to implement the intended access
control policy correctly even in the presence of dynamic and traffic-dependent
middlebox actions. In addition to enforcing the policy, the \Tags also provides
new capabilities for verifying that the intended policy is implemented
correctly. For instance,  we can collect  packet-level logs at the switches and
middleboxes and correlate them using the \Tags  to create an end-to-end view of
a packet as it traverses the network.


==> diff <==
3d2
< %\usepackage{lmodern}
77,78c76,77
< %\newcommand{\vyas}[1]{{\footnotesize\color{red}[VS: #1]}}
< %\newcommand{\seyed}[1]{{\footnotesize\color{blue}[SF: #1]}}
---
> \newcommand{\vyas}[1]{{\footnotesize\color{red}[VS: #1]}}
> \newcommand{\seyed}[1]{{\footnotesize\color{blue}[SF: #1]}}
80,81c79,80
< \newcommand{\vyas}[1]{}
< \newcommand{\seyed}[1]{}
---
> %\newcommand{\vyas}[1]{}
> %\newcommand{\seyed}[1]{}
96c95
< \title{\vspace{-30pt}\Name: Testing Context-Dependent Policies in  Stateful Data Planes}
---
> \title{\vspace{-30pt}\Name: Testing Contextual Policies in  Stateful Data Planes}
98c97
< \author{Seyed K. Fayaz$^\dagger$, Yoshiaki Tobioka$^\dagger$, Sagar Chaki$^+$, Vyas Sekar$^\dagger$ \\ $^\dagger$ CMU, $^+$ SEI \vspace{-30pt}} 
---
> \author{Seyed K. Fayaz$^\dagger$, Yoshiaki Tobioka$^\dagger$, Sagar Chaki$^+$, Vyas Sekar$^\dagger$ \\ $^\dagger$ CMU, $^+$ SEI} 
103a103,104
> 
> 
116,140c117
< 
< \newcommand\blfootnote[1]{%
<   \begingroup
<   \renewcommand\thefootnote{}\footnote{#1}%
<   \addtocounter{footnote}{-1}%
<   \endgroup
< }
< 
< 
< \renewcommand{\baselinestretch}{0.05}
< \blfootnote{\fontsize{4}{11}\selectfont Copyright 2014 Carnegie Mellon
<   University. This material is based upon
<   work funded and supported by the Department of Defense under
<   Contract No. FA8721-05-C-0003 with Carnegie Mellon University for
<   the operation of the Software Engineering Institute, a federally
<   funded research and development center. NO WARRANTY. THIS CARNEGIE
<   MELLON UNIVERSITY AND SOFTWARE ENGINEERING INSTITUTE MATERIAL IS
<   FURNISHED ON AN “AS-IS” BASIS. CARNEGIE MELLON UNIVERSITY MAKES NO
<   WARRANTIES OF ANY KIND, EITHER EXPRESSED OR IMPLIED, AS TO ANY
<   MATTER INCLUDING, BUT NOT LIMITED TO, WARRANTY OF FITNESS FOR
<   PURPOSE OR MERCHANTABILITY, EXCLUSIVITY, OR RESULTS OBTAINED FROM
<   USE OF THE MATERIAL. CARNEGIE MELLON UNIVERSITY DOES NOT MAKE ANY
<   WARRANTY OF ANY KIND WITH RESPECT TO FREEDOM FROM PATENT, TRADEMARK,
<   OR COPYRIGHT INFRINGEMENT. This material has been approved for
<   public release and unlimited distribution. DM-0001673.}
---
>  %% 0.5 buffer for rest


==> evaluation.tex <==
\section{Evaluation}
\label{sec:eval}
\seyed{TODO: use larger networks}
\seyed{TODO: effect of key ideas should be micro benchmarked}

In this section we evaluate the effectiveness and performance of \Name
and show that: (1) \Name's optimizations provide more than three 
orders of magnitude speedup and enable close-to-interactive running 
times even for large topologies (\S\ref{sec:eval_performance}); and 
(2) \Name successfully helps diagnose a broad spectrum
of data plane problems (\S\ref{sec:eval_effectiveness}); 
(3) \Name is also useful for incremental testing, testing \DPF 
implementations, and testing reachability (\S\ref{sec:eval_other}). 
We begin with our setup and approach.

\myparatight{Testbed} In order to run realistic large-scale
experiments with topologies of 100+ nodes, we use a testbed of 13
server-grade machines (20-core 2.8GHz servers with 128GB RAM)
connected via a combination of direct 1GbE links and a 10GbE Pica8
OpenFlow-enabled switch.
%We  also separately ran
%experiments on Mininet~\cite{mininet_hotnets}; we do not present these results
%for brevity as our testbed results supersede them.  
 On each server with KVM
installed,  we run each injectors and  middleboxes as separate VMs. The VMs are
interconnected via OpenvSwitch  on each server.  The middleboxes we use are 
 iptables~\cite{iptables} as a NAT and a stateful firewall,
Squid~\cite{squid} as  proxy, Snort~\cite{snort} as  IPS/IDS,
 Balance~\cite{balance} as the load balancer, and PRADS~\cite{prads} as a passive
monitor.  These were instrumented with {\tt FlowTags} to handle
dynamic middlebox actions~\cite{flowtags_nsdilong}.


\myparatight{Topologies and policies} In addition to the example scenarios from
\Section\ref{sec:motivation},  we use 8 recent ($>$2010)  topologies  from the
Internet Topology Zoo~\cite{topology_zoo}. We use these as
switch-level topologies and extend them with middleboxes and use
various service chaining policies; e.g., a policy chain of length 3
made of a NAT, IPS, and load balancer.

% \vyas{was there some rationale in picking these specific
%topologies?}
%\seyed{we should say we use these as switch topology. will be augmented 
%with \DPFs and end nodes to build complete networks.}

%\begin{table}[th]  
%\begin{small}
%\begin{center}
%    \begin{tabular}{ l|l}
%    Topology & \# of nodes \\ \hline
%    Heanet & 6 \\ %\hline 
%    Hostway International & 15	\\ %\hline
%    UniC & 25	 	\\ %\hline
%    Cwix & 35	 	\\ %\hline
%    Tinet & 52	 	\\ %\hline
%    OTEGlobe & 92 	\\ %\hline
%    TATA & 144	 	\\ %\hline
%    Cogent & 196 	%\\ %\hline
%    \end{tabular}
%\end{center}
%\end{small}
%\tightcaption{Topologies used in experiments.}
%\label{tab:topos}
%\end{table}

\myparatight{Background traffic} We generate background traffic
intended to {\em interfere} with the specific behaviors we want to
test; i.e., it induces state transitions that can affect our
tests. For example, in Figure~\ref{fig:dynamic_policy}, we use
background TCP port scanning traffic as it affects the suspicious
connection count per host at the L-IPS. Given the intended policies
and data plane model, we modify our trace generation tool for this
purpose.

%such interfering traffic. (We skip details for brevity and refer readers to our
%extended technical report~\cite{TR}.)

%------------------------------------------------------------------------------------%
\subsection{Performance and Scalability}
\label{sec:eval_performance}

One of our goals is that operators should be able to use \Name in a
reasonably interactive fashion; i.e., the time for an end-to-end test
should be a few seconds or less.

\myparatight{Test traffic generation} We measure the time for \Name to
generate a test trace across different topologies and service chain
sizes.  We evaluate the utility of the optimizations we introduced in
\Section\ref{sec:traffic-gen}.


%\vyas{how do we argue that the optimizations arent impacting correctness?}
%\seyed{optimizations are just using the info from intended policy and network 
%topo to help klee narrow down the search. maybe just say this in sec 6?}

Figure~\ref{fig:tg_latency_fixed_policy} shows the average time to
generate test traffic for a given intended behavior for a fixed
logical policy chain of length 3 (composed of a NAT, a firewall, and a
proxy) across different topologies. The smallest topology has one
instance of this logical policy chain (with 8 individual \intents),
and we increase the number of instances in other topologies linearly
with the number of switches; i.e., number of \intents and hence tests
grows linearly (this is done for other experiments of this subsection
too).  Since all values are close to the average, we do not show error
bars.  To put our numbers in perspective, using \klee without any of
our optimizations even on a network of six switches and one policy
chain instance with three middleboxes took over {\em 19 hours} to
complete.  The graph also shows the (projected) value of the
unoptimized setup using this baseline result.

%example (i.e., using no optimizations). We projected this value
%based on the measured one on the smallest topology due to huge run time.


The first optimization (minimizing the number of symbolic variables)
dropped the latency of the baseline example to less than 12 seconds
(more than three orders of magnitude reduction).  Constraining the
values of symbolic variables yields another $>9\times$ latency
reduction. Finally, other minor optimizations reduce the time for test
traffic generation by about $6\%$.

%\myparatight{traffic generaion latency---fixed policy}
%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=200pt]{./plots/traffic_gen_latency_fixed_policy_variable_topo_new.pdf}
  \tightcaption{Traffic generation latency with a fixed logical policy chain of length 3 across different topologies.}
  \label{fig:tg_latency_fixed_policy}
\end{figure}

%---------------------------------------------------------------------%

Figure~\ref{fig:tg_latency_fixed_topo} shows the average traffic
generation latency with a fixed topology with 52 switches (Tinet) and
variable policy chain length (all values were close to the average in
different runs). The effect of optimizations are consistent with
Figure~\ref{fig:tg_latency_fixed_policy}.

%\myparatight{traffic generaion latency---fixed topology}
%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=200pt]{./plots/traffic_gen_latency_fixed_topo_variable_policy_lines.pdf}
  \tightcaption{Test generation times for a fixed topology (Tinet + 53 switches) and variable policy chain length.}
   \label{fig:tg_latency_fixed_topo}
%\vspace{-0.3cm}
\end{figure}

%---------------------------------------------------------------------%
Recall that test generation in \Name has two logical stages: (1)
high-level test planning and (2) concrete test manifest generation. In
general, we find that the test manifest generation times are between
4--6\% of the time to generate the test plan and are largely
independent of topology size and policy chain length (not shown).

%\vyas{fig 4 -- add topology names? fix legend}

Overall these results confirm that with our optimizations, \Name is
practical and generates tests for even large topologies with 100+
nodes in less than 30 seconds.

%\vyas{what are these numbers for -- single line or the entire suite of intended behaviors?}

\myparatight{Monitoring overhead} Across different topologies using
the monitoring strategy of monitoring only stateful \DPF ports
outperforms \allPortsMon of \Section\ref{sec:validation} by at least
\%30 for the smallest topology and over $\times2$ for the largest
topology. The total size of the monitoring logs did not exceed $1\%$
of the total traffic volume across different topologies. Furthermore,
the fraction of the test traffic to the total network traffic (using
background traffic generated based on the gravity model traffic
matrix) is extremely small ($<$0.01\%). This is not surprising because
the duration of test is very short (less than 10 seconds) and the test
sequences we generate are targeted to trigger certain network
conditions (as opposed to large data transfers).

%\vyas{what is being measured? how is it being normalized?}

\mycomment
{
\begin{figure}[th]
  \centering
  \includegraphics[width=220pt]{./plots/mon_fixed_policy_variable_topo.pdf}
  \tightcaption{Normalized network-wide log size across different topologies.}
   \label{fig:mon_fixed_pol}
\end{figure}

Figure~\ref{fig:mon_fixed_topo} shows the normalized network-wide log
size across different policy chain lengths. Note that as the policy
chain size grows, the advantage of the second methods diminishes, as
there are more switch ports to monitor.

\begin{figure}[th]
  \centering
  \includegraphics[width=220pt]{./plots/mon_fixed_topo_variable_policy.pdf}
  \tightcaption{Normalized network-wide log size across various policy chain length.}
   \label{fig:mon_fixed_topo}
\end{figure}
}


\myparatight{Validation}The latency of validation is composed of two
components: analysis of monitoring logs and follow-up test traffic
generation (if necessary).  Table~\ref{tab:validation} shows the
average validation latency across different topologies. The policy
chain in this case is fixed (of length of three), and one randomly
selected data plane element fails. In another experiment (not shown)
we varied the length of the logical policy chain on fixed
topologies. The validation latency in this case increases linearly
with the length of the logical policy chain.  We also measured the
contribution of each of the validation stages (analysis of monitoring
and generating to the validation latency). Across different topologies
and policy chain lengths, generating follow up test takes between
between 26\% to 29\% of the total validation latency. In the largest
topology (Cogent) with 196 switches and 33 stateful \DPFs, validation
and follow up test took $\approx$42 and $\approx$17 seconds,
respectively.
% \vyas{give raw numbers not percentages}


 \begin{table}[t]
  \begin{center}
  \begin{footnotesize}
%  \begin{tabular}{p{1.2cm}|p{.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}}
 %         Topo.(\# of switches)   	  & Heanet(6)  	&  HtInt(15) 	& UniC(25) 		& Cwix(35) 		& Tinet(52) 		& OTEGlobe(92) 		& TATA(144) 	&Cogent(196)\\ \hline
  %        Time (s)               &  1.7    &  4.2          &7.1		& 10.4		& 15.2		& 28.0	        & 43.5		& 58.8     \\

  \begin{tabular}{p{1.2cm}|p{.8cm}|p{0.8cm}|p{0.8cm}|p{1cm}|p{0.8cm}}
         Topo.(\# of switches)     & Heanet (6)  & UniC (25) 		& Cwix (35) 		& OTEGlobe (92) 		&Cogent (196)\\ \hline
          Time (s)               &  1.7            &10.4	& 15.2		& 28.0	        	& 58.8     \\
     \end{tabular}
  \end{footnotesize}
  \end{center}
  \vspace{-0.4cm}
 \tightcaption{Validation times for different topologies.}
%  \vspace{-0.4cm}
 %\vspace{-0.1cm}
 \label{tab:validation}
 \end{table}

\mycomment
{
%\myparatight{validation latency fixed policy variable topology}
%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=220pt]{./plots/validation_latency_fixed_policy_variable_topo.pdf}
  \tightcaption{Validation latency across different topologies.}   
  \label{fig:validation_latency_fixed_policy}
\end{figure}

% %---------------------------------------------------------------------%


Figure~\ref{fig:validation_latency_fixed_topo} shows the validation 
latency across different policy chain lengths.

%\myparatight{validation latency fixed topology variable policy}
%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=220pt]{./plots/val_fixed_topo_variable_policy.pdf}
  \tightcaption{Validation latency across different policy chains.}   
  \label{fig:validation_latency_fixed_topo}
\end{figure}

% %---------------------------------------------------------------------%

We have also measure the contribution of each of the validation stages 
(analysis of monitoring and generating to the validation latency. Across 
different topologies and policy chain lengths, generating follow up test takes 
 between 26\% to 29\% of the validation latency. 


\mycomment{
Figure~\ref{fig:validation_latency_breakdown} shows the average 
breakdown of these two components across different topologies.

%\myparatight{validation latency fixed policy variable topology}
%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=220pt]{./plots/val_breakdown_fixed_policy_variable_topo.pdf}
  \tightcaption{Validation latency breakdown.}   
  \label{fig:validation_latency_breakdown}
\end{figure}
% %---------------------------------------------------------------------%
}
}

%------------------------------------------------------------------------------------%
\subsection{Validation}
\label{sec:eval_effectiveness}

\mypara{Finding hidden errors} We validate the effectiveness of \Name
using a {\em red team--blue team} exercise.  Here, the blue team
(Student 1) has a pre-defined set of \intents for each network; i.e.,
these are the expected behaviors and there is no ``overfitting'' or
additional instrumentation necessary for each run.  Then, the red team
(Student 2) picks one of the intended behaviors (at random) and
creates a failure mode that causes the network to violate this
\intent; e.g., misconfiguring the L-IPS count threshold or disabling
some control module.  The blue team used \Name to (a) identify that a
violation occurred and (b) localize the source of the policy
violation.  We also repeated these experiments reversing the student
roles; but do not show these results for brevity.


%\vyas{this fact that we pre-populate the set of
%all scenarios should be  specified in implementation}  \seyed{will do}

\begin{table}[t]  
\begin{footnotesize}
\begin{center}
    \begin{tabular}{ p{3.5cm} | p{3.5cm} }
    ``Red Team'' scenario &  \Name test trace that revealed the failure to ``Blue Team'' \\ \hline
Proxy/Mon (Fig.~\ref{fig:proxy_monitoring}); $S_1$-$S_2$ link is down &  Non-cached rqst from inside the Dept, followed by request for the same object from by another source host in the Dept\\ \hline
Proxy/Mon (Fig.~\ref{fig:proxy_monitoring}); The port of $S_1$ (Pica8)  connected to proxy is (mis)configured to not support OpenFlow & HTTP rqst from Dept	\\ \hline
 Cascaded NATs  (Fig.~\ref{fig:cascaded_nats}); {\tt FlowTags} controller  shut down &  $H_1$ attempts to access to the server \\ \hline
%Multi-stage trigger (Fig.~\ref{fig:dynamic_policy});  L-IPS  misconfigured to alarm after  5 conns \& Host $H_1$ makes 9 scan attempts. \\ \hline
 Multi-stage triggers (Fig.~\ref{fig:dynamic_policy}); L-IPS miscounts by summing three hosts  & $H_1$ makes 9  scan attempts followed by 9 scans by $H_2$  \\ \hline
Conn. limit.; Login counter resets  &  $H_1$ makes 3 continuous log in attempts with a wrong password   \\ \hline
Conn. limit.; $S_1$ missing switch forwarding rules from AuthServer to the protected server  & $H_2$ makes a log in attempt with the correct password
\end{tabular}
\end{center}
\end{footnotesize}
%\vspace{-0.3cm}
\tightcaption{Some example red-blue team scenarios.}
\label{tab:bug_scenarios}
%\vspace{-0.3cm}
\end{table}

%\vyas{check the table carefully!!}

 
Table~\ref{tab:bug_scenarios} highlights the results for a subset of
these scenarios and also shows the specific traces that blue-team
used.  Three of the scenarios use the motivating examples
from \Section\ref{sec:motivation}. In the last scenario
(Conn. limit.), two hosts are connected to a server through an
authentication server to prevent brute-force password guessing
attacks. The authentication server is expected to halt a host's access
after 3 consecutive failed log in attempts.  In all scenarios the
blue-team successfully localized the failure (i.e., which \DPF,
switch, or link is the root cause) within 10 seconds. Note that these
bugs could not be exposed with existing debugging tools such as
ATPG~\cite{atpg}, ping, or traceroute.\footnote{They can detect
  obvious failure modes such a link/switch being down but cannot
  capture subtle bugs w.r.t.\ stateful/contextual behaviors.}
 


%\vyas{were the last two scenarios not discovered?}

%\vyas{can we say why existing techniques would have failed here?}

%\vyas{can we say how long it took to do this end to end?}

%\vyas{are we modifying the policy/assertion for each scenario to be different? need some more details here}
%\seyed{this should go to implementation?}


\myparatight{Finding real bugs} \Name also helped us identify an
actual bug in our {\tt FlowTags} re-implementation in
OpenDaylight.\footnote{Our original implementation was in {\tt POX};
  the bug arose during the (non-trivial) process of porting it to
  OpenDaylight; OpenDaylight is a significant codebase with a lot of
  complexity.} Essentially, the controller code in charge of decoding
{\tt FlowTags} (e.g., to distinguish sources hidden behind a NAT or
proxy) was assigning the same tag value to traffic from different
sources.  By using test traffic in network of
Figure~\ref{fig:proxy_monitoring}, we observed that proxy hit replies
bypass the monitoring device, which is a violation of the intended
behaviors. \Name validation also localized the policy violation (i.e.,
at the proxy).  It also provided the traffic trace indicating that the
tag values of cache miss and hit cases are identical, that gave us a
hint to focus on the proxy tag assignment code of {\tt FlowTags}
controller.

%\vyas{this is too close to row 2 in the table?}\seyed{we have done one more scenario 
%with pica8 not supporting openflow on a certain port. maybe use than one instead of row
%2 of table?}

%effecting the violation helped us identify  the buggy behavior
% in the {\tt FlowTags} controller module. Specifically, the test trace 
%\vyas{how did we diagnose that it was a controller bug?}

%------------------------------------------------------------------------------------%
\subsection{Other use cases}%\seyed{must be shortened and maybe cite tech report for longer versions?}
\label{sec:eval_other}

\myparatight{Testing  {\tt Flowtags}-enhanced \DPFs} One of the  original
 motivations for \Name  was that  existing tools 
 were inadequate to test our {\tt FlowTags} implementation~\cite{flowtags_nsdilong}.  To this
end, we define intended behaviors for single \DPFs and exhaustively test
externally observable middlebox actions; e.g., the  tagging
behavior of the IPS to ensure it tags according to the intended alarm thresholds.

% We believe that the ideas in \Name may be  independently 
% helpful for testing individual middlebox implementations. 

\myparatight{Incremental Testing}:   One natural question is if  we can
incrementally test the network; e.g., when policies change. While a full
discussion is outside the scope of this work, we have early evidence to show
that \Name is amenable to incremental testing.  We update the set of \intents
that are affected by the policy change rather than rerun the full suite of
behaviors.  In general, incremental testing requires time
proportional to the fraction of affected \intents (not shown).

\myparatight{Loops and reachability} While reachability checking in stateless
data planes is a ``solved'' problem~\cite{hsa}, it is unclear if this is true
for stateful data planes. %To this end, We  extend \Name to  support
reachability properties via new types of assertions. For instance, to detect
loops we add  assertions of the form: {\tt assert(seen[ADU.id][port]<K)}, where
{\tt ADU} is symbolic \PADU, {\tt port} is a switch port, and {\tt K} reflects
a simplified definition of a loop that  the same \PADU is observed at the same
port $\geq$ {\tt K} times. Similarly, to check if some traffic  can reach  
{\tt PortB} from {\tt PortA} in the network, we initialize a \PADU with the port field 
 to be {\tt PortA} and use an assertion of the form {\tt
assert(\PADU.port != PortB)}. Using this technique we were able to detect 
synthetically induced switch forwarding loops
 (not shown).

% and traffic violating teachability policies. 

% \seyed{ack that existing
%work can do this too but this is just an extra feature of our system covering
%stuff beyond service chaining}




==> evaluation_before_vyas.tex <==
\section{Evaluation}
\label{sec:eval}
%\seyed{TODO: use larger networks}
%\seyed{TODO: effect of key ideas should be micro benchmarked}

In this section,  we show that \Name: \\
 (1) \Name's  enables close-to-interactive running 
times even for large topologies (\Section\ref{sec:eval_performance}); \\ 
 (2) \Name's design are critical for scalability 
(\Section\ref{sec:design_choices_effect}); and \\
% (3) \Name outperforms the 
%status-quo with respect to expressiveness and scalability 
%(\Section\ref{sec:status_quo});
(3) \Name successfully helps diagnose 
a broad spectrum of data plane problems 
(\Section\ref{sec:eval_effectiveness}).

% (5) \Name is also useful for 
%incremental testing and testing reachability (\Section\ref{sec:eval_other}). 
%We begin with describing our setup and approach.

\myparatight{Testbed and topologies} To run realistic large-scale experiments with large
topologies, we use a testbed of 13 server-grade machines (20-core 2.8GHz
servers with 128GB RAM) connected via a combination of direct 1GbE links and a
10GbE Pica8 OpenFlow-enabled switch.  On each server, with KVM installed,  we
run injectors and  software \DPFs  as separate VMs, connected via a {\tt
OpenvSwitch} software switch. The specific \DPFs are iptables~\cite{iptables}
as a NAT and a stateful firewall, Squid~\cite{squid} as  proxy,
Snort~\cite{snort} as  IPS/IDS, Balance~\cite{balance} as the load balancer,
and PRADS~\cite{prads} as a passive monitor.  

% To enable us to track dynamic middlebox 
% actions, these \DPFs were instrumented with tagging capabilities 
% similar to {\tt FlowTags}~\cite{flowtags}.

%These were instrumented
%with {\tt FlowTags} to handle dynamic middlebox
%actions~\cite{flowtags_nsdilong} (of course, \Name does not make any
%assumptions about the correctness of  {\tt FlowTags} as part of the policy
%enforcement mechanism).


In addition to the example scenarios from
\Section\ref{sec:motivation},  we use 8 randomly selected recent  topologies
from the Internet Topology Zoo~\cite{topology_zoo} with 6--192 nodes. We also
use two larger topologies (400 and 600 nodes)  by extending these topologies.
These serve as  switch-level  topologies; we  extend them with different \DPFs
to enforce service  chaining policies. 

% e.g., a policy chain of length 3 made of a NAT,  an proxy, and a firewall.

% \vyas{was there some rationale in picking these specific
%topologies?}
%\seyed{we should say we use these as switch topology. will be augmented 
%with \DPFs and end nodes to build complete networks.}

%\begin{table}[th]  
%\begin{small}
%\begin{center}
%    \begin{tabular}{ l|l}
%    Topology & \# of nodes \\ \hline
%    Heanet & 6 \\ %\hline 
%    Hostway International & 15	\\ %\hline
%    UniC & 25	 	\\ %\hline
%    Cwix & 35	 	\\ %\hline
%    Tinet & 52	 	\\ %\hline
%    OTEGlobe & 92 	\\ %\hline
%    TATA & 144	 	\\ %\hline
%    Cogent & 196 	%\\ %\hline
%    \end{tabular}
%\end{center}
%\end{small}
%\tightcaption{Topologies used in experiments.}
%\label{tab:topos}
%\end{table}

\comment{
\seyed{dropped background traffic stuff}

\myparatight{Background traffic} We generate background traffic
intended to {\em interfere} with the specific behaviors we want to
test; i.e., it induces state transitions that can affect our
tests. For example, in Figure~\ref{fig:dynamic_policy}, we use
background TCP port scanning traffic as it affects the suspicious
connection count per host at the L-IPS. Given the intended policies
and data plane model, we modify our trace generation tool for this
purpose.
}

%such interfering traffic. (We skip details for brevity and refer readers to our
%extended technical report~\cite{TR}.)

%------------------------------------------------------------------------------------%
\subsection{Scalability of \Name}
\label{sec:eval_performance}

We envision operators using \Name in a interactive fashion; i.e., the time for test generation should be 
 within 1-2 minutes even for large networks with hundreds of switches and 
middleboxes. To investigate this, first, we measure test traffic generation
latency of \Name across network topologies of different sizes. 

\comment
{To this
end, we fix the policy chain to a NAT, followed by a proxy, followed by 
a stateful firewall. The firewall is expected to block access from a fixed 
subset of origin hosts to certain web content. We connect a host to 
each switch. We set the total number of middleboxes to half the 
number of switches and connect each middlebox to a randomly 
selected switch while ensuring there is at most one middlebox 
connected to each switch. The smallest topology with 6 switches 
(Heanet) has one instance of the policy chain (i.e., using a NAT, a proxy,
and a firewall), and we linearly increase the number of physical chains
with the topology size (we use the same method in other experiments
of the section that involve various topologies). 
}

\mypara{Impact of topology size} For this experiment,  we fix the network
service chaining policy to include a NAT, followed by a proxy, followed by a
stateful firewall. The firewall is expected to block access from a fixed subset
of origin hosts to certain web content. To each switch-level topology, 
 we add  a  number of middleboxes (0.5$\times$ \#switches)  and connect each middlebox to a randomly
 selected switch with  at most one middlebox connected to each
switch. The smallest topology with 6 switches (Heanet) has one instance of the
policy chain (i.e.,  a NAT, a proxy, and a firewall), and we linearly
increase the number of such policy chains we want to test as a function of topology size. 


Figure~\ref{fig:new_topology_size_effect} shows the average test traffic
generation latency. (Values are close to the average we do not show error
bars). In the largest topology with 600 switches and 300 middleboxes (i.e., 100
policy chain instances), the traffic generation latency of \Name is 113
seconds. To put this number in context, we also show the traffic generation
time of a strawman solution of
$\langle\mathit{IO=Pkt},\mathit{Model=FSMsEnsemble},\mathit{Search=MC}\rangle$
using \cbmc~\cite{cbmc} as the model checker, which took about 25 hours in the
smallest topology with 6 switches and 3 middleboxes---about five orders of
magnitude slower than \Name.

%\footnote{We initially intended to use a more naive strawman 
%solution of the form 
%$\langle\mathit{IO=Pkt},\mathit{Model=ImplCode},\mathit{Search=MC}\rangle$
%using the implementation code as the model, but even in a topology 
%with one switch and one middlebox, test traffic generation did not 
%finish in 30 hours.} The figure also shows the projected values of this 
%strawman solution on other topologies based on this value.

%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=230pt]{./plots/new_scale_vs_topo.pdf}
  \tightcaption{Traffic generation latency as a function of topology size.}
  \label{fig:new_topology_size_effect}
\end{figure}
%---------------------------------------------------------------------%


\mypara{Impact of policy complexity}  Next we consider the effect of policy chain 
length on traffic generation time. We fix the topology to have 92 
switches (OTE GLOBE). We then take the above policy chain of 3 
middleboxes as a building block and build longer policy chains in which
the intended actoin depends on context from each of the middleboxes
on the policy chain. Figure~\ref{fig:new_policy_size_effect} shows 
the \Name traffic generation time as function of policy chain length; 
it is about 84 seconds in case of the longest policy chain with 15 
middleboxes. We also show the projected values of the above 
strawman solution as a point of reference.
%(Note that our goal here is to study the effect policy chain length; 
%otherwise, we believe it is extremely unlikely to see such a long 
%policy chain, e.g., between a host and a server, in real world.)

%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=230pt]{./plots/new_scale_vs_policy.pdf}
  \tightcaption{Traffic generation latency as a function of policy chain length.}
  \label{fig:new_policy_size_effect}
\end{figure}
%---------------------------------------------------------------------%

\mypara{Break-down of test traffic generation latency} Recall 
from~\Section\ref{sec:traffic-gen} that test generation in \Name 
has two stages. We find that translating abstract test traffic
into concrete test traffic composes between 4--6\% of the entire 
time to generate the test traffic; this is the case across different
topology sizes and policy chain lengths (not shown).

\mypara{Other latency components of \Name} As we say 
in~\Section\ref{sec:implementation}, after \Name generates 
test traffic, it injects the test traffic, monitors it, and determines 
the result. While the actual test traffic initiated by test traffic 
injection was observed on the data plane for less than 3 seconds 
in our experiments with 600 switches and 300 middleboxes 
(bulk of which is due to file transfers by HTTP/FTP), \Name 
monitors the network for a longer (and configurable) period 
of time  to ensure it captures any possible relevant traffic 
across the network (we have set this to 10 seconds). The 
average latency of analysis of collected monitoring logs
to determine the test result is shown in 
Table~\ref{tab:validation}.


 \begin{table}[t]
  \begin{center}
  \begin{footnotesize}
%  \begin{tabular}{p{1.2cm}|p{.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}|p{0.4cm}}
 %         Topo.(\# of switches)   	  & Heanet(6)  	&  HtInt(15) 	& UniC(25) 		& Cwix(35) 		& Tinet(52) 		& OTEGlobe(92) 		& TATA(144) 	&Cogent(196)\\ \hline
  %        Time (s)               &  1.7    &  4.2          &7.1		& 10.4		& 15.2		& 28.0	        & 43.5		& 58.8     \\

  \begin{tabular}{p{1.4cm}|p{.7cm}|p{1.2cm}|p{0.8cm}|p{0.7cm}|p{0.7cm}}
         Topo.(\# of switches)     &  Cwix (35)  & OTEGlobe (92) 	&Cogent (196) & 400-node & 600-node\\ \hline
          Time (s)               &   3.8  & 	 9.9     &   25.2 & 56.3 & 87.6   \\
     \end{tabular}
  \end{footnotesize}
  \end{center}
  \vspace{-0.4cm}
 \tightcaption{Latency of monitoring logs analysis across different topologies.}
%  \vspace{-0.4cm}
 %\vspace{-0.1cm}
 \label{tab:validation}
 \end{table}

%\seyed{monitoring and validation eval commented out for now...}
\comment{
\myparatight{Monitoring overhead} Across different topologies using
the monitoring strategy of monitoring only stateful \DPF ports
outperforms \allPortsMon of \Section\ref{sec:validation} by at least
\%30 for the smallest topology and over $\times2$ for the largest
topology. The total size of the monitoring logs did not exceed $1\%$
of the total traffic volume across different topologies. Furthermore,
the fraction of the test traffic to the total network traffic (using
background traffic generated based on the gravity model traffic
matrix) is extremely small ($<$0.01\%). This is not surprising because
the duration of test is very short (less than 10 seconds) and the test
sequences we generate are targeted to trigger certain network
conditions (as opposed to large data transfers).


\myparatight{Validation}

}
%------------------------------------------------------------------------------------%
\subsection{ \Name design choices}
\label{sec:design_choices_effect}

Next, we do a component wise analysis to demonstrate the effect of our key
design choices and optimizations.


\mypara{Code vs.\ models}  Running \klee on  smallest 
 \DPF codebase of around 2000 LOC (i.e., balance~\cite{balance}) took about 20 
hours. In very small experiment with policy chain of length 2 involving 
only one switch directly connected to a client, a server, a load balancer, 
and a monitor~\cite{prads}, traffic generation time took took 57 
hours (see~Table\ref{tab:se_on_code}).

% (Besides scalability, there 
%are also other practical limitations to symbolic execution tools with 
%respect to implementation language, multi-threadedness, etc; for 
%example, due to \klee constraints, we had to remove balance's 
%multithreading behavior to run \klee.)


 \begin{table}[t]
  \begin{center}
  \begin{footnotesize}

  \begin{tabular}{p{2.6cm}|p{2.6cm}|p{2.3cm}}
         			 &  Load balancer (LB)	& LB+Monitor\\ \hline
          \klee on ``raw'' code  &   20 (hrs)  & 	 57 (hrs)        \\ \hline
          \Name  &   $<$ 1 sec  & 	 $<$ 1 sec      \\
     \end{tabular}
  \end{footnotesize}
  \end{center}
  \vspace{-0.4cm}
 \tightcaption{Traffic generation latencies of \Name vs. use of symbolic 
 execution for search on implementation code as model.}
%  \vspace{-0.4cm}
 %\vspace{-0.1cm}
 \label{tab:se_on_code}
 \end{table}



\mypara{\PADU vs.\ packet} First, to see how aggregating 
a sequence of packets as an \PADU helps with scalability, we measured 
the number of packets in a HTTP request and responses across different 
file request scenarios in terms of the file size. Then we used \Name to 
generate test traffic to test the proxy-monitor policy of 
Figure~\ref{fig:proxy_monitoring_policy}, once in terms of \PADUs and 
the other time in terms of individual IP packets ,each of an 1500-byte 
MTU size, as the abstract traffic unit. The results are shown in 
Figure~\ref{fig:adu_effect}. Our experiments with FTP (not shown) 
in instead of FTP show consistent results. The take-away here is 
since the number of test packets is dominated by the number of object 
retrieval packets, aggregating all file retrieval packets as one \PADU 
significantly cuts the latency of the test traffic generation and make 
traffic generation time of \Name independent of such app-layer 
semantics.

%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=230pt]{./plots/new_bdu_vs_pkt.pdf}
  \tightcaption{Effect of using \PADU as the traffic aggregation unit in \Name.}
  \label{fig:adu_effect}
\end{figure}
%---------------------------------------------------------------------%





\mypara{Symbolic Execution vs.\ Model Checking} Our earlier results already
showed dramatic gains w.r.t.\ model checking on the raw code even on trivial
topologies. One natural question is if model checking could have benefited from
the other \Name optimizations.  We also independently compared the performance
gain of using symbolic execution (\klee~\cite{klee}) vs.\ model checking using
\cbmc~\cite{cbmc} if we made our ther optimizations such as FSM Ensembles,
\PADUs, and other SE optimizations (\Section\ref{sec:traffic-gen}) available to
the model checking solution.   This ``optimized'' model checking  was
significantly faster than before but it was still takes two orders of magnitude
slower than \Name (not shown).  This result suggests that while  our
abstractions may be independently   useful for other network verification
efforts using model checking , it is  not suitable for the interactive testing
scenarios we envision in \Name. 


% while using model checking by initializing 
%and constraining \PADU fields whenever possible. 
%The results are shown in Figure~\ref{fig:new_mc_vs_se} where 
%we increase the policy chain length. The optimized model checking 
%still takes two orders of magnitude longer than \Name to generate 
%test traffic despite all the extra optimizations.
%about 3 hours in a 600-node topology.


%---------------------------------------------------------------------%
\comment
{\begin{figure}[th]
  \centering
  \includegraphics[width=230pt]{./plots/new_mc_vs_se.pdf}
  \tightcaption{Traffic generation latency of \Name vs. optimized model checking 
  on FSM Ensembles based on \PADUs.\seyed{candidate plot to drop}}
  \label{fig:new_mc_vs_se}
\end{figure}
}
%---------------------------------------------------------------------%

\mypara{Impact of  SE optimizations} We examine the effect of the SE-specific
optimizations described in \Section\ref{sec:traffic-gen}  in
Figure~\ref{fig:opt_effect}. To put our numbers in perspective, using \klee
without any of our optimizations even on a network of six switches and one
policy chain instance with three middleboxes took over {\em 19 hours} to
complete.  The graph also shows the value of the unoptimized setup using this
baseline result (the unoptimized latencies are projected values based on the
19-hour latency in the smallest topology). The first optimization (minimizing
the number of symbolic variables) drops the latency of by more than three
orders of magnitude.  Scoping the values of symbolic variables yields another
$>9\times$ latency reduction. 

%Finally, other minor optimizations reduce the time for test traffic generation by about 
%$6\%$ (we do not show this in the figure, as the corresponding line 
%would overlap with the \Name line on the log-scale).


%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=230pt]{./plots/new_decision_effects.pdf}
  \tightcaption{Effect of optimizations on top of symbolic execution.}
  \label{fig:opt_effect}
\end{figure}
%---------------------------------------------------------------------%



\comment
{
%------------------------------------------------------------------------------------%
\subsection{Comparing \Name to the status quo}
\label{sec:status_quo}
We compare the expressiveness and scalability of \Name with 
representative existing approaches.

\mypara{Expressiveness} We choose ATPG, a recent as a recent 
active testing method, as a comparison point with respect to 
expressiveness. First, we tried but were not able to use ATPG 
to generate test traffic to test the policies in the scenarios of 
Figures~\ref{fig:one_fw},~\ref{fig:proxy_monitoring_policy},
\ref{fig:cascaded_nats}, and~\ref{fig:dynamic_policy}. This
is because ATPG is fundamentally incapable of testing 
scenarios that involve any stateful \DPFs and context-dependent 
policies for the reasons we discussed in~\Section{sec:motivation}.
Here we briefly summarize these experiments. In the simplest 
of these scenarios from Figures~\ref{fig:one_fw} we model the 
stateful firewall as a $(*,inSwPrt) \rightarrow (*,outSwPrt)$ 
transfer function as the header space algebra suggests~\cite{hsa}.
We repeated the test for 100 times with the goal of testing 
reachability from the Internet into the department, but ATPG 
never generated test traffic that can exercise the policy of blocking 
unsolicited traffic, since ATPG cannot capture any semantics 
beyond single-packet semantics. Next, in Figure~\ref{fig:cascaded_nats}, 
even if we assume that the NATs are both static (i.e., have a fixed 
external IP address) and that even their transport port mapping
behavior is static (a highly unlikely assumption in real-world NATs)
to enable capturing them as HSA-like transfer functions, the existence 
of the state of firewall created a smiler problem to the first simplified 
scenario. We had even more fundamental problems in using ATPG
in testing the scenarios of Figures~\ref{fig:proxy_monitoring_policy}
and~\ref{fig:dynamic_policy} due to context-dependent nature of the
policies. (We discuss the use of \Name in~\ref{sec:eval_effectiveness}.)

\seyed{commented out details}
\comment{
Next, we tried to use ATPG in two 
simplified versions of the scenario of Figures~\ref{fig:one_fw} 
 and Figures~\ref{fig:cascaded_nats} as follows.  
 In Figures~\ref{fig:one_fw}, suppose there is a host $H_1$ inside 
 the department and we replace the ``Internet'' 
in the figure with a host $H_2$. Switch $S_1$ is configured to send  
packets from the department or the server to the firewall, and 
packets from firewall depending on the destination IP, either to 
the department or the server. We model the stateful firewall as a 
$(*,inSwPrt) \rightarrow (*,outSwPrt)$ transfer function as the 
header space algebra suggests~\cite{hsa}. This model, however, 
is overly permissive by allowing every input packet to output from 
the firewall and reach the server. To see why, the packets 
generated by ATPG from originating at $H_2$ destined to 
$H1$, went to the firewall, which mirrors them out, and then 
the switch sends them to the server. Such a test packet, while 
injected into the the network, however, may or may not pass 
the pass the firewall and reach the hosts depending on 
firewall state associate with the connection. We repeated
the test for 100 times with the goal of testing reachability from 
$H_2$ to  $H_1$. We never receive test traffic that can exercise
the policy of blocking unsolicited traffic, since ATPG cannot 
capture any semantics beyond single-packet semantics.
We repeated the same experiment with 
Figures~\ref{fig:cascaded_nats} assuming they are static NATs,
which allows modeling their IP-mapping behavior by HSA-like 
transfer functions. However, the existence of the state of
firewall created a smiler problem to the first simplified scenario.
(We discuss the use of \Name in~\ref{sec:eval_effectiveness}.)
}
}

\comment
{
\mypara{Scalability} Ignoring the fundamental problem of using a 
middlebox's implementation code as model used for testing it, the 
code can be deemed as expressive model of the middlebox that 
naturally captures its stateful semantics. However, it is not practical 
to use any realistic middlebox code because of the well-understood 
limitations of symbolic execution. Running \klee on  smallest 
codebase of around  2K (i.e., balance~\cite{balance}) took about 20 
hours. In very small experiment with policy chain of length 2 involving 
only one switch directly connected to a client, a server, a load balancer, 
and a monitor~\cite{prads}, traffic generation time took took 57 
hours (see~Table\ref{tab:se_on_code}). (Besides scalability, there 
are also other practical limitations to symbolic execution tools with 
respect to implementation language, multi-threadedness, etc; for 
example, due to \klee constraints, we had to remove balance's 
multithreading behavior to run \klee.)
}

 \begin{table}[t]
  \begin{center}
  \begin{footnotesize}

  \begin{tabular}{p{4.9cm}|p{1.1cm}|p{1.3cm}}
         			 &  Load balancer 	& Load balancer+Monitor\\ \hline
          $\langle\mathit{IO=Pkt},\mathit{Model=Impl Code},\mathit{SE}\rangle$  &   20 (hrs)  & 	 57 (hrs)        \\ \hline
          \Name  &   $<$ 1 sec  & 	 $<$ 1 sec      \\
     \end{tabular}
  \end{footnotesize}
  \end{center}
  \vspace{-0.4cm}
 \tightcaption{Traffic generation latencies of \Name vs. use of symbolic 
 execution for search on implementation code as model.}
%  \vspace{-0.4cm}
 %\vspace{-0.1cm}
 \label{tab:se_on_code}
 \end{table}


%\vyas{what is being measured? how is it being normalized?}

\mycomment
{
\begin{figure}[th]
  \centering
  \includegraphics[width=220pt]{./plots/mon_fixed_policy_variable_topo.pdf}
  \tightcaption{Normalized network-wide log size across different topologies.}
   \label{fig:mon_fixed_pol}
\end{figure}

Figure~\ref{fig:mon_fixed_topo} shows the normalized network-wide log
size across different policy chain lengths. Note that as the policy
chain size grows, the advantage of the second methods diminishes, as
there are more switch ports to monitor.

\begin{figure}[th]
  \centering
  \includegraphics[width=220pt]{./plots/mon_fixed_topo_variable_policy.pdf}
  \tightcaption{Normalized network-wide log size across various policy chain length.}
   \label{fig:mon_fixed_topo}
\end{figure}
}


% \vyas{give raw numbers not percentages}




\mycomment
{
%\myparatight{validation latency fixed policy variable topology}
%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=220pt]{./plots/validation_latency_fixed_policy_variable_topo.pdf}
  \tightcaption{Validation latency across different topologies.}   
  \label{fig:validation_latency_fixed_policy}
\end{figure}

% %---------------------------------------------------------------------%


Figure~\ref{fig:validation_latency_fixed_topo} shows the validation 
latency across different policy chain lengths.

%\myparatight{validation latency fixed topology variable policy}
%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=220pt]{./plots/val_fixed_topo_variable_policy.pdf}
  \tightcaption{Validation latency across different policy chains.}   
  \label{fig:validation_latency_fixed_topo}
\end{figure}

% %---------------------------------------------------------------------%

We have also measure the contribution of each of the validation stages 
(analysis of monitoring and generating to the validation latency. Across 
different topologies and policy chain lengths, generating follow up test takes 
 between 26\% to 29\% of the validation latency. 


\mycomment{
Figure~\ref{fig:validation_latency_breakdown} shows the average 
breakdown of these two components across different topologies.

%\myparatight{validation latency fixed policy variable topology}
%---------------------------------------------------------------------%
\begin{figure}[th]
  \centering
  \includegraphics[width=220pt]{./plots/val_breakdown_fixed_policy_variable_topo.pdf}
  \tightcaption{Validation latency breakdown.}   
  \label{fig:validation_latency_breakdown}
\end{figure}
% %---------------------------------------------------------------------%
}
}



%------------------------------------------------------------------------------------%
\subsection{Validation\seyed{change title}}
\label{sec:eval_effectiveness}

Next	 we also demonstrate the effectiveness of \Name in finding 
policy violations in the data plane using a {\em red team--blue team} 
exercise.  Here, the red team (Student 1) informs of the blue team
(Student 2) of \intents for each network, and then secretly picks one of 
the intended behaviors (at random) and creates a failure mode that 
causes the network to violate this \intent; e.g., misconfiguring the 
L-IPS count threshold or disabling some control module.  The blue 
team used \Name to (a) identify that a violation occurred and (b) 
localize the source of the policy violation.  We also repeated these 
experiments reversing the student roles; but do not show these 
results for brevity.

\comment{
\mypara{Finding hidden errors} 
We validate the effectiveness of \Name
using a {\em red team--blue team} exercise.  Here, the blue team
(Student 1) has a pre-defined set of \intents for each network; i.e.,
these are the expected behaviors and there is no ``overfitting'' or
additional instrumentation necessary for each run.  Then, the red team
(Student 2) picks one of the intended behaviors (at random) and
creates a failure mode that causes the network to violate this
\intent; e.g., misconfiguring the L-IPS count threshold or disabling
some control module.  The blue team used \Name to (a) identify that a
violation occurred and (b) localize the source of the policy
violation.  We also repeated these experiments reversing the student
roles; but do not show these results for brevity.
}

%\vyas{this fact that we pre-populate the set of
%all scenarios should be  specified in implementation}  \seyed{will do}

\begin{table}[t]  
\begin{footnotesize}
\begin{center}
    \begin{tabular}{ p{3.5cm} | p{3.5cm} }
    {\bf ``Red Team'' scenario} &  {\bf \Name test trace} 
    %which revealed the failure to ``Blue Team'' 
    \\ \hline
Proxy/Mon (Fig.~\ref{fig:proxy_monitoring_policy}); $S_1$-$S_2$ link is down &  Non-cached rqst from inside the Dept, followed by request for the same object from by another source host in the Dept\\ \hline
Proxy/Mon (Fig.~\ref{fig:proxy_monitoring_policy}); The port of $S_1$ (Pica8)  connected to proxy is (mis)configured to not support OpenFlow & HTTP rqst from Dept	\\ \hline
 Cascaded NATs  (Fig.~\ref{fig:cascaded_nats}); {\tt FlowTags} controller  shut down &  $H_1$ attempts to access to the server \\ \hline
%Multi-stage trigger (Fig.~\ref{fig:dynamic_policy});  L-IPS  misconfigured to alarm after  5 conns \& Host $H_1$ makes 9 scan attempts. \\ \hline
 Multi-stage triggers (Fig.~\ref{fig:dynamic_policy}); L-IPS miscounts by summing three hosts  & $H_1$ makes 9  scan attempts followed by 9 scans by $H_2$  \\ \hline
Conn. limit.; Login counter resets  &  $H_1$ makes 3 continuous log in attempts with a wrong password   \\ \hline
Conn. limit.; $S_1$ missing switch forwarding rules from AuthServer to the protected server  & $H_2$ makes a log in attempt with the correct password
\end{tabular}
\end{center}
\end{footnotesize}
%\vspace{-0.3cm}
\tightcaption{Some example red-blue team scenarios.}
\label{tab:bug_scenarios}
%\vspace{-0.3cm}
\end{table}

%\vyas{check the table carefully!!}

 
Table~\ref{tab:bug_scenarios} highlights the results for a subset of
these scenarios and also shows the specific traces that \Name 
generated.  Three of the scenarios use the motivating examples
from \Section\ref{sec:motivation}. In the last scenario
(Conn. limit.), two hosts are connected to a server through an
authentication server to prevent brute-force password guessing
attacks. The authentication server is expected to halt a host's access
after 3 consecutive failed log in attempts.  In all scenarios the
blue-team successfully localized the failure (i.e., which \DPF,
switch, or link is the root cause) within 10 seconds. Note that these
bugs could not be exposed with existing debugging tools such as
ATPG~\cite{atpg}, ping, or traceroute.\footnote{They can detect
  obvious failure modes such a link/switch being down but cannot
  capture subtle bugs w.r.t.\ stateful/contextual behaviors.}
 


%\vyas{were the last two scenarios not discovered?}

%\vyas{can we say why existing techniques would have failed here?}

%\vyas{can we say how long it took to do this end to end?}

%\vyas{are we modifying the policy/assertion for each scenario to be different? need some more details here}
%\seyed{this should go to implementation?}

\seyed{commented out flowtags real bug para for now...}
\comment{
\myparatight{Finding real bugs} \Name also helped us identify an
actual bug in our {\tt FlowTags} re-implementation in
OpenDaylight.\footnote{Our original implementation was in {\tt POX};
  the bug arose during the (non-trivial) process of porting it to
  OpenDaylight; OpenDaylight is a significant codebase with a lot of
  complexity.} Essentially, the controller code in charge of decoding
{\tt FlowTags} (e.g., to distinguish sources hidden behind a NAT or
proxy) was assigning the same tag value to traffic from different
sources.  By using test traffic in network of
Figure~\ref{fig:proxy_monitoring_policy}, we observed that proxy hit replies
bypass the monitoring device, which is a violation of the intended
behaviors. \Name validation also localized the policy violation (i.e.,
at the proxy).  It also provided the traffic trace indicating that the
tag values of cache miss and hit cases are identical, that gave us a
hint to focus on the proxy tag assignment code of {\tt FlowTags}
controller.
}

%\vyas{this is too close to row 2 in the table?}\seyed{we have done one more scenario 
%with pica8 not supporting openflow on a certain port. maybe use than one instead of row
%2 of table?}

%effecting the violation helped us identify  the buggy behavior
% in the {\tt FlowTags} controller module. Specifically, the test trace 
%\vyas{how did we diagnose that it was a controller bug?}

\comment
{
%------------------------------------------------------------------------------------%
\subsection{Other use cases}%\seyed{must be shortened and maybe cite tech report for longer versions?}
\label{sec:eval_other}

\seyed{dropped para on ``Testing  {\tt Flowtags}-enhanced \DPFs''}
\comment{ 
\myparatight{Testing  {\tt Flowtags}-enhanced \DPFs} One of the  original
 motivations for \Name  was that  existing tools 
 were inadequate to test our {\tt FlowTags} implementation~\cite{flowtags_nsdilong}.  To this
end, we define intended behaviors for single \DPFs and exhaustively test
externally observable middlebox actions; e.g., the  tagging
behavior of the IPS to ensure it tags according to the intended alarm thresholds.
}
% We believe that the ideas in \Name may be  independently 
% helpful for testing individual middlebox implementations. 

\myparatight{Incremental Testing}:   One natural question is if  we can
incrementally test the network when policies partially change. While a full
discussion is outside the scope of this work, we have early evidence to show
that \Name is amenable to incremental testing.  The intuition here is if only a
suffix of policy chain changes, we do not need to generation traffic from 
scratch; instead we can augment existing test scripts to explore the newly
added behavior. For examples, if we decide to add a firewall after the proxy
and monitor in Figure~\ref{fig:proxy_monitoring_policy}, new test scripts can
be incrementally obtained based on existing traces that already explore the
existing two policy terminal branches in the figure.

\myparatight{Loops and reachability} While reachability checking in stateless
data planes is a ``solved'' problem~\cite{hsa}, it is unclear if this is true
for stateful data planes. %To this end, We  extend 
\Name supports reachability properties via new types of assertions. For instance, 
to detect loops we add  assertions of the form: {\tt assert(seen[ADU.id][port]<K)}, 
where {\tt ADU} is symbolic \PADU, {\tt port} is a switch port, and {\tt K} reflects
a simplified definition of a loop that  the same \PADU is observed at the same
port $\geq$ {\tt K} times. Similarly, to check if some traffic  can reach  {\tt PortB} 
from {\tt PortA} in the network, we initialize a \PADU with the port field  to be 
{\tt PortA} and use an assertion of the form {\tt assert(\PADU.port != PortB)}. 
Using this technique we were able to detect synthetically induced switch 
forwarding loops an stateful data planes (not shown).
}

% and traffic violating teachability policies. 

% \seyed{ack that existing
%work can do this too but this is just an extra feature of our system covering
%stuff beyond service chaining}




==> formulation_old.tex <==
\section{Problem Formulation}
\label{sec:formulation}

\newtheorem{definition}{Definition}
\newcommand{\set}[1]{\{{#1}\}}
\newcommand{\seq}[1]{\langle{#1}\rangle}
\newcommand{\such}{\centerdot}
\newcommand{\ipaddr}{\mathsf{IPAddr}}
\newcommand{\ports}{\mathsf{Port}}
\newcommand{\prots}{\mathsf{Proto}}
\newcommand{\packet}{\mathcal{\pi}}
\newcommand{\packets}{\mathcal{P}}
\newcommand{\alp}{\Sigma}
\newcommand{\ip}{ip}
\newcommand{\port}{port}
\newcommand{\prot}{proto}
\newcommand{\action}{action\xspace}
\newcommand{\actions}{actions\xspace}
\newcommand{\Actions}{Actions\xspace}

%The previous section shed light on the types of  high-level contextual policies
%involving stateful \DPFs that we want to test.  
  
In this section, we begin by  formally defining  the problem that we want to
solve before going into the technical ideas underlying \Name.  This formalism
serves three key roles. First, it helps us precisely define the policies and
goals for the high-level examples from the previous section. Second, it sheds
light on  the key technical components that any solution to this
problem needs to address.  Finally, it will highlight the challenges
 in realizing in practical and the practical relaxations 
 we make in designing \Name.  

\subsection{Preliminaries}


%Let $\ipaddr$ be the set of all IP
%addresses, $\ports$ be the set of  all transport-layer ports and $\prots$ be
%the set of protocols (e.g., TCP, UDP). A packet is a 5-tuple $(\ip_{src},
%\port_{src}, \ip_{dst}, \port_{dst}, \prot)$ such that: (i) $\ip_{src},
%\ip_{dst} \in \ipaddr$; (ii) $\port_{src}, \port_{dst} \in \ports$; and (iii)
%$\prot \in \prots$. 


%\seyed{two things: 1) do we need restrict the def. to the 5-tuple part of
%packets? or we should say can say a packet is a n-bit string?, 2) do we need to
%define the located packet here too, as we use it in the next section?}
%Let $\alp$ be a denumerable set of \actions. \Actions denote the
%response of a DPF to a packet, e.g., $\mathsf{ok}$, $\mathsf{alarm}$,
%etc. %Informally, 

As seen in the previous section, a  \DPF can be viewed as a  ``stateful packet transformers''  that repeatedly 
accepts packets, modifies them, and redirects them to one of its output 
 ports. If $\packets$ denotes the set of IP packets, then we can
 formally define a \DPF as:

%\footnote{\seyed{this is my interpretation of a channel... can be incorrect} 
%A channel here represents a \DPF's physical interface
%to the network (e.g., an Ethernet port).} based on its current state, and 
%updates its state. More formally, 
% We now define it formally.
%\seyed{how about calling them response instead of \action?}

%---------------------------------------------------------------------%
\begin{definition}[DPF]
 A \DPF is a 4-tuple $(S, I, O, \delta)$ where: (i) $S$ is a
finite set of states; (ii) $I \in S$ is the initial state; (iii) $O$
is the set of output channels; and (iv) $\delta : S \times \packets
\mapsto S \times \packets \times O \times \alp$ is the transition
relation. Here,  $\alp$ is a finite set of \actions that  denote the
 response of a DPF to a packet, e.g., $\mathsf{ok}$, $\mathsf{alarm}$. 

\end{definition}

That is,  if $\delta(s, \packet) = (s', \packet', o, \alpha)$
then this means that if the \DPF receives packet $\packet$ when it is in
state $s$, then: (i) it constructs a packet $\packet'$ (note that $\packets'$
could be the same as $\packet$ in case the input packet is transmitted
unmodified); (ii) sends out $\packet'$ over output port $o$; (iii)
updates its state to $s'$; and (iv) emits \action $\alpha$.

Note that this definition of a \DPF is quite general and it encompasses both
stateful \DPFs that we saw in the previous section as well as simpler L2-L3
devices that are stateless.

\seyed{maybe we need to add input port l too, so it becomes:
$\delta : S \times \packets \times InChannels \mapsto S \times \packets \times O \times \alp$
}
\newcommand{\nodes}{\mathcal{N}}
\newcommand{\topo}{\tau}
\newcommand{\netw}{\eta}
\newcommand{\nstate}{\mathcal{S}}

%---------------------------------------------------------------------%
\mypara{Network} A network is simply a collection of \DPFs and a topology
defining the interconnections between the \DPFs. Formally, it is a pair
$(\nodes, \topo)$ such that: (i) $\nodes = \set { \DPF_1, \dots, \DPF_k}$ is
a set of \DPFs with $\DPF_i = (S_i, I_i, O_i, \delta_i)$; and (ii) $\tau :
\bigcup_{i=1}^k O_i \mapsto \set{ \DPF_1, \dots, \DPF_k }$ is a topology
that maps each output port to a \DPF. Informally, if $\tau(o) = \DPF$
then any packet sent out on channel $o$ is received by  $\DPF$.
\seyed{this is assuming each \DPF has one single input channel. we can
naturally generalize it.}

%A network naturally induces a directed graph and whose nodes
%correspond to \DPFs and whose edges correspond to the topology. 
 We assume that the graph has  some well-defined sources (with no incoming
edges), and one more sinks (with no outgoing edges).

%\seyed{how to model end nodes, i.e., hosts/servers that are end points of
%traffic? are we assuming they are all abstracts behind these virtual 
%source and sink nodes? i think we need a formalization of end nodes 
%to which we can refer in the traffic generation section too.}

%---------------------------------------------------------------------%
\mypara{Packet traversal} A packet introduced at a source 
flows through the edges of the network and stops at a sink. In the
process, it causes each \DPF that it passes through to emit an \action
and update its state according to its transition relation. 

%Each packet causes two types of transitions in a network's state: (i) {\em per-hop} 
%  transition (labeled by an \action) denoting the movement
%of a packet from one \DPF to the next; (ii) a {\em multi-hop}  transition
% composed of a sequence of per-hop  transitions (and therefore
%labeled by a sequence of \actions) denoting the movement of the packet
%through the network from the source \DPF to a sink \DPF.

% We now define these state transitions formally.

Let $\netw = (\nodes, \topo)$ be a network such that $\nodes = \set {
  \DPF_1, \dots, \DPF_k}$ with $\DPF_i = (S_i, I_i, O_i, \delta_i)$. A state of
$\netw$ is a tuple $(s_1, \dots, s_k)$; i.e., 
% such that $\forall 1 \leq i
%\leq k \such s_i \in S_i$. Informally, this means that
 each \DPF $N_i$
is in state $s_i$. Thus, the set of all states of $\netw$,
denoted $\nstate (\netw)$, is $S_1 \times \dots \times S_k$.

\newcommand{\sstep}[3]{{#1}\stackrel{#2}{\longrightarrow}{#3}}
\newcommand{\lstep}{\mathcal{R}}

%---------------------------------------------------------------------%
%\emph{Small Step Transition.}
%
We first define a {\em per-hop} state transition on this network.
Let $\sigma = (s_1, \dots, s_k)$ and $\sigma' = (s'_1, \dots, s'_k)$
be two network states, $j, j' \in \set{1, \dots, k}$ be two \DPF
indices, and $\packet$ and $\packet'$ be two packets. We say that there is a
small-step transition from $(\sigma, j, \packet)$ to $(\sigma', j', \packet')$
labeled by \action $\alpha$, denoted $\sstep {(\sigma, j, \packet)}
{\alpha} {(\sigma', j', \packet')}$ if the following two conditions hold:
%
\begin{eqnarray*}
&\exists o \in O_j \such \delta_j (s_j, \packet) = (s'_j, \packet', o, \alpha)
  \land N_{j'} = \topo(o) \\
%
&\forall 1 \leq i \leq k \such i \neq j \Rightarrow s'_i = s_i
\end{eqnarray*}

That is $N_j$ processes the packet $\packet$,
moves from state $s_j$ to $s'_j$, transforming $\packet$ to $\packet'$, and
emitting \action $\alpha$. The new packet $\packet'$ moves to \DPF
$N_{j'}$.  All other \DPFs remain in the same state.

%---------------------------------------------------------------------%
%\emph{Large Step Transition.}


An {\em end-to-end} state transition then is a relation $\lstep
(\netw) \subseteq \nstate(\netw) \times \packets \times \alp^+ \times
\nstate(\netw)$ such that $(\sigma, \packet, \seq{\alpha_1, \dots,
  \alpha_n}, \sigma') \in \lstep (\netw)$ iff there exists a sequence
of DPF indices $j_0, j_1, \dots, j_n$, a sequence of packets $\packet_0,
\packet_1, \dots, \packet_n$, and a sequence of network states $\sigma_0,
\sigma_1, \dots, \sigma_n$ such that: (i) $N_{j_0}$ is a source DPF;
(ii) $N_{j_n}$ is a sink DPF; and (iii) the following holds:
%
\begin{eqnarray*}
&\packet = \packet_0 \land \sigma = \sigma_0 \land \sigma' = \sigma_n
  \\ &\forall 1 \leq i \leq n \such \sstep {(\sigma_{i-1}, j_{i-1},
    \packet_{i-1})} {\alpha_i} {(\sigma_i, j_i, \packet_i)}
\end{eqnarray*}

Thus, the insertion of packet $\packet$ when the network is in state
$\sigma$ causes the sequence of \actions $\seq{\alpha_1, \dots,
  \alpha_n}$ to be emitted and the network to move to state $\sigma'$.

\newcommand{\aseq}{\vec{\alpha}}
\newcommand{\sem}[1]{[\![{#1}]\!]}

%---------------------------------------------------------------------%

\mypara{Network Policies}
%
The end-to-end state transition leads naturally to the notion of a network's
semantics.
% This semantics is defined in terms of network traces, which
%we present first.

%\emph{Trace.}
%
A network trace (or trace for short) is a sequence $\packet_1, \aseq_1,
\dots, \packet_n, \aseq_n$ of alternating packets and \action sequences
(i.e., $\forall 1 \leq i \leq n \such \packet_i \in \packets \land \aseq_i
\in \alp^+$).

%---------------------------------------------------------------------%
%\%emph{Network Semantics.}
%
%The semantics of network $\netw$, denoted $\sem{\netw}$, is the set of
%traces defined as follows. 

A trace $\packet_1, \aseq_1, \dots, \packet_n,
\aseq_n$ belongs to $\sem{\netw}$ iff there is a sequence of network
states $\sigma_0, \dots, \sigma_n$ such that $\sigma_0 = (I_1, \dots,
I_k)$ and $\forall 1 \leq i \leq n \such (\sigma_{i-1}, \packet_i,
\aseq_i, \sigma_i) \in \lstep (\netw)$. In other words, $\sigma_0$ is
the initial state of the network, and each successive state $\sigma_i$
is obtained by a large step transition using the corresponding packet
$\packet_i$ and witnessed by the \action sequence $\aseq_i$.

%---------------------------------------------------------------------%
%\emph{Network Policy.}
%

A {\em network policy} is specified by a set of traces. However, while
a network semantics represents the \emph{actual} behavior of a
network, and is defined \emph{implicitly} via the network, a network
policy is specified \emph{explicitly} and represents the
\emph{desired} behavior of the network.

\newcommand{\npol}{\varphi}

%---------------------------------------------------------------------%
\subsection{Problem Definition}
%
Given these preliminaries, we can now formally define the  objective of  \Name. 
%It
%consists of the following steps. First, we construct a model of the
%network $\netw$. Next, we specify a network policy $\npol$. We then
use symbolic analysis to construct a trace $t \in \sem{\netw} \cap
\npol$. In other words $t$ is a behavior of the network model that
also respects the policy. From our point of view $t$ becomes a ``test
traffic'' for the actual network. Let $t = \seq{ \packet_1, \aseq_1,
  \dots, \packet_n, \aseq_n}$. We then execute $t$ on the actual network
by inserting the packets $\packet_1, \dots, \packet_n$ in sequence into the
source DPF. We wait for packet $\packet_{i-1}$ to reach a sink DPF before
inserting $\packet_i$. We monitor the network to construct the trace
$\widehat{t}$ exhibited by the real network. If $t = \widehat{t}$ we
declare the test $t$ to be successful. Otherwise, $t$ is a failure and
we provide $t$ and $t'$ as diagnostic feedback to the
administrator. We repeat this step for several different test traffics
to improve the coverage of FlowTest. In the rest of the paper, we
present these steps in more detail, along with experimental results.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% old stuff -- commented out
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Before we can test a data plane, there should be a clear way of
%% defining intended policies. As we saw in the examples of
%% \S\ref{sec:motivation}, intended policies can be contextual, which
%% means intended traffic processing may depend on \DPF states w.r.t. the
%% traffic (e.g., Figure~\ref{fig:dynamic_policy}). Networks operator
%% should be able to specify such policies. To this end, we build on the
%% notion of dynamic policy graphs (DPGs)~\cite{flowtags_nsdilong}, and
%% propose the \emph{Contextual Policy Specification} (\policy).

%% \mypara{Definition} A \policy represents the intended policies of a
%% network with the following Backus-Naur Form (BNF):\\

%% \noindent $policy::=policyLine<EOL>policy \;|\; policyLine$ \hfill (1)

%% \noindent $policyLine::=\{guard\}: DPFset\;fate$ \hfill (2)

%% \noindent $guard::=(5tuple) guard \;|\; (5tuple) $ \hfill (3)

%% \noindent $5tuple::=(srcIP, dstIP, proto, srcPort, dstPort)$ \hfill (4)

%% \noindent $DPFset::=(\DPF,state).DPFset \;|\; \epsilon$ \hfill (5)

%% \noindent $\DPF::=firewall \;|\; proxy \;|\; nat \;|\; IPS \;|\; IDS \;|\; \dots$ \hfill (6)

%% \noindent $state::=ok \;|\; alarm \;|\; hit \;|\; miss \;|\; count \;|\; \epsilon \;|\; \dots$ \hfill (7)

%% \noindent $fate::=dst \;|\; terminate()$ \hfill (8) \\

%% A \policy is a set of policies (1) that represents intended traffic
%% processing of the data planes. In each line, it specifies how traffic
%% whose 5-tuple values satisfies the line's guard (3, 4) should go
%% through a sequence of \DPFs and under what \emph{state}(2). In
%% particular, $state$ is a postcondition of \DPF after processing
%% traffic (5). Rules (6) and (7) show some example \DPFs and their
%% states. The last element of a policy line indicates the intended fate
%% of the traffic, which is either delivery to a destination (as
%% specified by the destination part of the guard) or getting terminated
%% (e.g., malicious traffic)(8). The symbol $\epsilon$ denotes an empty
%% string.  For brevity, we do not show the derivation rules for obvious
%% symbols such as IP addresses.
 
%% A guard in general is a non-empty set of traffic 5-tuple values
%% (source IP, destination IP, protocol, source Port, destination
%% port). All traffic whose 5-tuple match a guard must be processed
%% according to the corresponding policy line. States are \DPF-dependent
%% (e.g., hit/miss states for a proxy) and represent the state of the
%% particular \DPF \emph{after} processing traffic.  Traffic may be
%% delivered to a destination or be dropped as part of the intended
%% policy. Function $terminate()$ represents the latter behavior, which
%% is traffic dependent (e.g., dropping a packet on a stateless packet
%% filter, or sending a \texttt{RST} in a TCP connection).  By contract,
%% if traffic does not match any guards of the \policy, it should be
%% blocked.\footnote{On the contrary, we may want to choose to make this
%%   default policy behavior completely permissive and do not expose the
%%   unspecified traffic to any \DPF processing.}

%% \mypara{Example} The intended policy of the example of
%% Figure~\ref{fig:dynamic_policy} is expressed as the following
%% \policy. $Int.$ shows the gateway router of the enterprise
%% network. $lIPS$ and $hIPS$ represent the light and heavy IPS. For ease
%% of presentation here the guards only show source and destination
%% entities and ${\bf H}=\{(H_1)(H_2)(H_3)\}$:\\

%% \noindent $\{{\bf H}\; to\; Int.\}: (lIPS,ok).dst\\$
%% \noindent $\{{\bf H} \; to\; Int.\}: (lIPS,alarm).(hIPS,ok).dst\\$
%% \noindent $\{{\bf H} \; to\; Int.\}: (lIPS,alarm).(hIPS,alarm).terminate()\\$
%% \noindent $\{Int.\; to\; {\bf H}\}:dst\\$

%% The first three lines of this example \policy show policies for
%% traffic going from hosts to the internet. The last line shows the
%% policy path for the response traffic from the Internet---in this case
%% a simple reachability policy with stateful processing.

%% \mypara{Policy equivalence classes} Flows that math the same guard
%% belong to the same \emph{policy equivalence class}. (We will use this
%% definition in the following sections.) In the above example, flows (in
%% the sense of the IP 5-tuple) from $H_1$, $H_2$, and $H_3$ belong to
%% the same policy equivalence class.

%% \mypara{\policy correctness} Since a \policy is a specification of the
%% intended policies, it is important to make sure this specification
%% ``makes sense" before proceeding to the test activity. To this end
%% \Name parses a given \policy to ensure each possible flow does not
%% match more than one guard. Further, states specified for each \DPF in
%% form of $(\DPF,state)$ should be relevant to that \DPF.

%% \mypara{Test goal} The goal of \Name is to test the data plane to
%% ensure actual traffic is processed as specified by the \policy (e.g.,
%% traffic from host $H_1$ that triggers an alarm at the light IPS but
%% not at the heavy IPS can reach the internet).

%% \mypara{\policy in practice} We end this section with three practical
%% considerations regarding \policy. First, \DPFs appearing in a \policy
%% merely represent the functionality of that \DPF type (e.g., a
%% proxy)---how this \DPF is realized in the actual data plane depends on
%% the actual implementation, and \Name does not make any assumptions
%% about this. Second, a \policy is agnostic to physical interconnections
%% of \DPFs by switches. For example, if $\DPF_2$ appears after $\DPF_1$
%% in a policy line, the instances of these \DPFs may be connect through
%% the shortest path in the physical network. Finally, a \policy can
%% change over time (we revisit this in \S\ref{sec:eval}). This can be
%% either because of explicit change of policies by the operator, or
%% based on pre-defined events in the network (e.g., launching more
%% firewall instances when traffic volume increases).

%% \mypara{\seyed{section to do}}

%% \begin{packeditemize}

%% \item while not making a huge deal about \policy, we should say why
%%   not existing policy notations? why something new.

%% \item give some intuition on where \policy is coming from?
%%   handwritten? extracted from higher level policy descriptions?

%% \end{packeditemize}

%%- the formalization section will be based on actual dpfs dealing with real (low level) packets.


%%- in the modeling section, we say it is not practical to model dpfs based on how we formalized before because: 

%%1) the models become too complex (the code itself in the extreme). the other extreme is to consider very high level models (http as the unit of proxy), but this is not composable. so we do abstract data units. 

%%2) it's not practical to proactively generate traffic at the packet level (e.g., we dont know what TCP seq number will be used by the OS).


%%- the other modeling idea to is to have an ensemble of dpfs as opposed to one giant fsm (we can give the example of a proxy which is three logically independent fsms for client-side tcp, server-side tcp, and cache)

%%- somewhere we should say even though possible states in real world are infinite, we are doing fsms because that's good enough to capture polices (b/c policies are finite, e.g., we don't have distinct intended policies for all existing websites in the universe)


%%- finally in the modeling section we should talk about the fact that state transitions in models should reflect the granularity of intended policies. e.g., if we have policies for hit/miss responses, modeling http get fragmentation would be overkill.

%% 


==> intro_old.tex <==
\section{Introduction}
\label{sec:intro}

%\begin{itemize}

%\item p1: ensuring networks behave correctly is hard .. ppl spend a lot of effort
Many previous studies have shown that it is difficult to ensure that the
network configuration meets the  policy goals that operators intended to
enforce. For instance, one recent survey found 35\% of networks  generate more
than 100 problem tickets per month and nearly one-fourth of these problem
tickets take multiple engineer-hours to resolve~\cite{atpg-survey}.  Anecdotal
evidence suggests network administrators go to great lengths to test and debug
their networks; e.g., creating ``shadow'' configurations of entire
infrastructures purely for testing~\cite{attpc}. \vyas{find more interesting
citations/anecdotes here} 

%ets per month. 40.4% of respondents estimate that one
%engineer needs less than 30 minutes to solve one such
%ticket. But 24.6% of res
% that XXX\% of operators spend    
 


%\item p2: success of sdn has inspired several recent works on verification, 
% programming correctness, testing etc -- 
%In this context, the success of software-defined networking (SDN) has
%rejuvenated the areas of  network testing and verification, with an ultimate
%vision of developing  ``CAD tools for networks''~\cite{nickmtalk}.  

Recognizing this challenge, there are a range of concurrent in this space
including work on statically checking reachability and isolation
policies~\cite{hsa,veriflow,netplumber}, formal foundations of network
controller and data plane design~\cite{frenetic,netkat}, creating
correct-by-construction controller platforms~\cite{vericon}. \vyas{cite more
and cover the space} To date, however,  these efforts have largely focused on
forwarding-centric properties; e.g., ensuring who-can-talk-to-whom or if there
are potential loops or checking if the network can violate isolation properties
across tenants~\cite{}. 


While rechability  properties are critical  
 and necessary to validate, we observe that real network settings 
 are more complex on two key dimensions:
\begin{packeditemize}


%In addition to
%traditional L2/L3 network functions such as switches and routers,

\item {\bf Stateful and higher-layer network functions:}  Networks rely on a
wide spectrum of network appliances or middleboxes such as proxies, stateful
firewalls, NATs, intrusion prevention systems (IPSes), load balancers, WAN
optimizers~\cite{}.  There are two key distinguishing features of Such advanced
network functions, which we collectively refer to as {\em \DPFs}, typically
operate at a higher-layer beyond L2/L3  and they are {\em stateful} in that
their actions are dependent on the history of the traffic they have processed.
For instance, a web proxy operates atop HTTP  and may directly respond with
cached responses. 

%while load
%b%alancers may also be application-aware~\cite{ananta}. Second, and more
%importantly, they  are {\em stateful} functions that keep per-flow,
%per-session, and cross-session states that  depend on  the   history of traffic
%traversing them. Thus, their  actions  crucially depend on the current state.
%F%or instance, (1)  a proxy may directly respond with cached static objects; (2)
%a% NAT tracks the set of  public IPs and ports in use when assigning new
%connection mappings; (3) a load balancer will maintain flow affinity; and (4)
%stateful firewalls will allow incoming traffic only for previously observed
%outgoing connections.

\item {\bf Context-dependent policies:}  Operators use such \DPFs, to implement
contextual policies beyond simple forwarding and access control logics.   The
simplest contextual policy is {\em service chaining} to compose \DPFs; e.g.,
ensuring that HTTP traffic  goes through a {\em sequence} of a firewall, IPS,
and proxy  before exiting the network boundary. Other types of contextual
policies may involve event ``triggers''; e.g., a host generating too many
failed connections may be  flagged for anomalous   behavior     and
subsequently subject to more detailed analysis~\cite{pyresonance,slick}.

\end{packeditemize}

  

%\item p3: focus mostly on the forwarding layer2/layer3 centric aspects. real 
% networks are more complex on two dimenions 
%	\begin{itemize}
%	\item stateful network functions
%	\item complex contextual policies
%	\end{itemize} 

%\item 

 In conjunction, stateful \DPFs and the attendant contextual policies used in
their configurations, introduce new types of requirements that fall outside the
scope of existing network verification and testing tools. 
%Many of these efforts
%explicitly acknowledge this limitation and their inability to handle such
%scenarios~\cite{}. 
Our goal is to address this key missing piece
to take us closer to realizing the CAD-for-networks vision~\cite{}.  

%Ideally,
%we would like to {\em verify} mechanisms that can guarantee that the network
%with such stateful \DPFs implements the desired contextual policy.
%Unfortunately,  many of the \DPFs involve proprietary code  and hidden actions,
%which may make it difficult to systematically verify a network with such
%``black boxes''.  Moreover, 
Given the dynamic nature of real networks and the
traffic-dependent processing that the \DPFs entail, we believe that 
 % viable
%t%o statically verify that the network always implements the policy. 
%To this end, we take a pragmatic  stance  and take an alternative 
 a {\em model-based  testing} approach is more suitable relative 
 to other static checking techniques.  That is, given an abstract network model of
different \DPFs and their interconnections   and the intended policy, our goal
is to systematically  generate {\em live test traffic} to test the network to
 check if it meets the intended policies. 
%There are two key points to note here.
%First,  given the stateful and contextual nature of the \DPFs and the policies,
%what we need is in effect is a multi-step test plan to generate a traffic trace
%rather than a single packet, which sufficed for simple reachability
%testing~\cite{}.  Second, our test cases are intended to test the policy
%semantics and not aimed at more traditional security penetration testing or
%scalability testing~\cite{}. 
%also emphasize pro activeness as opposed to diagnosis etc.
%believe testing a
%model specification might be a more pragmatic first step 
%to be practical we
%need mechanisms to capture these richer semantics. given the complex behaviors,
%statically verifying abstract models isnt  sufficient so we believe testing a
%model specification might be a more pragmatic first step 


However, there are key challenges in every step in realizing this approach: 
\begin{packeditemize}

\item {\em Modeling:}  We need practical {\em high-fidelity}  models (to capture 
 key semantics) of individual \DPFs  that are  {\em composable} (to reuse 
 the models across policy scenarios). 
% Model fidelity is essential to
%capture the key intricacies of the \DPFs and  composability is essential to
%reuse \DPF models across different policies. 
 The challenge here is that \DPFs are complex and diverse. At one extreme, we can consider using the raw
binary/code of the \DPF; this is composable but may result in an intractable
model. At the other end, we can envision highly simplified models (e.g., a
proxy has two states of cache or not-cached) but this  may not be immediately
composable or provide the desired fidelity. 

\item {\em Test generation:} Even if we address the above modeling challenge,
we run into classical state-space explosion problems when we want to use the
models to generate test cases.  For instance,  \plsfill

\item {\em Diagnosis:} Finally, given our goal of live testing, we need
to ensure that the test results can be suitably validated. For instance, we
need to rule out side effects from background traffic that could have caused
false positives or false negatives when the test succeeds or fails. 
 Finally, we also need mechanisms for initial root-causing to help 
 focus the administrators diagnostic efforts.

\end{packeditemize} 

%p6: what makes this hard 
%	\begin{itemize}
%	\item  capture diversity of the network data plane 
%	\item  need to balance model fidelity and tractability
%	\item  state space explosion
%	\item  interference/validation
%	\end{itemize}

In this paper, we present the design and implementation of \Name, a framework
that makes  three key contributions to address these challenges:
\begin{packeditemize}
\item  To address the modeling  challenge, we introduce the {\em \PADU} abstraction
extending existing located packet abstractions that serves as unifying lowest
common denominator across diverse \DPFs.  We also use the insight that most
\DPF behaviors can be captured  via a suitable {\em \fsmensemble} abstraction
building on the familiar notion of finite-state machines (FSM).

\item  We use {\em symbolic execution} using the abstract data plane 
 model to  obtain a high-level test plan in terms of the sequence of \PADUs 
 that need to be generated. While symbolic execution by itself 
 is not immune to state-space explosion, it allows us 
 to engineer domain-specific insights to make it tractable. \vyas{too fluffy}    

%representative traffic
%from each equivalent class of traffic (i.e., traffic that will be processed the
%same way by the data plane). The intuition here is to use this test traffic to
%systematically explore the state space of the data plane w.r.t. intended
%network-wide policies. Symbolic execution, in general, suffers from state
%explosion. Thus, to plan test traffic efficiently while meeting test
%requirements (e.g., coverage), we identify and use  insights on the behavior of
%the specific network data plane under test  (e.g., characteristics of the
%network topology) as well as the given policies and test goals.

\item  Finally, we leverage new SDN capabilities for extensible data plane
monitoring   to identify potentially interfering traffic and to rule out
interference.   We also extend our test trace generation to produce partial
prefixes to help the diagnosis of potential policy violations.
  
 
\end{packeditemize}

% {  we make two key observations   
 
  
%p7: we design flowtest to address these challenges.  to capture
% diversity we extend located packet abstraction to capture 
% diff protocol layers. to balance model fidelity we do foo. to 
% tackle state space explosion we do blah. for interference, we rely 
% on xxx. 

 We have implemented models for various \DPFs as simple \fsmensembles   written
in {\tt C}. In light of several recent domain-specific languages that extend PL
techniques to networking~\cite{},   the choice of C may seem odd at first.  We
believe that  this is actually a  more pragmatic choice that helps us leverage
a rich body of tools that are explicitly targeted at C such as {\tt KLEE}. We
extend {\tt KLEE} with several domain-specific heuristics outlined above. We
use a custom traffic translation layer that generates ``raw'' request traces
from the \PADUs specified by {\tt KLEE}.  We evaluate \Name using a combination
of large-scale simulations and a real testbed evaluation. We find that \plsfill.
  

%p8: say something abt results, eval interestingness


%\end{itemize}

\comment
{
\begin{packeditemize}

\item Network data planes are complex systems composed of numerous
heterogeneous elements. This complexity gives rise to many potential violations
of intended network policies caused by various reasons: a mis-configured
switch,  buggy firewall code, a mis-configured proxy, to name a few. In
practice, network operators spend a lot of time dealing with consequences of
policy violations  when they arise. \seyed{citations or anecdote on how much
time admins spend testing the network.}

\item To ensure successful enforcement of network policies and avoid costly
future policy violations, it is important to proactively test the network as
close to the wire as possible (i.e., the data plane), where packets are
processed. This involves testing the network data plane in a live manner by
injecting test traffic into it and validating the observed behavior of the
network. The rationale here is to use test traffic to infer how the network
\emph{would} behave given production traffic, and find and fix problems
proactively.

\item Today's realistic network testing scenarios, unfortunately, fall outside
the purvey of the existing solutions in that both policy requirements and data
plane elements are complex: \emph{(1) contextual policies}: service chaining
policies~\cite{ietfnsc} are by structure contextual (e.g., send traffic to the
heavy IPS only if it has triggered an alarm on the light IPS), \emph{(2)
stateful data plane behavior}: many data plane elements  that are widely used
expose stateful behavior (e.g., stateful firewall, providing a cached response
by a proxy)\footnote{We refer to  data plane elements other than
switches/routers as data plane functions (\DPFs).}. \seyed{get rid of the term
dynamic as  stateful kinda of capture it} 

\item \seyed{need a para here to say what is challenging and why existing work
is inadequate}

\item We have developed \Name to test realistic data planes. At a high level,
\Name is a framework to systematically test a data plane versus intended
policies via test traffic.  Given a set of network-wide policies, first, \Name
models the data plane as a finite state machine to facilitate formulating the
test goals and make the test process intuitive.  Then \Name generates test
traffic that is  carefully chosen as to efficiently explore the ``state space''
of data plane. Finally, \Name monitors network-wide behavior in response to
test traffic and validates it versus the policies. We believe \Name is a timely
step forward in the broader domain of correct network policy management and CAD
for networks, as an active area of research \seyed{cite sigcomm 12 and 14
keynotes}.


\item In this paper, we make three contributions toward addressing these challenges:

\begin{packeditemize}

\item \mypara{Modeling stateful data planes} We model individual data plane
elements (e.g., firewalls, proxies) with the goal of representing
specifications/requirements of \DPFs as viewed by network operators (e.g., a
stateful firewall is expected to disallow unsolicited inbound TCP initiation).
Inherent diversity of \emph{operations} (e.g., caching operations by a proxy,
stateful traffic processing by a firewall) as well as \emph{semantics level}
(e.g., processing traffic at IP, transport, or application layer) of various
\DPFs make modeling data planes challenging. We have modeled a range of
representative \DPFs (e.g., firewalls, packet filters, proxies) based on their
specifications such that they can be composed with one another as well as
switches to yield a model of the entire data plane in form of a finite state
machine (FSM).  The key enabler in doing so is to specify each model w.r.t. to
its behavior in processing \locPkts\footnote{\seyed{maybe too much detail for
intro?}A \locPkt is a packet along with its location (i.e., port) in the data
plane\cite{hsa, consistentupdate}. While prior work has used the \locPkt
abstraction to model stateless data planes (i.e., only composed of switches),
we go beyond this by modeling stateful data planes as \locPkt processors.} in
form of a finite state-machine.  In generating the model of the data plane for
a specific data plane, we account for the intended policies (e.g., an IPS in
general has many capabilities, but we may solely use it as a counting IPS in a
particular network). This specialized data plane model is used to plan test
traffic.\footnote{As an aside, the model that is in form of a FSM is a visual
representation of network data plane and intended policies, which is intuitive
for the human operator to grasp.} \seyed{we have done generic modeling (e.g.,
template model of a firewall, ips). for a give problem (i.e., a specific
topology and set of intended policies), these generic models get specialized
and composed to yield the model of the data plane. THIS SHOULD COME ACROSS}

\item \mypara{Planning test traffic} Given the data plane model, we identify
and implement a ``network test planner". To this end, we use symbolic execution
on the model of the data plane as a mechanism to obtain representative traffic
from each equivalent class of traffic (i.e., traffic that will be processed the
same way by the data plane). The intuition here is to use this test traffic to
systematically explore the state space of the data plane w.r.t. intended
network-wide policies. Symbolic execution, in general, suffers from state
explosion. Thus, to plan test traffic efficiently while meeting test
requirements (e.g., coverage), we identify and use  insights on the behavior of
the specific network data plane under test  (e.g., characteristics of the
network topology) as well as the given policies and test goals.

\item \mypara{Test validation} \Name monitors the behavior of the data plane
after injecting test traffic and infers whether it complies with our intended
policies. In so doing, we have overcome the challenge of mutual
\emph{interference} between regular network traffic (e.g., from users,
departments) and test traffic, w.r.t. both performance and correctness. To this
end we have developed heuristics to efficiently monitor relevant aspects of
network behavior at scale and validate the results. In case of observing policy
violations, we have designed procedures to localize the root cause (either in
an offline manner, or via follow up tests depending on the violation.)

\end{packeditemize}

\end{packeditemize}
}

We evaluate \Name w.r.t. its effectiveness, performance, and practicality in a
variety of settings using both emulation and a physical SDN network. Our
results XYZ.

This paper is organized as follows\dots




==> modeling-on.tex <==
\section{Network Policies}
The goal of this paper is to test whether network policies are enforced correctly. So we need
to first clearly define what these policies are. While there are different network policies (e.g.,
reachability, isolation, etc.), for now, we focus on Dynamic Policy Graphs (\DPGs). A \DPG 
is a specification of intended policies taking into account dynamic and stateful behavior of 
middleboxes. 

Roughly speaking, each node in this graph represents a middlebox. Each edge in the \DPG 
is annotated with the  condition $\condition_{\logicalmidboxindex,\nextlogicalmidboxindex}$ 
under which a packet needs to be steered from node $\logicalmidboxindex$ to node 
$\nextlogicalmidboxindex$.  $\condition_{\logicalmidboxindex,\nextlogicalmidboxindex}$ has 
two components:  (1) the  traffic class, and (2) the {\em processing context}  of node $\logicalmidboxindex$, 
if applicable. Figure~\ref{fig:dpgs} shows two example \DPGs.

\begin{figure}[t]
\centering
\subfloat[Dynamic policy routing]
{
\includegraphics[width=200pt]{figs/lips_hips_dpg.pdf}
\label{fig:webserver}
} \\
\subfloat[Middlebox context]
{
\includegraphics[width=200pt]{figs/proxy_dpg.pdf}
\label{fig:proxy}
}
\tightcaption{Example \DPGs. Rectangles with solid lines denote ``Ingress'' 
nodes and  with dotted lines denote ``Egress'' nodes. Circles denote middleboxes. 
Each edge is annotated with a condition of the form $\condition = \{\trafficClass; \NodeContext\}$ 
denoting the traffic class and the processing context(s). All traffic is initialized as ``\{null\};-''.}
\label{fig:dpgs}
\end{figure}

\section{Correctness of Policy Enforcement}
The goal of the test activity is to determine whether a given \DPG is enforced ``correctly" in the
actual network. To do so, first, we need to define correctness.

Let's define a path as an end-to-end (i.e., starting and ending at ingress/egress nodes) path that a 
traffic class may take. Note that each traffic class can possibly take more than one path in the \DPG 
depending on the $\NodeContext$ component of transition conditions. For example, traffic class 
$\{H_1\}$ in Figures~\ref{fig:proxy} may either take the path $\{H_1\} \rightarrow Proxy \rightarrow 
\{H_1\}$ (i.e., cache hit) or the path $\{H_1\} \rightarrow Proxy \rightarrow Internet$ (i.e., cache miss). 
Similarly, traffic class $\{H_2\}$ has three potential paths to take.

We can think of a \DPG in terms of path(s) that each traffic class takes in it. Let 
$\Path_{\trafficClass_\trafficClassIndex}$ denote the set of \DPG paths that traffic class 
$\trafficClass_\trafficClassIndex$ may take:\\
\\
\noindent
$\Path_{\trafficClass_\trafficClassIndex} = \{ 
\Path_{\trafficClass_\trafficClassIndex}^1,
\dots,
\Path_{\trafficClass_\trafficClassIndex}^\PathIndex,
\dots
\}$\\

Each path $\Path_{\trafficClass_\trafficClassIndex}^\PathIndex$ is composed of a sequence of
middleboxes and transition conditions:\\
\\
\noindent
$\Path_{\trafficClass_\trafficClassIndex}^\PathIndex=
\dots
\rightarrow
\logicalmidboxindex
\xrightarrow{\condition_{\logicalmidboxindex,\nextlogicalmidboxindex}^\trafficClassIndex}
\nextlogicalmidboxindex
\xrightarrow{\condition_{\nextlogicalmidboxindex,\nextnextlogicalmidboxindex}^\trafficClassIndex}
\nextnextlogicalmidboxindex
\dots
$\\

Since the traffic class component of each transition conditions is already denoted by the sub-script 
$\trafficClass$, we can state the above expressions as:\\
\\
\noindent
$\Path_{\trafficClass_\trafficClassIndex}^\PathIndex=
\dots
\rightarrow
\logicalmidboxindex
\xrightarrow{\NodeContext_{\logicalmidboxindex,\nextlogicalmidboxindex}^\trafficClassIndex}
\nextlogicalmidboxindex
\xrightarrow{\NodeContext_{\nextlogicalmidboxindex,\nextnextlogicalmidboxindex}^\trafficClassIndex}
\nextnextlogicalmidboxindex
\dots
$\\

We say the \DPG is correctly enforced if the following two conditions hold:

\mypara{Condition 1} $\forall \pkt \in \trafficClass_\trafficClassIndex$: if all context conditions of path
$\Path_{\trafficClass_\trafficClassIndex}^\PathIndex$ holds for \pkt $\Rightarrow \pkt$ traverses 
$\Path_{\trafficClass_\trafficClassIndex}^\PathIndex$.

\mypara{Condition 2} $\forall \pkt$ that take $\Path_{\trafficClass_\trafficClassIndex}^\PathIndex$: 
$\exists \trafficClassIndex$ s.t. $\pkt \in \trafficClass_\trafficClassIndex$ 
and all context conditions of path $\Path_{\trafficClass_\trafficClassIndex}^\PathIndex$ holds for \pkt.

%\seyed{not sure if sound and complete make sense here}

\section{Coverage}
A real data plane may be difficult to test due to:

\begin{packeditemize}
	\item number of traffic classes,
	\item number of possible contexts,
	\item number of middleboxes,
	\item large state space of middleboxes,
	\item practical constraints such as time, bandwidth, and computing resources required for testing.
\end{packeditemize}

Therefore, it may not be possible to verify the correctness using the definition given in the last 
section. In practice, we may choose to perform partial test in the following two sense:

\mypara{w.r.t. \DPG paths} covering only a subset of  $\Path_{\trafficClass_\trafficClassIndex}$

\mypara{w.r.t. traffic space} covering only a subset each traffic class (e.g., representative packets)

\seyed{another notion of partial coverage is when we may cover all paths but do not consider
possible values of inconsequential context. should be thought about\dots}

\seyed{how to quantify coverage? e.g., just the fraction of tested \DPG paths? 
maybe relative priority/importance of different traffic classes acts as a weight...}

\section{\DPF Models}

Middleboxes process input traffic and output the processed traffic. This processing behavior
may depend on the current state of the middlebox w.r.t. the observed traffic among other things.
This makes finite state machines (FSMs) a natural language for modeling middleboxes. In general,
the output traffic is a function of the input traffic and the current state of the middlebox (see
Figure~\ref{fig:overview}). Figure~\ref{fig:overview} shows the FSM model of a stateful firewall
based on TCP. While the output traffic in a firewall is either the same is the input or nil, for some
types of middleboxes such as NATs (not shown here) the output traffic can be a modified version 
of the input traffic.

\begin{figure}[t]
  \centering \includegraphics[width=170pt]{./figs/FSM_with_output.pdf}
  \tightcaption{In the FSM model of a middlebox, output packet of each state is a 
  function of the input packet and current sate.}
\label{fig:overview}
 \end{figure}
 
 \begin{figure}[t]
  \centering \includegraphics[width=170pt]{./figs/mealy_firewall_FSM.pdf}
  \tightcaption{The FSM model of a stateful firewall. Each edge is labeled by 
  \emph{input traffic/output traffic} while  \emph{\{\}} denotes no traffic (i.e., dropped traffic). 
  The output   is either the   same is input   or nil.}
\label{fig:overview}
 \end{figure}


\section{Data Plane Model}
To model the entire data plane, we need to interconnect/compose the models of individual
middleboxes given the physical network topology. This involves taking into account stateless
data plane elements such as switches and links.

Assuming there is only one flow in the network, we can compose the models of middleboxes
on its path in a serial manner, which naturally maps to the way the actual packets of flow are 
processed in the network traversing one middlebox after the other..

\section{Test Traffic Planning and Generation}
The task of testing the network can be viewed as generating and injecting test traffic that 
systematically traverses the state space of the data plane and infers which subset \DPG paths
$\Path_{\trafficClass_\trafficClassIndex}$ are enforced correctly w.r.t. soundness and completeness.


\section{To Do's}

\mypara{modeling story possibilities}
\begin{packeditemize}
	\item We have a generic spec model of each middlebox type (e.g., firewall, proxy). This means
	if the test fails, one possible reason is that some physical middlebox does not comply with this spec.
	\seyed{if this makes sense, we need some sort of model equivalence checking capability, e.g., 
	both the spec and the code should behave consistently w.r.t. test input...}
	\item first we synthesize a model from scratch given actual code of middleboxes, then we base our
	test traffic generation on these models.\seyed{this way we may not capture bad implementations.}
	\item \dots
\end{packeditemize}



==> motivation.tex <==
\section{Motivation} 
\label{sec:motivation}
\seyed{TODO: figures must be shrunk}

In this section, we use small but realistic network scenarios to highlight the
types of  {\em stateful data plane functions} and {\em context-dependent
policies} used by network operators. We  highlight the need for mechanisms to
reason about and test these scenarios to check the correctness of policy
implementations.  We also discuss why  existing  network test/verification
mechanisms fail to do so.

\mycomment
{
\begin{figure*}[t!]
\centering
\subfloat[Dynamic  cache actions.]
{
\vspace{-0.6cm}
\includegraphics[width=100pt]{figs_fullpaper/motivating_ex_departmental_proxy.pdf}
\label{fig:proxy_monitoring}
}
\hspace{0.1cm}
\subfloat[Blocking policy is difficult due to NATs.]
{
\vspace{-0.6cm}
\includegraphics[width=100pt]{figs_fullpaper/motivating_ex_cascaded_nats.pdf}
\label{fig:cascaded_nats}
}
\hspace{0.1cm}
\subfloat[Dynamic ``triggers''.]
{
\vspace{-0.6cm}
\includegraphics[width=100pt]{figs_fullpaper/motivating_ex_lips_hips.pdf}
\label{fig:dynamic_policy}
}
\tightcaption{Scenarios to highlight challenges with stateful data planes and context-dependent policies.}
\label{fig:qoe-sec6}
\end{figure*}
}

%------------------------------------------------------------------------------%
\subsection{Motivating Examples} 
\label{subsec:motivating_examples}


\begin{figure*}[t!]
\centering
\subfloat[Cached responses to host $H_2$ may bypass the monitor.]
{
\vspace{-0.6cm}
\includegraphics[width=170pt]{figs_fullpaper/motivating_ex_departmental_proxy.pdf}
\label{fig:proxy_monitoring_reality}
}
\hspace{0.1cm}
\subfloat[Operators high-level intended policy to use proxy and also restrict $H_2$'s web access.]
{
\vspace{-0.6cm}
\includegraphics[width=170pt]{figs_fullpaper/motivating_ex_departmental_proxy_high_level_policy.pdf}
\label{fig:proxy_monitoring_policy}
}
\tightcaption{Dynamic cache actions.}
\label{fig:proxy_monitoring}
\end{figure*}


%------------------------------------------------------------------------------%
\mypara{Stateful firewalling} Today's firewalls go beyond the
traditional match-then-drop paradigm.  A common policy is reflexive
firewalling; i.e., the firewall keeps the states of outgoing connections from
internal hosts and allows incoming packets for previously established
connections.  Unfortunately, even this basic stateful processing
cannot be handled by existing ``memoryless'' static checkers.  For
instance, ATPG~\cite{atpg} and HSA~\cite{hsa} can only check for
single packet effects and cannot model connection establishment logic
and reflexive rules.

\begin{figure*}[t!]
\centering
\subfloat[Cascaded NATs make correct firewalling difficult.]
{
\vspace{-0.6cm}
\includegraphics[width=170pt]{figs_fullpaper/motivating_ex_cascaded_nats.pdf}
\label{fig:cascaded_nats_reality}
}
\hspace{0.1cm}
\subfloat[Operators high-level  intended policy to to block $H_1$'s access to remote server
after NATs.]
{
\vspace{-0.6cm}
\includegraphics[width=170pt]{figs_fullpaper/motivating_ex_cascaded_nats_high_level_policy.pdf}
\label{fig:cascaded_nats_policy}
}
\tightcaption{Blocking policy is difficult due to NATs.}
\label{fig:cascaded_nats}
\end{figure*}

%---------------------------------------------------------------------%
\mypara{Dynamic policy violations} In network of
Figure~\ref{fig:proxy_monitoring_reality}, the operator intends to use proxy
for performance reasons and also restrict web access of certain hosts
(the policy is shown in Figure~\ref{fig:proxy_monitoring_policy}). 
The problem here is subtle, as the proxy may send cached
responses bypassing the monitor, defeating our goal. Potential fixes
to this problem include placing the monitor before the proxy or using
 techniques like {\tt FlowTags} to explicitly steer cached responses~\cite{flowtags_nsdilong}.  
There are two related challenges here. First, an administrator 
 must be able to  identify  such potential policy violations. 
 Second, having identified the problem and using a suitable
 fix (e.g., using {\tt FlowTags}), we need to check the specific 
  implementation.  

Note that to identify this policy violation, we need to model the stateful
behavior of the proxy across connections as well as the context of the traffic
after the proxy (i.e., the actual origin of the traffic in the department,
whether it is a cached response).

%\footnote{\Name was partly motivated by the failure of
%existing tools to validate systems such as FlowTags implementation 
%fixes the problem.}
 
 \seyed{the NAT example is pretty useless.}
 
\mypara{Firewalling with Cascaded NATs} Figure~\ref{fig:cascaded_nats}
shows a scenario where hosts are doubly NAT-ed -- at the department
and the enterprise border.  Prior work shows cascaded NATs are
notoriously error-prone~\cite{hotmbox_nats, netblaster}.  Suppose the
remote web server's firewall needs to to block host $H_1$ but allow
$H_2$. Even this seemingly easy access control policy is difficult to
check with existing L2/L3 reachability tools because the hosts are
hidden behind NATs hiding the necessary context; e.g., HSA/ATPG 
models them as ``black-boxes'.


\begin{figure*}[t!]
\centering
\subfloat[Testing the intended policy requires cognizance of IPS behaviors.]
{
\vspace{-0.6cm}
\includegraphics[width=170pt]{figs_fullpaper/motivating_ex_lips_hips.pdf}
\label{fig:dynamic_policy_reality}
}
\hspace{0.1cm}
\subfloat[Operators high-level  intended policy to of using heavy IPS based on traffic
context.]
{
\vspace{-0.6cm}
\includegraphics[width=170pt]{figs_fullpaper/motivating_ex_lips_hips_policy.pdf}
\label{fig:dynamic_policy_policy}
}
\tightcaption{Dynamic ``triggers''.}
\label{fig:dynamic_policy}
\end{figure*}


\mypara{Multi-stage triggers} Figure~\ref{fig:dynamic_policy} shows
two intrusion prevention systems (IPS) used in sequence.  The intended
policy is to use the light-weight IPS (L-IPS) in the common case and
only subject suspicious hosts flagged by the L-IPS (e.g., when a host
generates scans) to the more expensive H-IPS. Such multi-stage
detection is useful; e.g., to minimize latency and/or reduce the H-IPS
load.  Again, it is difficult to check that this multi-stage operation
works correctly using existing static checkers and reachability
verifiers~\cite{hsa, atpg}, because they ignore hidden state inside
the IPSes (e.g., the current per-host count of bad connections 
inside the L-IPS) and triggered sequence of intended actions 
(i.e., the context).


%--------------------------------------------------------------------%
\subsection{Strawman Solutions} 
\label{subsec:strawmans}

\seyed{my goal of this subsec is to demonstrate the three key
limitations of existing work by taking ATPG as the closest work.}

The above scenarios imply two aspects of policy enforcement that
make it difficult to ensure their correct enforcement: (1) capturing 
stateful data plane behaviors (e.g., stateful firewalls, proxy's cache); 
(2) context-dependent policies (e.g., LIPS-HIPS). 

To understand the fundamental reasons behind why existing work 
is not capable ensuring the correctness of policy enforcement in 
such scenarios, consider \emph{automatic test packet generation 
(ATPG)}~\cite{atpg}, a recent active testing tool motivated by limitations 
of {\tt ping}, {\tt traceroute}. ATPG is built based on three design 
decisions: (1) it uses packet as the I/O unit of it's model of the data 
plane; (2) it uses a models the data plane by modeling each switch 
as a transfer function that maps an input $(packet,port)$, called a 
located packet, to a set output located packets based on switch 
forwarding rules; (3) it finds sample test packets that exercise switch 
forwarding rules.

In an attempt to use ATPG to test the scenarios of this section, we
face three fundamental limitations:
\begin{packeditemize}

\item A \emph{located packet}, as the unit of test traffic generation, is too low-level.
stateful data plane elements such as stateful firewalls and proxies
operate at higher levels of semantics such as TCP connection and
HTTP session. Further, a located packet does not capture the necessary  
traffic context (i.e., the origin and relevant processing history of traffic) 
that is an integral part of the richer set of context-dependent policies 
(e.g., the IPSes example). Finally, a packet abstraction leads to scalability
issues: even in case of stateless data planes, ATPG had to resort to a 
greedy algorithm~\cite{atpg}.

\item A transfer function as the unit of a \emph{data plane model}, which
is a static mapping of input to output located packets, lacks the necessary
expressiveness, as it does not capture state that is a key behavioral part 
of stateful devices.

\item The \emph{search strategy} used in ATPG to find test packets is based
on the assumption that a transfer function processes each packet independently
of any other packets (i.e., stateless packet forwarding). In a stateful data plane, 
however, designing a search strategy is more challenging as it needs to 
efficiently explore a \emph{state space}, where processing of each packet
by a data plane element can change the behavior of the data plane for 
future packets (e.g., a stateful firewall).

\end {packeditemize}
 
Other recent work on static verification have the same underlying 
limitations (e.g., Anteater~\cite{anteater}, Hassel~\cite{hsa}, 
Veriflow~\cite{veriflow}, and NetPlumber~\cite{netplumber}).

%%%%%%%OLD TEXT BELOW%%%%%%%%
\comment{
\vyas{ dont like 2.2 .. what is the main point we want to highlight here??}

The above scenarios imply three key requirements: (1) capturing 
stateful data plane behaviors (e.g., stateful firewalls); (2) capturing 
contextual policies (e.g.,
LIPS-HIPS); and (3) active testing to reveal subtle traffic-dependent
bugs that may not be directly visible from just looking at the network
configuration (e.g., dynamic cache actions or cascaded NATs).

Below we discuss why existing solutions cannot address
the scenarios described earlier (Table~\ref{tab:relwork} 
summarizes these).

\vyas{active testing doesnt naturally follow}

\mypara{Test packet generation} Active testing of a network today is 
primarily limited to 

\mypara{Static verificatin}

\mypara{Verifying data plane software}

\comment{
Table~\ref{tab:relwork} summarizes if/how some existing solutions
address the scenarios described earlier. Across all motivating
scenarios, we find that existing tools for checking network policies
are inadequate. At a high level, the problem is that many existing
tools for network reachability testing explicitly acknowledge these
challenges and treat them as being out-of-scope to make their work
tractable. While there is some recent work on testing software data
planes, the focus is on different types of errors (e.g., crash or CPU
cycles/packet) rather than the network-wide policy violations we
consider here. Our overarching goal is to bring the benefits that
these aforementioned efforts have provided for reachability
correctness to the types of stateful network processing and 
contextual policies introduced by the above scenarios. Given the 
richer, and more complex, set of network policies that SDN has 
enabled (e.g., Pyretic~\cite{pyretic}, Kinetic~\cite{kinetic}) we believe 
offering the capability to validate policy enforcement in the data plane 
is particularly timely.
}
 
\begin{table}[h]  
\begin{footnotesize}
\begin{center}
    \begin{tabular}{  p{2.9cm} | p{1.6cm} | p{1.4cm} | p{1.1cm}   }
 					&{\bf Stateful data planes} & {\bf Context-dependent policies} & {\bf Active testing}		 \\ \hline
		{\it Relevant examples in~\S\ref{subsec:motivating_examples}} & {\it 1, 2, 3, 4} & {\it 2, 3, 4} & {\it 1, 2, 3, 4} \\ \hline

					
	{\tt ping}, {\tt traceroute}, test packet generation (e.g., ATPG~\cite{atpg})					& No					& No					& Yes				\\ \hline
	Static verification (e.g., Anteater~\cite{anteater}, Hassel~\cite{hsa}, Veriflow~\cite{veriflow}, and NetPlumber~\cite{netplumber})& No\footnote{}				&No					&No    				\\ \hline
	Verifying data plane software (e.g.,~\cite{epfl14})			& Yes				& No					&  No  				\\ 
    \end{tabular}
\end{center}
\end{footnotesize}
\vspace{-0.4cm}
\tightcaption{ Strawman solutions (rows) vs.\ requirements from 
 the motivating scenarios (columns).
 \\
 \footnotesize{$^3$Some recent work on static verification model 
 state (e.g., NoD~\cite{msr_nod}, and~\cite{pandaarxiv}).}}
\vspace{-0.2cm}
\label{tab:relwork}
\end{table}


Given the limitations of the strawman solutions, we aim to build a 
system to automatically generate test traffic that is capable of testing 
context-dependent policies in stateful data planes.
}

%\seyed{merge the above with the below}


%\seyed{the workflow figure and the section also needs to make the e2e data plane
%model things explicit. otherwise it looks like we test one \DPF at a time.}


% \seyed{more remote related work like control plane test and policy steering
% will go to del work section.}

%\seyed{if we change policy to something else we should apply it everywhere (including the paper title}

%\seyed{cite Penetration test(pybull) in relwork.}


==> motivation_old.tex <==
\section{Motivating Scenarios}

\label{sec:motivation}

%\subsection{Illustrating the problem}
In this section, we  present illustrative  network management tasks to
highlight how  dynamic traffic modifications by middleboxes  impact the ability
to correctly implement the intended policy.  We also highlight the shortcomings
of some natural   strawman solutions.


\subsection{Policy Routing} 

\begin{figure}[ht]
  \centering \includegraphics[width=200pt]{./figs/policyrouting.pdf}
  \tightcaption{{\bf Policy routing:}  S2 cannot
decide if the NAT-ed flow is from H1 or H2.}
% In this case,  
% placing Firewall before NAT  may
%solve the problem. In the general case, even careful placement
%cannot solve the problem.} 
\label{fig:polrouting}
 \end{figure}


Prior studies show that enterprises use different \emph{policy chains} of
middleboxes for different traffic classes (e.g.,
HTTP, E-mail)~\cite{dilip,comb}.  In Figure~\ref{fig:polrouting}, we have  two
internal hosts (H1 and H2),  two switches (S1 and S2), a NAT and an
application-layer firewall. 
Suppose our policy chains are $\mathit{H1}: \mathit{NAT}$ and  $\mathit{H2}:
\mathit{NAT}, \mathit{AppFirewall}$.  Here, the NAT maps
the internal source IPs (H1, H2) to public IPs.  Ideally, we want
flows from H2 to be forwarded to the AppFirewall while flows from H1  pass
through at S2.  Because  the controller is unaware of this mapping, it cannot
set up forwarding rules at S2 to route the traffic appropriately.  

%That is flows from H2 should go to
%AppFirewall while flows from H1 just pass through. (We would need analogous
%rules for the reverse flows as well.) 

We could consider some heuristics to reverse engineer the private-to-public IP
mappings; e.g., tracking the payloads to detect similar traffic between
incoming/outgoing connections at S1.  Even if we are willing to incur the
overheads of doing this analysis, the SDN controler cannot really reason about
the correctness of these inferrred mappings.  In this specific example,
placing AppFirewall before NAT  may solve the problem. In the general case,
however, placement cannot solve the problem.
 
 % The network administrator would like to define two
%classes of web traffic: class A traffic faces no filtering, but incoming web
%traffic of class B is filtered based on its content. Suppose traffics of H1
%and H2 belong to class A and class B, respectively. The problem here is as
%follows.

\mypara{Implications} This example highlights that even basic data plane
forwarding decisions may  depend on the internal logic of the middleboxes that
is not exposed to the SDN controller. In short, using Layer-3/Layer-2
information alone to implement forwarding decisions is no longer be sufficient
in the presence of middleboxes that modify traffic.



%This is an example of the policy routing problem where
%given a desired set of policies to be applied on different traffics, each type
%of traffic needs to traverse a sequence of middleboxes in an order that the
%policy set is satisfied.


\subsection{Forensics and performance diagnostics}
% Next, we focus on two other common network management tasks: forensic 
%analysis to detect abnormal behaviors after the fact and also 
% performance diagnostics to detect bottlenecks.


% therefore, the administrator decides to monitor the number of distinct connections 
%established by each internal host over a certain period of time (say 10-minute 
%intervals) using an IDS.  
% ($i\in\{1,2\}$) whose number of 
%distinct connections to remote server $s$, denoted by $N_{is}$ exceeds $N_{Threshold}$, 
%it raises an alarm. 
 %bserves $N=\sum_{i}\sum_{s}N_{is}$ distinct  
 % connections to a remote server such that $N > N_{Threshold}$, it cannot infer whether this 
%is a policy violation (i.e., $\exists i,s: N_{is} > N_{Threshold}$) or not (i.e.,
%$\forall\, i,s:\,N_{is}<N_{Threshold}$). The reason behind this issue is that IDS has no way 
%to identify individual hosts because of the effect of the NAT.

In the network of Figure~\ref{fig:forensics}, the administrator wants to flag
any internal host trying to establish many connections using an IDS (i.e., scan
detection)~\cite{}.  In the example, H1 creates two flows to destination D1 and
H2 spawns two flows to D2, D3.  Suppose the NAT maps Flow1/Flow3 to the public
source IP P1 and the other two to P2. Because the IDS can only see the NAT-ed
flows and cannot see the original $H_i$, it cannot accurately detect if some
$H_i$ has sent $N_{i} > N_\mathit{threshold}$. 
 

\begin{figure}[htbf]
  \centering \includegraphics[width=200pt]{./figs/forensics.pdf}
  \tightcaption{{\bf Forensics and diagnostics:} The challenge 
 here is in attributing   diagnostic or forensic measurements to
 the specific host/flow that is associated with the traffic.}
\label{fig:forensics}
\end{figure}

Extending the example, consider a data center setting with  \emph{virtual
middleboxes}.  The administrator wants to  run diagnostic probes to  detect if
specific traffic flows are being bottlenecked by middleboxes; e.g., to decide
if more virtual instances are necessary.  Such  performance measurements (e.g.,
latency, bandwidthh), however, may not be useful because we cannot correlate
the specific flows coming in/out of the NAT if both hosts are contacting the
same destination. Note that while placing the IDS before the NAT may solve the
forensic problem, it cannot solve the general problem when there are multiple
middleboxes modifying the traffic in sequence.


%\vyas{instead of internet, make this servers? and instead of nat add load
%balancer}

%\seyed{Is really an app used for this case in real worlk or is some sort of middlbebox needed?}
%{\bf Example 3--} 

% Figure~\ref{fig:fig3} depicts an enterprise
%network in which a load balancer (LB) distributes the request between the
%servers based on some hashing algorithm that accounts for current loads of the
%servers. Furthermore, a flow measurement application (APP) is launched to
%estimate end-to-end flow throughput and help detect the bottleneck servers, if
%any exists. While the load balancer is useful to distribute load between the
%servers evenly, it makes it difficult for the APP to detect which of the
%servers might be performing poorly because from the APP's standpoint, it is not
%possible to pair a given flow with its corresponding server.

%{\bf Implications--} Middlebox modifications, such as the one-to-many nature of 
%the load balancer in this example, can make network forensics tasks even more 
%challenging than they typically are.


%\begin{figure}[htbf]
%  \centering \includegraphics[scale=0.36]{./figs/fig3.pdf}
%  \tightcaption{Effect of middleboxes on forensics.}
%\label{fig:fig3}
%\end{figure}

\mypara{Implications}  The above  scenarios highlight  the difficulty in
\emph{attributing} network-level observations to the correct ``principal''
(i.e.,  host or a IP flow) responsible for that traffic in the presence of
middleboxes.  

% Middleboxes may hinder diagnostics applications, as they modify 
%the traffic. Note that as opposed to example 1, here there is only one class of 
%traffic.
%\vyas{Attributing usage/performance to principals is hard}


\subsection{Access control and resource management}
 Next, we consider a slightly more complex scenario involving a proxy. A proxy
is not only stateful, but it may also implement several optimziations such as
content caching and  connection caching. This means that we can no longer
assume a one-to-one mapping between incoming and outgoing flows/packets at such
middleboxes. (This may also apply to other kinds of middlboxes such as WAN
optimizers and application-specific gateways.) 
Suppose we have a proxy in conjunction with a resource
management device (Figure~\ref{fig:fig4}) and we want to implemnent  two 
 policies: (1) rate limiting access to the external network (WAN) and (2)
application-level access control (e.g., blocking access to social networking
sites during office hours).  

 In the rate limiting case, we face the attribution problem once again. The
downstream middlebox  cannot attribute connections coming from the proxy on
behalf of the hosts. What makes this problem harder is that the proxy may
\emph{multiplex} connections from multiple  sources  on to  a persistent
connection to an external server.  Thus, we need to  identify the \emph{set} of
hosts that have a causal relationship with the proxy-initiated connection.  As
discussed earlier, in some cases attribution problems can be solved by
reordering the placement of the middleboxes. In this case, there is no feasible
placement.  For instance,   H2 may receive a cached response  in which case it
did not contribute to the WAN footprint; placing the rate limiter before the
proxy, however, may cause us to incorrectly account for H2's WAN footprint. 


The same problems arise for the access control application as well.  Suppose we
want to allow H1 to access a particular website xyz but  block H2's access.
With a  H2 may be able to get cached versions of  xyz  and thus evade the
policy implemented at the access control device. In this case, we want the
cached responses to also be subject to the access control restrictions. This
again confirms that placement alone will not solve the problem---placing the
control device before the proxy may solve the attribution problem but
introduces new correctness problems if responses can be cached.



%Any peer to peer traffic will be dropped once a certain threshold has been reached. 
%Moreover, the proxy cache is deployed to reduce the request latency time by caching 
%recently retrieved content. Note that if a requested content resides at the cache,
%it should not be counted toward the p2p traffic, therefore, it should not face rate
%limiting. Due to function of the proxy cache, the rate limiter observes the aggregate 
%p2p traffic associated with both H1 and H2, which is a problem. For example, if the per 
%host limit is 50Mpbs and RL observes 80Mbps of p2p traffic, it has no clear way to decide 
%whether each host is operating in its alloted rate (e.g., each host has 40Mpbs of p2p 
%traffic) or one host is violating the limit (e.g., H1 is using 80Mpbs of p2p while H2
%is inactive).

%{\bf Implications--} The operational logic of some middleboxes, in particular, 
%the $1\rightarrow 0$ (cache hits) or $N\rightarrow 1$ (persistent sessions upon 
%cache miss) nature of flow mapping by cache proxies can create difficult challenges 
%to resource management applications. 

\begin{figure}[htbf]
  \centering \includegraphics[width=200pt]{./figs/accesscontrol.pdf}
  \tightcaption{{\bf Access control and rate limiting:} This example highlights the 
aditional complications introduced by connection multiplexing, 
 traffic dependence, and response caching. It  further highlights 
 that there is no single placement of middleboxes that can correctly 
 implement the policy.}
\label{fig:fig4}
\end{figure}


%{\bf Example 5--} There are two middleboxes in the network of Figure~\ref{fig:fig5}.
%A network-level firewall is deployed to enforce source and destination-based web 
%access restrictions. In particular, the administrator would like to prevent
%H1 from accessing facebook.com during work hours. This seemingly easy-to-implement
%policy turns into a challenge because of the presence of the proxy cache. Consider
%a request from H1 to access facebook during work hours. If the request results in
%a cache miss, the proxy cache will forward the request on behalf of H1 rewriting
%source information (IP and Port), which makes it difficult (if not impossible) for the 
%firewall to decide whether the corresponding flow is coming from H1. Some cache proxies that 
%support persistent connections may merge request packets from different users into 
%a single connection to the server (persistent session) that makes the problem of identifying individual 
%flows even harder. Finally, the case of cache hit introduces yet another challenge: 
%the firewall does not see any flows associated with H1's request.

\mypara{Implications}   More complex middleboxes whose actions depend on the
actual traffic requests (e.g., cached responses) and those that multiplex
connections may further impact correctness of policy enforcement. In this case,
there may be no feasible placement of middleboxes that can correctly implement
the policy.


%\seyed{say something different from the last case?}
%\vyas{placement will not solve the problem (e.g., rate limiter).
%the traffic dependence makes the problem harder (e.g., caching) and multiplexing 
% makes things harder}

%\begin{figure}[htbf]
%  \centering \includegraphics[scale=0.36]{./figs/fig5.pdf}
%  \tightcaption{Effect of middleboxes on reachability.}
%\label{fig:fig5}
%\end{figure}

%It is important to note that in all the above five classes of network policies,
%if the middleboxes have a proprietary logic, the problem becomes even more challenging.

%Table~\ref{tab:framework} shows attributes of the challenges faced in each example. Mapping 
%granularity indicates the level at which the traffic must be traceable in order for the 
%desired desired policy to be enforced.


%\seyed{should be decided how to fit in the context.}


% \seyed{how about ending the sec with this para?} While involving different network settings
% and middlebox functionalities, all of the above scenarios suffer from lack of an
% appropriate level of traffic ``visibility'' caused by middleboxes, which makes
% policy enforcement difficult.

%  In this example, the set of polices to apply to each
%traffic depends on real-time outcome of a middlebox and cannot be predicted in
%advance.

\comment
{
\begin{table*}[tbf]
  \centering
        \begin{small}
\begin{tabular}{|l | l| c | c |} 
    \hline
    {\bf Example} & {\bf Policy Class} & {\bf Required Mapping Granularity} & {\bf Mapping Multiplicity}\\
    \hline
	Example 1 & Policy Routing & $session \rightarrow session$ & $N \rightarrow 1$ (NAT) \\  \hline                        
	Example 2 & Diagnostics & $flow \rightarrow  flow$ & $N\rightarrow 1$ (NAT)\\  \hline                        
	Example 3 & Forensics & $flow \rightarrow  flow$ & $1\rightarrow N$ (Load Balancer)\\  \hline                        
	Example 4 & Resource Management  & $flow \rightarrow  flow$ & $1\rightarrow 0$, $N\rightarrow 1$ (Proxy-Cache)\\  \hline                        
	Example 5 & Reachability & $packet \rightarrow packet$ & $1\rightarrow 0$, $N\rightarrow 1$ (Proxy-Cache)\\    \hline
\end{tabular}
        \end{small}
  \vspace{-2mm}
  \tightcaption{Summary of how middleboxes affect policy enforcement in the example scenarios. \seyed{it seems for granularity we just need to say X rather than $X \rightarrow X$}}
  \label{tab:framework}
\end{table*}
}

\comment
{
\subsection{Strawman Solutions}

%\vyas{start with some high level text again. why this falls outside the scope
%of existing work in the SDN and net mgmt space}

The policy enforcement challenges that middleboxes cause due to complicated traffic 
modifications call for creating new capabilities. Previous related research mainly relies
on \textit{predictable} behavior of network elements, whereas some middleboxes violate
this assumption as we saw earlier in this section. Here we briefly discuss some of the
most relevant work.

Header space analysis~\cite{hsa} aims to model packet processing in a
network as a set of transformations on packet headers. If each `box' (e.g.,
switch or middlebox) in the network can be represented  as an invertible
transformation, many polices can be systematically verified. While useful for
certain scenarios, header space analysis cannot be applied if any of the
middleboxes: (i) behaves in a dynamic/randomized fashion (e.g., a load
balancer), (ii) cut the flow (e.g., a cache in case of cache hit), or (iii)
change the packet content. In cases (i) and (ii) the corresponding middlebox
cannot be modeled or it's inverse cannot be determined. In case (iii), on the
other hand, transformation involves an entire packet as opposed to header-only
transformations.

The idea in Verflow~\cite{veriflow} is to model the network as a set of
graphs each of which being traversed by the flows belonging to an equivalence
class. Flows in each equivalence class experience the same set of forwarding
actions.  Because of the reasons (i) and (ii) above, Veriflow is not a
sufficient solution (and it is not meant to be) for the case of dynamic
transformations.

Rearrangement of middleboxes might be deemed as a possible solution. For
instance, in the example network, if the proxy-cache is moved further ``down''
in the network, the problems can be partially addressed.\footnote{Note that in
this example the middlebox do not need to be physically moved due to the
connectivity of the switches; Only the forwarding information of the switches
should be adjusted to apply the desired sequence of middlebox processing.}
However, given the size of real-world networks, vast domain of network
policies, the diversity of middleboxes, and the interaction of middleboxes with
each other, it is impossible to find a feasible solution by shuffling the
middleboxes orders to find a ``good'' deployment. Furthermore, in some cases
rearranging middleboxes cannot solve the problem. For instance, in Example 4, even
if the rate limiter is located before the proxy-cache, the problem persists, as
the rate limiter should not drop p2p request that will result in a hit at the
proxy cache-- the rate limiter cannot predict hit or miss result of request.

It might appear that if all middlebox functionalities required for each traffic
can be applied at a single location rather than at different individual middleboxes,
the problem can be solved. CoMb~\cite{comb} is an example of consolidating various
middlebox functionalities, possibly within an individual machine. A policy shim steers 
traffic to and from various modules, each corresponding to a middlebox. While being 
partly helpful, the shim needs to determine the correct order of traversing middlbebox
modules such that the polices are enforced consistently. This approach reduces to the
previously described attempt of rearranging middleboxes, and therefore, is insufficient.

\vyas{what can we say abt this -- their focus seems orthogonal in state migration etc, not necessarily 
for these mgmt tasks, maybe say they are also looking at extending mboxes into the SDN fold. we are 
focusing on a more minimal set of info from mboxes rather than export full state info} Aditiya's hotnet '12 paper (middlebox interfaces)?\seyed{TBD}

Jeff's forwarded reference \seyed{TBD}

In the next section, we describe our solution to policy enforcement and verification in SDN, which is based on flow tagging.
}

\subsection{Summary} The above scenarios highlight the challenges that the dynamic
actions of middleboxes can cause for data plane correctess:  forwarding and
attributing the observed traffic to the right network-level principals. These
problems are further aggravated by middleboxes with 
non-deterministic and traffic dependent operations (e.g.,  cache responses
or multiplex connections). The common theme here is the \emph{lack of visibility} into the relationship 
 between the incoming and outgoing traffic at each middlebox. As 
 a  consequence, it is difficult to reason about the network-wide transformations that a
 single packet/flow  undergoes through a sequence of middleboxes and also 
 understand the causal context for why/how a specific observed packet 
 was created.
  



==> oldredteamtable <==
\begin{table*}[th]  
\begin{small}
\begin{center}
    \begin{tabular}{ p{4cm} | p{5.75cm} | p{5.75cm} }
   % \hline
    {\bf Scenario} 	& {\bf ``Red team'' bug} 	& {\bf ``Blue team'' Test trace}	\\ \hline
    
    (1) Proxy/Mon (Fig.~\ref{fig:proxy_monitoring})		
    & $S_1$-$S_3$ link is down.								
    & 	 %Bug found.      \emph{Test trace}:
  Missed HTTP request by Department 1 trying to reach the Internet.
    \\ \hline
    
    (1) Proxy/Mon (Fig.~\ref{fig:proxy_monitoring})		
    & {\tt Flowtags} controller assigns same tag values to Proxy 1 hit 
    and miss outgoing traffic.						
    &	%Bug found.      \emph{Test trace}: 
    Fetch an non-cached HTTP object by Department 1 and 
    then requesting the same object (now cached) by Department 2.
    \\ \hline
    
    (2) Conn. limitation (Fig.~\ref{fig:isolation})			
    & The counter of failed log in attempts at the authentication server keeps getting reset. 						
    &  % Bug found.      \emph{Test trace}: 
	Failed log in attempt by host $H_1$ beyond the intended threshold.
    \\ \hline
    
    (2) Conn. limitation (Fig.~\ref{fig:isolation})			
    & Switch $S_1$ does not have forwarding rules from the authentication server to switch $S_2$				 						
    &
	%5Bug found.      \emph{Test trace}
 Successful log in attempt by host $H_2$.				 
    \\ \hline
    
    (3) Multi-stage triggers (Fig.~\ref{fig:dynamic_policy})	
    & Light IPS is misconfigured to alarm after seeing 5 remote conn. attempts by a host (instead 
    of intended threshold of 10).
    & %Bug found.      \emph{Test trace}:
	 Host $H_1$ makes 9 scan attempts.					 
    \\ \hline
    
    (3) Multi-stage triggers (Fig.~\ref{fig:dynamic_policy})	
    & The light IPS is misconfigured to sum connection attempts of the three hosts (instead of 
    keeping separate counts).
    & %Bug found.      \emph{Test trace}:
 $H_1$ makes 10 scan attempts followed by 9 scans by $H_2$ (first of 
    which raises an alarm at L-IPS incorrectly)
    \\ \hline
    
    (4) Cascaded NATs 							
    & {\tt FlowTags} controller module is shut down.
    &  %\emph{Test trace}: 
	$H_1$ attempts to access to the server.
    \\ \hline\tightcaption{Red/blue team bug finding scenarios.}
\label{tab:bug_scenarios}
\end{table*}

    
    (4) Cascaded NATs 							
    &  {\tt FlowTags} assigns same tag value of $H_2$ to $H_1$.
    &	$H_1$ attempts to access to the server.	
%    \\ \hline
    \end{tabular}
\end{center}
\end{small}
\tightcaption{Red/blue team bug finding scenarios.}
\label{tab:bug_scenarios}
\end{table*}



==> overview.tex <==
\section{System Overview}
\label{sec:overview}

%----------------------------------------------------------------------------------------%

\vyas{

1.  goal -- enable operators to specify high level policies, and check if the implementations are correct
  we are the bridge between high level spec and the actual data plane 

2. talk about design choices and problem scope 
	a. testing vs verification
	b. model vs code
	
3. key components and workflow
	a. policy spec
	b. models 
	c. test case generation
	d. checking/diagnosis 

4. what does b, c entail -- reiterate the hsa model and problems

5. requirement, insights, ideas  how they meet requirements etc

6. concrete e2e workflow using adu + klee + library

6. low level optimizations -- delayed binding -- test generaton at abstract
granularity and move actual stuff 


}


%----------------------------------------------------------------------------------------------------%
\subsection{High-level Intuition}
\label{subsec:high_level_intuition}

Our goal is to help network operators with ensuing whether the data plane
behavior complies with their policies. To put this in context, network operators
have a set of intended policies in mind, examples of which we saw in the previous
section, which they enforce using a variety of ways (e.g., manual configuration 
of switches and \DPFs, or using higher level platforms such as Pyretic~\cite{pyretic}).
A major challenge for a network operator is to ensure if their intended policies
are enforced correctly.

In practice, there are two orthogonal approaches to ensuring correct policy 
enforcement: (1) static verification (e.g.,HSA~\cite{hsa}, Veriflow~\cite{veriflow},
 Vericon~\cite{vericon}), in which control plane information (e.g., a controller 
 application, or switch forwarding rules) are input to a verification engine that infers 
 whether the control plane information comply with intended policies (e.g., 
 reachability from node $A$ to node $B$); (2) active testing (e.g., {\tt ping}, 
 ATPG~\cite{atpg}), where the correct behavior is ensured by observing the 
 behavior of the data plane in response to injected test traffic. This allows 
 operators to ``see'' the behavior of the data plane, where actual packets 
 are processed. Active testing also helps capture faults that static verification 
 fundamentally misses (e.g., a  buggy firewall or switch, a broken link). Despite
 this important characteristics, it has surprisingly attracted very little attention
 as compared to static verification. For  these pragmatic reasons, we take 
 the active testing approach.
 
 \seyed{this para must explain why model's}
 Generating test traffic requires a \emph{model of the data  plane}, which 
 specifies the expected behavior of the data plane given operators
 policy. To illustrate this, consider a simple example. Suppose in a 
 network operator uses an implementation of a stateful firewall  with the 
 policy in mind that unsolicited connection attempts from outside world 
 should be disallowed. She configures and deploys the firewall  in the 
 network. Now to actively test this simple firewall policy using manually
 generated test traffic, in addition her intended policy (i.e., disallowing 
 unsolicited outside traffic), she also needs to know two things. She 
 needs to  have a model of a stateful firewall (perhaps implicitly in her 
 mind),  capturing the fact that it is  expected to remember state of each 
 TCP  connection (e.g.,  {\tt SYNACK\_RECEIVED}, {\tt ESTABLISHED}) 
 and  transition between  states  in a certain expected manner (if the current 
 state of a connection  is {\tt SYN\_SENT} and a {\tt SYN\_ACK} packet 
 is received from the  server, the new state will be {\tt ESTABLISHED}). 
 Based on this expectation  of a firewall and her intended policy, she 
 may generate test traffic to see,  for example, by sending {\tt SYN} 
 from an outside machine and observe if the firewall drops it. 
  
 %----------------------------------------------------------------------------------------------------%
\subsection{Challenges of Automatic Test Traffic Generation}
\label{subsec:tg_challenge}
 This manual test generation process we just described, however, quickly 
 becomes  cumbersome even in networks with a handful of stateful devices 
 and  simple policies  involving them. To automate this process, analogous 
 to the manual approach,  we need to use a model of the data plane  as 
 well as intended policies. 

\begin{figure}[th!]
\centering
\includegraphics[width=260pt]{figs_fullpaper/new_overview_fig.pdf}
\tightcaption{Three key components of an automatic test traffic generation.}
\label{fig:new_overview_fig}
\end{figure}

 The three key required components for automatic test traffic generation 
 are shown in Figure~\ref{fig:new_overview_fig}. First, we need to choose
 a unit of model-level traffic that traverses the data plane model (i.e., an
 interconnection of individual \DPF models). Second, we need to have 
 a way of modeling each \DPF, including stateless (i.e., switches) and 
 stateful \DPFs. Third, we need to have a strategy for searching
 the state space of the model with the goal of finding abstract traffic
 that when input into the model triggers certain states of the data plane 
 (e.g., the state in the  schematic model of the firewall shown in a different 
 color in the figure). (In a practical system there are other required elements 
 such as generating concrete test traffic given abstract test traffic and 
 monitoring  the data plane that we will discuss in~\S\ref{sec:workflow} 
 and~\S\ref{sec:implementation}.)
 \seyed{by this point people must know the intuition of model-based 
 test generation at an abstract level..}
 
Our choices with respect to these three dimensions need to satisfy 
two key requirements:

\begin{packedenumerate}

\item {\bf Expressiveness:} First, the system needs to provide a way of 
binding context to traffic in the model as to enable modeling 
context-dependent policies. Second, the model of the data plane 
needs to capture its stateful traffic processing behavior.

\item {\bf Scalability:} First, the unit of abstract traffic needs to support
the traffic processing scalability of the model. Second, the model of a 
stateful data plane needs to be tractable. Third, the system requires 
a scalable mechanism for systematic exploration of the model to automatically
generate test cases.

\end{packedenumerate}

To see the challenge of designing a model-based tester to test context-dependent
policies in stateful data planes, we present two representative design points 
and discuss their shortcomings.
 
 \mypara{$<$Traffic Unit=packet, Model=Implementation Code, Search strategy=Model Checking$>$}
This design choice might be temping for two reasons: (1) implementation code of 
 data plane elements (e.g., a firewall's code) might be available, and (2) a packet is 
 the real world traffic unit in a physical data plane. This design choice, however, is 
 infeasible on several fronts. First, packet is too level considering semantics of stateful
 devices such as proxies that operate at higher levels (e.g., HTTP or FTP session),
which will make arguing about such \DPFs difficult. Second, packet as the traffic 
unit does not capture the necessary context cross \DPFs. Third, choosing implementation 
code is the model of each \DPF is fundamentally wrong, as its possible bugs will
infect test traffic generation, defeating the purpose of testing! Fourth, implementation 
code of any reasonably realistic \DPF is too detailed and large to search. Finally,
model checking tools hardly scale beyond a few hundred lines of code.

 \mypara{$<$HSA/ATPG((Traffic Unit=located packet, Model=transfer function, Search strategy=
 custom search in the n-Dimention packet header space$>$}  The choice 
 of located packet as traffic unit, while a practical improvement over
 regular packets by binding packet to network port, suffers from the same shortcomings
 of choosing a packet as traffic unit. The choice of a transfer function, which 
 captures switch forwarding tables, teats stateful \DPFs as blackboxes, clearly 
 falling short of the expressiveness requirement. Finally, the search methods used
 in HSA and ATPG are based on the fundamental assumption of memory-less
 nature of switch behaviors as well as lack of traffic context, both critical for our goal.
 
%----------------------------------------------------------------------------------------------------%
\subsection{\Name End-to-End Workflow}
\label{sec:workflow}

To address the expressiveness and scalability requirements, we have made
careful design choices on three dimensions of the design space by (1) 
designing \PADUs as the traffic unit in the model~\S\ref{sec:traffic_unit}, 
(2) modeling each \DPF as an ensemble of FSMs and composing them 
together to yield the data plane model~\S\ref{sec:dpmodels}, and 
(3) choosing symbolic execution as the dat plane search strategy and applying
optimizations on top of \klee, a symbolic execution 
engine~\S\ref{sec:testgenerate}.
We have further implemented other required components of an 
automatic end-to-end test system as we will discuss 
in~\S\ref{sec:implementation} Figure~\ref{fig:workflow} illustrates 
the end-to-end workflow of our vision of \Name:

\begin{packedenumerate}

 \item The operator defines the intended network policies in a high-level form
 (e.g., high-level policy flowcharts shown in~\S\ref{sec:motivation});

 \item \Name uses a library of \DPF models to create an end-to-end data 
 plane model where each model inputs and outputs \PADUs as the unit of traffic, 
 which specifies;

\item \Name explores the policy-relevant states of the data plane model to 
generate an set of abstract (i.e., \PADU-level) test traffic,
 
 \item \Name translates this abstract test traffic into test scripts;
 
 \item When executed, the test scripts inject test traffic into the actual data 
 plane;
 
 \item \Name collects monitoring logs from the data plane;
 
 \item \Name analyzes monitoring logs and declares the final result of the test
 to the operator (i.e., success, or policy violation along with the \DPF in charge 
 of the violation).

\end{packedenumerate}

%\seyed{technically network topology is also an input to the system. if not obvious, 
%i will add it in the figure.}

\begin{figure}[t] \centering
\includegraphics[width=190pt]{./figs_fullpaper/buzz_workflow.pdf}
\vspace{-0.2cm}
\tightcaption{\Name workflow.} 
\vspace{-0.4cm}
\label{fig:workflow}
\end{figure}


\comment{
%----------------------------------------------------------------------------------------------------%
\subsubsection{Strawman Design Point 1: Human-Level Policy as Model}
\label{subsubsec:high_level_policy}

Network operators tend to have a high-level means of specifying
their intended policies, for example using a high-level flowchart that includes 
processing and decision boxes with three types of components:
 
\begin{packeditemize}
 
\item \emph{Traffic specification} as a condition box to represent the traffic 
relevant to the policy (e.g., in terms of 5-tuple such as traffic 
matching $proto=TCP$ and $dstPort=80$).

\item \emph{Internal process and condition boxes} of the flowchart each 
corresponds to a single logical stateful \DPF (e.g., a stateful firewall).

\item \emph{Terminal boxes} indicating externally observable traffic
processing events in the data plane (e.g., pass, drop).

\end{packeditemize}

Figure~\ref{fig:high_level_policy_of_proxy_monitoring} shows the 
high-level policy corresponding to the network of 
Figure~\ref{fig:proxy_monitoring}.

\begin{figure}[h]
\centering
\includegraphics[width=140pt]{figs_fullpaper/motivating_ex_departmental_proxy_high_level_policy.pdf}
\tightcaption{High-level policy of Figure~\ref{fig:proxy_monitoring}.}
\label{fig:high_level_policy_of_proxy_monitoring}
\end{figure}

Perhaps the most natural candidate as a data plane model is the 
high-level policy itself, since it given by the operator anyway. A clear 
appeal of this choice is that a high-level policy is naturally scalable.  
The key shortcoming of a high-level policy, however, is the lack of 
expressiveness; it is too abstract to be useful for automatic test 
traffic generation, in that it hides the necessary information that 
affects traffic steering. To see why this is the case, consider the 
example network of Figure~\ref{fig:proxy_monitoring} and its 
corresponding high-level policy 
(Figure~\ref{fig:high_level_policy_of_proxy_monitoring}). Given 
the caching behavior of the proxy and the topology of the 
network, there is a subtlety here in an attempt to generate test traffic: 
we need to ensure the test traffic explores both cases of cache hit/miss 
(which are hidden in the high-level policy); otherwise, the test is 
fundamentally incomplete. For example, a cached response of the 
to-be-filtered {\tt XYZ.com} may be directly returned to $H_2$ (e.g., 
see~\cite{flowtags_nsdilong}). Being able to express such behavioral 
aspects of \DPFs is key to generate test traffic.\seyed{i already have flowchart
for the L-IPS, H-IPS if we need...}

%----------------------------------------------------------------------------------------------------%
\subsubsection{Strawman Design Point 2: Packet-Level Policy as Model}
\label{subsubsec:low_level_policy}

\begin{figure}[h]
\centering
\includegraphics[width=160pt]{figs_fullpaper/motivating_ex_departmental_proxy_packet_level_policy.pdf}
\tightcaption{Packet-level policy of the proxy of Figure~\ref{fig:proxy_monitoring}.}
\label{fig:low_level_policy_of_proxy_monitoring}
\end{figure}


The flowchart of Figure~\ref{fig:low_level_policy_of_proxy_monitoring} 
represents a very small fraction of the proxy's packet-level behavior when
receiving the first packet of HTTP response from a remote server. Such a 
model is naturally, expressive, as it is completely loyal to the 
intended packet-level behavior of the data plane, but it is too not scalable
due to capturing every single packet-level behavioral aspect of the proxy.
Even if we manage to write such a model, validating such it is as hard as 
our main goal of testing the actual data plane!
}

==> overview_sep15.tex <==
\subsection{\Name System Overview}
\label{sec:overview}

\vyas{

\begin{itemize}

\item P1: connect to previous section, re-emph stateful contextual and how 
 existing work fails 

\item P2: what we need is a systematic framework to check these things. 
 at a high level you can think of verification vs testing -- we go 
down testing road for pragmatic reasons 

\item P3: here is the overview of our framework.  we have a policy we want to
check.  we need a model of data plane.  then given policy and data plane, we
generate test cases.  test cases are given the data plane injectors we control.
if test case fails/succeeds we also need to validate 

\item P4: these functions naturally map to the  key components. 
 we highlight key challenges 
	\begin{itemize}
	\item policy model to capture semantics of context/state
	\item data plane model to capture diverse elements and balance 
 tractability vs fidelity. give key idea and fwd pointer. e.g., 
 extended located packet abstraction and policy-based model refinement
	\item efficient test case generation. give key idea and fwd pointer. 
 e.g., we find representative  instances and use symbolic rather tmodel check
	\item validation for correctness. give key ideas and fwd pointer.
  
	\end{itemize}  

\item P5: end to end walkthrough with one of the example scenarios maybe 
 to clarify things

\end{itemize}
}


%\subsection{System architecture}
\seyed{section needs to be tightened}
%\seyed{i think we should generalize the ``test manifest" 
%to include elements like mbox config instruction (e.g., the 
%"clear cache" instruction for a proxy), not just pure traffic to inject?} 

%\seyed{to decide: moving this high-level design to intro}

In this section, we begin with the overall vision of the \Name framework to 
address the challenges in testing contextual policies in  stateful  data planes.
We then provide an overview of the main components of \Name.

Figure~\ref{fig:io-behavior} shows the high-level input-output behavior of  \Name. 
There are three inputs to \Name:

\begin{packeditemize}

\item \emph{Network-wide policies}: These are intended network policies 
determined by the operator (e.g., reachability, service chaining).
\comment{While there are different alternatives, we describe 
an intuitive and precise way of specifying network policies (\DPG++).}

\item \emph{Network topology}: This specifies the type of network nodes (e.g., 
switches, end hosts, as well as \DPFs such as firewall and proxy) and their 
interconnections.

\item \emph{Test constraints\seyed{or scenarios?}}: These include a set of
practical constraints on the test activity; e.g., what hosts we can use as test traffic 
injection points, what servers can participate in the test (e.g., a TCP server while
testing a stateful firewall), how long the test can take, test success criteria
(e.g., coverage), and the maximum fraction of bandwidth consumed by test traffic.

\end{packeditemize}

The output of \Name is a report on which policies have succeeded/failed along
with relevant information (e.g., the traffic trace leading to a violation, test stats).

  \begin{figure}[th]
 \centering 
 \includegraphics[width=200pt]{./figs_fullpaper/flowtest_IO_behavior.pdf}
 \tightcaption{Input-output behavior \Name.}
\label{fig:io-behavior}
\end{figure}

Zooming into the \Name element of Figure~\ref{fig:io-behavior}, the top part 
of Figure~\ref{fig:overview} shows the high-level architecture of  \Name with 
three  logical components: 

%\subsection{Test traffic generator}
\mypara{1- Test traffic generator} It  generates a  \textit{test manifest}, which is
the concrete test traffic, and coordinates the actions of the \textit{injectors} to generate  
traffic traces that systematically test the intended policies in the actual data plane.

\begin{figure}[th]
\centering 
\includegraphics[width=230pt]{./figs_fullpaper/overview.pdf}
\tightcaption{High-level architecture of \Name.}
\label{fig:overview}
\end{figure}

Figure~\ref{fig:planner_arch} shows the building blocks of the test traffic 
planner component. Its output is a test manifest for the various  injectors,  
indicating the  sequence of test traces to inject, the time to inject, and  the 
set of locations at which to inject these packets. It uses a model of the data
plane to systematically generate test traffic. Its inputs are:

\begin{figure}[t]
  \centering \includegraphics[width=220pt]{./figs_fullpaper/planner_arch.pdf}
  \tightcaption{Design of the test traffic planner component of \Name.}
\label{fig:planner_arch}
 \end{figure}

{\em Models of data plane elements:} 
  First, we need abstract models \seyed{since any model is abstract, how about ``template models"?} 
  to capture different \DPFs. While stateless \DPFs (i.e., switches 
 and routers) can be modeled using {\em transfer functions}
 \footnote{A transfer function models the packet forwarding behavior of a switch. It 
 takes  as input a located packet and outputs  a set of located packets~\cite{hsa}.}, 
 we  need new models for stateful \DPFs such as proxies and stateful firewalls, which
 will used a library of temple models. 

{\em Network model:}  To generate test traffic, we need to model the entire 
data plane (i.e., how the \DPFs  are connected and what each of them do)
by composing the models of individual elements. 
%This is essential to test service chaining policies and dynamic data flows.

{\em Policy requirements:}  In addition to traditional network
reachability properties (e.g., loop-freeness or black holes), the power of
advanced  data planes coupled with new SDN control planes will  likely lead to
more complex policies\seyed{just cite and say ``...has led to..."}. We already saw 
some examples with a service chaining policy in Figure~\ref{fig:proxy_monitoring} 
and a contextual data flow in Figure~\ref{fig:dynamic_policy}.  This implicates more 
sophisticated test requirements; e.g., whether a NAT maps all packets in a flow 
consistently; whether a stateful firewall blocks reverse-direction traffic for unestablished 
connections; and whether a rate limiter honors the configured thresholds. (Network 
topology and test constraints are other inputs as discussed earlier in this section.)

Given these inputs, the test planner  generates a ``high-level''  test plan; e.g., \emph{``inject 
flow $f$ into the network from host/server $I$ at time $t$''}.  Intuitively, the purpose of test
plan is to devise test traffic that can systematically  explore  different states of the data 
plane and test its behavior in these states w.r.t. policies. For instance, in the example 
of Figure~\ref{fig:dynamic_policy}, to ensure that L-IPS triggers a suspicious flag, 
we need a host  to generate three consecutive failed connections.

The  test manifest generator  translates the output of the planner into a
concrete traffic trace, which can be injected into the network.  While one 
could conceptually combine the functions  of test planning and  test manifest 
generation, we take a pragmatic  decision to decouple them  to enable a more  
modular design so that we can independently refine the respective  algorithms 
for  test planning and manifest generation.

%\subsection{Injection/Monitoring} 
\mypara{2- Injection/Monitoring} \textit{\Injectors} are regular hosts or servers running 
 test traffic generators or trace injection software  and run the commands issued 
 by the planner. Monitoring passively monitor the status of the SDN controller and 
 the  data plane\seyed{do we want to say anything about SDN here? I would save it 
 for later maybe the implementation section.}.  This serves two purposes.  First, the current state can inform 
 the actions of the planner; e.g., which are the reachable prefixes.  Second, monitoring 
 reports help us validate if a test succeeded or  help diagnose why a test may have 
 failed; e.g., is it a legitimate failure or caused by interference from background traffic?

%\subsection{Validation/Diagnosis} 
\mypara{3- Validation/Diagnosis} Given monitoring reports, this module determines whether
the intended policies are enforced correctly. If a policy has been determined to have failed, 
this modules gives further information as to what specific reasons caused the violation (e.g.,
broken link, middlebox misbehavior).\seyed{we probably need a feedback loop from the 
validation back to traffic generation to conduct diagnosis. this is b/c certain failures require
some minimal follow-up test for diagnosis purposes}



==> testgenerate_sep19.tex <==
\section{Test Traffic Generation}
\label{sec:traffic-gen}


As we saw in \S\ref{sec:overview}, the goal of test traffic planning is to 
generate traffic traces that systematically explore relevant states of the 
data plane to examine whether the intended policies are correctly 
enforced. Given the template model of the data plane from the last section 
as well as the intended network policies, the goal of test traffic generation 
is to generate concrete test traffic that will be inject into the data plan to test 
in a live manner whether the policies are enforced correctly. In this section, 
we discuss how the policies are used to \emph{specialize} the template model 
the data plane for the specific network under test and how test manifest is 
generated given concrete data plane models .

\subsection{Requirements/Challenges}
Test manifest generation involves certain requirements:

\begin{packeditemize}

\item \emph{Efficiency}: Generating test traffic should be fast. Further, test traffic
should not consume too much of network resources (e.g., bandwidth).
\seyed{strawman: inject * at all injection points.}

\item \emph{Test coverage}: What ``states" of the data plane state space  should
be covered by the test traffic given policies? \seyed{strawman: inject randomly
formed packets}
%Given a cap for test traffic volume, what 
%states are more important to cover? These aspects should be controllable.

\item \emph{Coping with topology constraints}: Conducting test in a live manner
requires consideration of the physical network characteristics. Some examples 
of these constraints
are as follows: only a subset of network hosts/severs may be used to inject test 
traffic; certain test scenarios such as testing a stateful firewall require capture 
end-to-end connection semantics (as opposed to individual traffic packet as in 
ATPG~\cite{atpg}), which means there has to exist a cooperating server and the 
source IP of the test traffic should be routable.

\item \emph{Expressing contextual policies}: \seyed{maybe should not put this 
as a ``requirement" here. maybe it's an ``idea"} The operator needs to be able 
to specify contextual policies (e.g., service chains). 

\end{packeditemize}

In the rest of this section, first we introduce a way of expressing intended network 
policies that accommodates contextual policies. We then present our test traffic
generation solution to satisfy the above requirements.


\subsection{Test traffic planning via symbolic execution}
The goal of test is to ensure traffic is treated in the data plane as specified by 
the \policy. In general, this is a challenging test: many possible packets may
be injected into the physical network and it is not feasible to test all possible traffic
(violating the efficiency requirement). We may want to try picking sample test 
packets into the network. Doing so naively, however, is not helpful because test
traffic need to be carefully selected to exercise \policy regular expressions (the 
coverage requirement).

The question here is how to exercise policy paths efficiently while accommodating
network topology constraints?

\mypara{High-level idea} To systematically cover the policy space (i.e., exercising 
the regular expressions of \policy), while being efficient, we base our test traffic generation 
approach  on symbolic execution. Symbolic execution is a program analysis technique 
that attempts to explore possible behaviors of a program by considering symbolic 
inputs (as opposed to the typical case of using concrete inputs)~\cite{symbolic_execution_survey}.
Our approach is to use symbolic execution to explore the state space of the data plane.
At a high level, test packets are defined as symbolic variables and \policy is encoded
as assertions in the code of the data plane model. Symbolic execution, therefore, is 
used to find representative test packets (out of the equivalence class of packets that are
treated the same way in the data plane) whose values trigger important paths in the data 
plane.\footnote{Besides symbolic execution, we have also tried using model checking 
and AI planning to explore the data plane state space. While our results using these two
frameworks are similar to those using symbolic execution w.r.t. test correctness, symbolic 
execution outperforms those techniques.}

Symbolic execution, however, suffers from path explosion and quickly becomes 
unusable on programs with more than a few hundred lines of code if used naively.
We use a variety of techniques to tackle this and efficiently obtain test traffic as
discussed below.

\mypara{Encoding policies} Next, we instrument the code of the data plane model
on two fronts. First, we define a set of symbolic variables intended to be used as test 
packet. Second, we add assertions to the code that capture \policy. For example, if part 
of the \policy is that an IPS should alarm if it sees more than 10 SYN packets, the 
corresponding assertion looks like the following:\\

\noindent \texttt{assert(ipsCount < 10)}

The goal here is to guide the symbolic execution engine\footnote{We build on 
KLEE~\cite{klee}, a popular symbolic execution engine that runs on LLVM code.} 
to find test packet values that violate such assertions, thus resulting in test traffic.

\mypara{Constraining symbolic packets} The run time of symbolic execution is tightly
dependent on both the number and the possible values of symbolic variables. Simply 
making many packets whose all fields are symbolic, makes test traffic generation 
infeasible in any reasonable time frame. We use the knowledge of the policy as well
as topology to minimize the number of symbolic packets and minimize the number
of symbolic fields within each packet. For example, if we are testing a firewall in a 
network with 100 nodes (for ease of presentation, say with IP values $\in\{1\dots100\}$, 
we instrument the code to constrain the IP values of test packets:\\

\noindent \texttt{assume((pkt.srcIP >= 1) \&\& (pkt.srcIP <=100) )}

This greatly improves the performance of symbolic execution (which essentially
requires solving constraints on symbolic values).

\mypara{Generating test traffic generation code} Even though the data plane
is abstracted as a located packet processor, we cannot perform test on the actual 
network on a per-packet basis for practical reasons. For example, a TCP connection
involves OS-specified values for sequence numbers and congestion window size.
Specifying these platform-dependent values in advance is not practical. Therefore,
we generate test traffic generation code give the traffic packets output by the 
above symbolic execution-based mechanism. For example, three packets that
represent a TCP establishment three-way handshake, are encoded as a function:\\

\noindent \texttt{tcpEstab(sessionId, srcIP, dstIP, srcPort, dstPort)}

The test script that will be run on injector nodes is a sequence of such functions.

\mypara{Generating test manifest} Finally, the actions of test injectors need 
to be coordinated/timed. This requires accounting for network latency and 
timing of various injectors (e.g., while trying to trigger an IPS counter that 
resets every minute). 

The final output of test traffic generation is a test manifest, which is a set of time 
test scripts assigned to injector nodes.

\mypara{\seyed{section to do}}
\begin{packeditemize}

\item formulate test objective w.r.t. \policy: traffic satisfying a regex should
be treated the same in the data plane \dots

\item add a few code snippets of traffic generation code 

\end{packeditemize}

\comment{
\subsection{Strawman Solutions}

\begin{packeditemize}

\item \emph{Strawman solution 1}: Why bother with test traffic? If we verify the 
control plane and data plane configuration (e.g., switch forwarding and ACL rules), 
we do not need to test the data plane.

\item \emph{Rebuttal of strawman solution 1}: While static verification is useful, its power 
is limited on two fronts. First, existing solutions do not cannot capture stateful behavior of
the data plane and dynamic policies. Second, even if we can statically verify the control plane
and data plane, things can go wrong in the data plane (see~\cite{atpg}).

\item \emph{Strawman solution 2}: Test individual \DPFs using existing tools such 
as pybull~\cite{pytbull}.

\item \emph{Rebuttal of strawman solution 2}: These tools do not allow us to
test network-wide policies.

\item \emph{Strawman solution 3}: Simply use the data plane model to generate 
trace of test packets to inject into the network---similar to ATPG~\cite{atpg}.

\item \emph{Rebuttal of strawman solution 3}: In \Name, the assumptions on both 
the policies and data plane behavior are more general than those in ATPG. In particular,
in many scenarios (e.g., involving TCP/HTTP sessions) test traffic needs to be stateful.


\end{packeditemize}
}


==> tmp <==

\begin{packedenumerate}

\item \emph{Stateful data planes with hidden actions}: Existing
testing/verification tools focuses largely on the {\em stateless} behavior of
switches/routers modeling them as simple ``transfer functions'' that move
packets from one interface to another (e.g.,~\cite{hsa, veriflow}). In
practice,  networks contain an almost similar number of {\em stateful}
elements~\cite{aplomb}, whose  behaviors depend on both the history of observed
traffic and their internal states (e.g., a TCP connection state in a stateful
firewall). Moreover, many middleboxes induce  complex and hidden effects (e.g.,
a NAT modifying headers or a proxy returning cached responses) that make it
difficult to reason about data plane behavior.

\item \emph{Context-dependent policies}: A key reason for the deployment of
such stateful elements  is that the network operators want to implement more
complex and {\em context-dependent} policies that depend on {\bf XXX} and  go
significantly beyond basic reachability properties.  For example, there may be
compositional requirements to ensure traffic  is ``chained'' trough a sequence
of data plane modules~\cite{} or dynamically triggered  depending on the
history of a host's behavior (e.g., sending too many
connections)~\cite{intel_dynamic_sc, intel_on, cisco_nexus}. Furthermore, the
flexibility offered by new control mechanisms such as SDN/NFV will likely
enable even richer policies~\cite{kinetic}. Unfortunately, such richer policies
fall outside  the scope of existing network verification efforts
(e.g.,~\cite{hsa, veriflow, netplumber}).
\end{packedenumerate}

 

\comment
{

\begin{figure}[th!]
\centering
\includegraphics[width=220pt]{figs_fullpaper/buzz_intro.pdf}
\tightcaption{High-level vision of \Name based on active testing of policies in the data plane.}
\label{fig:intro_level_vision}
\end{figure}

VS: BELONGS LIKE A SECTION 3 STATEMENT
In an effort to bridge this critical yet largely neglected gap and take a step 
toward  the ``CAD-for-networks'' vision~\cite{mckeowntalklong}, one could adopt 
one of the two orthogonal paradigms of \emph{static verification} (i.e., inferring 
the properties of a network given the control plane information such as 
switch forwarding rules) or 
\emph{active testing} (i.e., observing the behavior of the data 
plane given test traffic) (see Figure~\ref{fig:intro_level_vision}). While static 
verification is useful, we take the active testing approach for a pragmatic 
reason: irrespective of what we can ``prove'' about a network based on its control 
plane information, the network operator needs practical assurance by 
observing whether things are working as expected in the data plane---where 
actual packets are processed.

 In this paper, we present \Name, a model-based testing (MBT) tool
 that actively tests context-dependent policies in stateful data planes 
via injecting automatically generated test traffic.\footnote{MBT, also known 
as specification-based testing, refers to a broad family of automatized 
software testing methods, where test inputs are generated 
given the intended behavior of a system; each test input is then 
executed in the system, and the observed behavior of the system 
is compared to the intended behavior for that input~\cite{mbt}.} At a 
high level, \Name takes high-level network policies from the human 
operator and generates and injects test traffic into the data plane. 
\Name then monitors and analyzes the behavior of the data plane 
and reports the result (i.e., whether the data plane behavior is 
compliant with the intended policies) to the operator.

In an effort toward building a model-based system to test 
context-dependent policies in stateful data planes, we face 
two challenges:

\begin{packeditemize}

\item {\bf Expressiveness:} Both the unit of model-level traffic 
(i.e., abstract traffic) and the data plane model (i.e., a specification
of the intended behavior of the data plane) need to be expressive. 
First, since our goal here is to test context-dependent policies, 
where the intended behavior of the network depends on some 
context associated with the traffic (e.g., the traffic has triggered 
an alarm on an upstream IPS should be steered to a heavy-weight 
signature detection element in the data plane), the system needs 
to provide a way of binding context to traffic. While a packet is a 
natural candidate, the necessary policy context (e.g., current 
packet has caused an alarm in a previous data plane element) 
is lost as the packet goes from one data plane element to the 
next.

Second, the model of the data plane needs to capture its 
stateful behavior (i.e., the packet dropping behavior of a firewall 
depends on the current connection state). While the most natural 
candidate as a data plane model is the high-level policy given by 
the operator, unfortunately, it is too abstract to be expressive, 
as it does not capture all the relevant stateful aspects of the data 
plane (e.g, caching behavior of a proxy). 

\item {\bf Scalability:} Three key components of a network model-based 
testing system can easily become a scalability bottleneck. First, if the unit 
of abstract traffic cannot be too fine granular, this leads to poor scalability 
of traffic processing in the model ruling out an individual packet 
as a seemingly natural candidate. Second, while choosing to model any
given stateful data plane element (e.g., a proxy) as an FSM seems to be 
a natural choice, this will lead to model intractability due to the huge 
number of states and transitions. Third, assuming we have a proper 
choice of data plane model and traffic I/O unit, we need a scalable 
mechanism for systematic exploration of the model to automatically
generate test cases. Several candidates including AI planning, model
checking, and custom search methods run into the scalability limitations 
when used on data planes with more than a handful of stateful 
elements.
\end{packeditemize}
}



==> todo.tex <==
\section{To Do/Think/Concerns}
\begin{itemize}
 
%\item just found non-interesting errors, e.g., ip v6 gets dropped

%\vyas{ignore ..no time}
 
 %\item what is the  guarantee? what is covered/non covered? should we worry about non-covered parts?
% should i be happy if you tell things are fine based on some sampling/statistical testing?

%\vyas{we said sthg abt coverage in sec6}
  
 \item what setting can we accommodate (enterprise, data center, cloud, interdomain, etc)? 
 are the principles  generalizable? 

\vyas{intro -- say this is quite general}
 
% \item what do we envision as the end product? an open flow app? a new architecture? a set of
% apis like flowtags?\dots

 \item failure plans to be added to policies. we should be able to test failure plans. failure plans have two elements time (performance), correctness
\vyas{sec 4 we say that intended behaviors can capture scenarios?}

\item  perf. test vs. correctness test

\vyas{one word in sec 3/4}

%\item  injection points

%\item  do emulation/static test before injecting things in the sensitive actual network. building on this, 
%since our traffic generation component has the majority of components of static checking/verification,
%we can propose {\bf the first framework to do both static and live analysis}.

%\item  toby: today about 90\% of operator time is spent on testing/debugging. things are painfully manual.

\item  correctness of physical/logical chains

%\item  how would sdn help with the whole thing

\item what is new? planning/symbolic execution/MC have been there... answer has
two parts: 1) no clear way of using them on existing fw, proxy etc code to
generate net-wide test traffic, 2) if run on actual code does not scale, but on
our models+some networking insight, it scales well.
\vyas{this is important -- relwork?}
 
% \item Check this out:~\cite{cisco_policy}
 
 \item non-determinism (e.g., random NATs). can we gain something by repeating
the test? are is it all hopeless?
\vyas{leave it as future work -- discussion of disclaimers in sec4}
 
% \item do we need a policy language (\DPG++) to capture the intended policies
%of section 2 examples?  (and justify why not use  e.g., pyretic, fattire, first
%order logic (as vericon says) etc...)
 
%  \item change of policy over time? can we test them incrementally and
%efficiently?
 
% \item use the notation i came up with in an earlier draft that formally
%describes policies, coverage etc
 
% \item section 4: problem formulation
 

% \item for some types of test the source ip should be routable (b/c of the response etc) e.g., proxy. for others
% it won't matter.
 
% \item we need also show what can of "network-specific" faults we can find (to avoid seeming like a software test solution)

 
 \item make it clear that we are not verifying data plane implementation's correctness 
(as opposed to epfl14). we are testing whether the policies are enforced correctly.
\vyas{this should be made clear in sec4/relwork}

\item In the paper we need to clearly argue why we decided to use models as opposed to real code. 
And what level of abstraction is good. The trade off here is as the model becomes more real, the 
traffic generation becomes easier but the performance of KLEE (or any other symbolic execution tool) 
goes down.

\vyas{check text in sec 5}

%\item check ``guarantee" claims of related work. e.g., vericon claims full coverage (para 3 of sec 6 of vericon)

%\item explain why we need to generate code snippets rather than packets. (e2e connections/policies etc)

%\item explain why the model needs to still be at the packet level (vs. say http\_get() level). it's because some policies
%and mbox behaviors are based on packets (e.g., firewalls etc)

%\item can we scale traffic generation by scaling out? maybe dpg decomposition is one way of doing so.

%\item speed up choice for klee: instead of loop: preprocess and hardcode the topology as f1(f2(f3(pkt)))?

%\item we are in fact testing a distributed system. what's the literature here (coverage, event interleaving,...)?

%\item what can we guarantee or do incrementally if the topology changes? (e.g., if one host joins to a big enterprise net,
%we probably should not do everything from scratch)

%\item can we do something like having a framework for "flexible validation middlebox models" as one contribution?
%what it means is if model a proxy as a simple two state fsm, then the system gives me a solution that validates that.
%if my model, on the other hand, has 10 states, again the systems gives a test trace that help me validate this specific
%model. this seems like a cool feature to have...

\item if decide to do MBT, where is the specification coming from? only human operator? or some 
pre-processing of config files? or both?

\vyas{sec 4}

%\item incremental testing (upon policy change or network topology change) is a big thing a few people 
%pointed out at hotsdn

\item reviewers may not be pl experts, so give some idea of why state explosion is not a concern
\vyas{this is important -- intro + sec 6}

%\item why do we model in C? can we do a better job of coverage etc of we use something else (e.g., 
%tools introduced in the taxonomy 2012 paper)

%\item an idea: can we do some sort of divide and conquer? in that maybe decomposing the code logic 
%we can scale better if the logic is independent

%\item prioritizing test cases can be useful thing (based on coverage power, path dependency, or importance of policies etc)

\item add the capability of "what if" failure test as vyas/toby said. e.g., we can fail a node as part of the test to see
what happens if...m
\vyas{sec4 -- intended behavior}

\item are we assuming atomic exec and sequential execution of events in the modeling and network run time?
if so, what are we missing?
\vyas{we are assuming in model but not in network -- make it clear in sec3}

%$\item add a concrete scale out example to section 2 (maybe opennf). this requires careful policy language, timing of test, and maybe
%dependency on the algorithm.

%\item the above example has two elements of correctness: what (have the flows been migrated successfully?) and when (is the
%migration triggered at the intended threshold)

%\item dpg++ should capture dynamic scaling scenarios (check opennf/split-merge)

\item for intuition, give the number of states to explore in a small example with a few nodes and show the value of symbolic ex etc.
\vyas{covered earlier .. see sec6 again}

%\item a survey to back what we say about contextual policies and service chains (like this: http://yuba.stanford.edu/~peyman/docs/atpg-survey.pdf)


%\item as part of the work we may want to think of asking the question "why is the network state what it is now?" and "can we trace it back
%to what got it here?" etc. this is a problem nick mentioned somewhere.

%\item use time machine for monitoring?

%\item there are two reasons that what klee explores can be different from the actual behavior of the program: 1) klee may have bugs, 
%2) program's non-determinism. that's why we want to run klee's generated test cases on the actual code and double check the results
%with gdb, gcov etc...

%\item why did epfl run into symbolic execution trouble on real code and restricted it to click, but we did not?

\item raja's point on modeling: what is the starting point of the modeling? can we do some automation to assist w modeling? should start from scratch? building blocks of models? a repository of models...? what are the key parameters of each middlebox? usability is important. 
\vyas{discussion if space}

%\item pip paper from jeff (old nsdi)
 
% \item should we worry about different versions of TCP etc affecting models/policies?
 
% \item how about i do model templates of typical behaviors (counting ups, signature matching ips. then the admin can just instantiate that
% by writing a dpg++ or just writing traditional device specific config files (that they should do anyway). first this makes the system much
% more usable (as opposed to admin writing crazy fsms everytime. second, we can find possible insconsistencies/bugs of config files by
% the use (the pre/static analysis stage)
 
% \item how about giving the admin a model refinement interface? something goes wrong (i.e., test of a single mbox fails): make
% admin's life easier by giving him the counter examples and a way of refining the fsm in a nice modular way.
 
% \item correctness of models can also be checked as follows: we have the model, test the actual device based on this. if we see
% inconsistency, it's either the device or the model that is doing something wrong: so give the example trace to human to decide what's
% the case (note that this is ok as long as the example is high-level, visual, fsm. for dist. systems like pip this is very low level and difficult
% for human).
 
% \item some faults are b/c of control plane or control-data plane commun channel (e.g., packet-ins). in other words, control plane
 %is not necessarily the only place that packets are processed. are we capturing these?
 
% \item things like firewall apps (hotsdn 14) are not really part of data plane? are they?
 
% \item what is the literature on test? check these: ~\cite{utting12, hierons09}

 \item we need device configurations/ACL files here too?
\vyas{might be important .. sec5?}

\item we need to say why Harpoon~\cite{harpoon} won't do.
\vyas{pentest/scale testing in relwork}

%\item  test manifest should be about more than mere traffic injection. sometimes we need server support for tcp etc. so 
%the manifest should specify those things.

%\item  in atpg we just need to something to inject as to exercise sw forwarding rules. here in flowtags
%we sometimes needs routable src ip addresses for a correct test.

\item  atpg simply is about packet injection (literally). our task is more elaborate for three reasons: 1) server side assumption/task, 2)
traffic validity (e.g., src ip rout ability), 3) timing (e.g., need to wait for syn/ack to send syn) 
\vyas{are we doing enough wrt atpg -- kill it in sec2/related work}

%\item the sequential composition that we do makes sense as it mimics how a packet traverses the net. can/should we  
%also compose fsms in parallel? 

%\item we need a way of validating policy on its own (e.g., no overlap b/w policy paths wrt packet header space). so 
%at this point we are sure policies are correct and consistent.

%\item should use efsm instead of fsm? http://www.seas.upenn.edu/~lee/10cis541/lecs/EFSM-Code-Generation-v4-1x2.pdf

%\item klee only works on sequential programs. (many dpfs are multithreaded)

%\item one limitation of logic verification is language dependence (vericon, princeton hotsdn14). this is a problem especially 
%real world \DPFs are not written in those fancy languages. even worse, \DPF code may not be accessible. 

%\item use raja's email points

%\item proxy also does dns. what are the consequences of capturing or not capturing such subtleties in the model?

\item the fsm models outputs one located packet. how about multicast/block? can be generalize the output
to a set rather than a single located packet?
\vyas{we dont do multicast/broadcast}

%\item people may wonder if this composition has anything to do with serial/parallel composition in pyretic\dots

%\item we successfully checked for loop freeness (annotating switch code and using a counter for the symbolic 
%observed packet). sent an email to vyas on this.

\item as opposed to symnet, we don't need to assume lack of global state, lack of state independence of different
boxes etc. any state is just a state and we can incorporate it.
\vyas{cite symnet in related work}

%\item bob lantz's point on race etc. good motivation for this work.

%\item synthesize a bit??

%\item refute hotsdn on fsm and planning and composition...

%\item maybe drop "located" part of located packets. does not seem to matter much?

%\item why not click instead of our c code? (symbolic execution on c++? and complexity)

%\item what happened to ``dynamic" keyword used in flowtags and hotsdn?

%\item testing individual \DPFs as well as network-wide test

\item make sure switches are explicit in modeling and throughout the paper. we want e2e models.
\vyas{emphasize in sec4 that we are modeling the full data plane}

%\item we can deal with blackbox and proprietary devices b/c the methods is based on specification.

%\item add example for notations

%\item compare to notations in consistent update paper

%\item iptables configuration mistakes 

%\item create problems with nats, cascaded nats with and w/o flowtags, with correct/incorrect flowtags

%\item create a buggy firewall with klee

%\item think about some cloud outsourcing. or virtual networks scenarios especially b/c sometime the physical
%info of the middlebox. so a primitive for testing the performance can be important.

%\item re. above: LB sends the first 5 flows to local server, then to remote slow server. here for even 
%performance testing we need intelligent traffic.

%\item do something w cascaded nats

%\item distbrituion for policlies

\item reordering effects that affect output behavior
\vyas{ack that the model is only intent .. we can use monitoring to check if this could cause}

%\item analogy with click to justify modeling
%
%\item can we think of sec of from a net operator point of view as follows: our observation is if we can specify the
%required behavior of a \DPF in terms of ip-layer located packet i/o, we are done (i.e., have a composable model
%of a data plane, analogous to click). this is a powerful notion using which we can deal with whiitebox blackbox
%hardware/software darA PLANES. and we show btw here is how to model fw, proxy, etc..

%\item maybe i should explicitly say i use klee in the mode that actually handles linux libraries and system calls.

\item cite berkeley's modeling middleboxes~\cite{modelingmiddleboxes}?
\vyas{add to related work}

%\item why not ndlog?

\item add Libra~\cite{libra}
\vyas{add to citation list}

%\item is fuzzing related work?

\item we need to formalize intended policies\dots
\vyas{check 3--6}

%\item are we pre-constrained with nodes capabilities for test traffic gen./servers? or is it part of the test to determine these?

\item make \DPF definition clear (does it include switches?)
\vyas{good point ... check for consistency at end}

%\item should make the default policy explicit? e.g., should we get test trace per policy path? or also per negation of a policy pass?


%item more reasons why not fuzzing etc: 1) what if config in wrong?, 2) take zoo long, 3) we are not doing sw/hw correctness test,
%e are testing a specific network (configured in a certain way etc) against a set of policies.

\item why not use tons of existing simulators as models? or even click as a model? we should bring existing simulations tools
as a modeling strawman solution. (e.g., say ns2 is c++ and > 300K LoC \dots)
\vyas{added to related work .. check}

%\item what if we cannot assume ip addresses? someone/anyone may attack the network.

\item we need to get eval number on switch-only nets (e.g., data centers with 1000s of switches) and show it is doable. 
intuition is it is only the state space of \DPFs that create challenge not switches. 
 %\vyas{what is the number??}

%\item maybe ratio of model size to actual code-base size is an interesting measure

\item what level of modeling abstraction can lead to what type of bug discovery?
\vyas{ack this in sec4/discussion}

\item what kind of bugs can/cannot flowtest catch?
\vyas{discussion/sec4}

%\item maybe we should specify why testing individual elements thoroughly and independently is not sufficient?
%why do we need end to end test? 
 
% \item katerina's feedback email
 
 \item wolfs (are we missing possible bugs due to klee opt on pre assignments) and hyentaeks (effect of level of model abstraction on bug types) questions were interesting. point them out in the paper.
 
% \item can reordering of test packets cause a problem?
 
 \item the examples should make it very clear that getting the right states triggered in the right ordered is difficult
\vyas{currently not being done -- why is it non trivial to get the specific tracesem effected?}
 
% \item reseting \DPF states by config reset (for test).

%\item maybe mention the policy validator script that makes sure the policy is well-defined.

%\item Are there any tradeoffs we can utilized. e.g., run \klee for longer to get more test cases.

\item output of DPFs can be events (fix in formalization)
\vyas{add somewhere in implementation that we also support timeouts}

%\item now the we have define PADU, the first klee optimization should be called minimizing symbolic variables (e.g.  PADU fields
%and number of time PADUs)

\item talk about flexibility of getting test trace for negation of policies etc. we can test something
good happens, something bad does not happen.
\vyas{?}

\item a sentence on scott vision of using software engineering tools/techniques
\vyas{?}

%\item plots 6 and 7, show the numerical value of max val on the right Y axis

\item we should clarify early on that logical and physical \DPFs are two different things.
\vyas{we should say it somewhere?}

\item cite MBT 2012 survey
\vyas{CITE}

\item we must say the 19 hour disaster is already attempting to do symbolic execution on the model code! doing it
on product scale code is even worse (beyond other reasons such as multithreaded code, and non-C code)
\vyas{say this in eval}

%\item specify that we intentionally over approx. the number of symbolic PADUs and why this is ok 
%(b/c of the assertion in side while). what is important is minimizing num of symbolic fields.

\item say somewhere we do reset \DPF states before doing the next test. other option is something like
opennf, so we know where we are starting.
\vyas{discussion -- }

\item somewhere we need to say FlowTest can deal with any data plane (sdn/non-sdn, 
click/proprietary/open-source middlebox with making no assumptions. the only requirement is 
we need to know the specification/model/requirement of each used element (which is a fair assumption. 
for one thing, we need to know why we are using something and what we expect from it.
\vyas{do we say SDN anywhere?}

%\item test coverage

%\item why are we giving new network notation?

%\item if the complain is it's modeling etc, hsa is also modeling switches and uses simple algebra on it, but
%it's about the usefulness, new capability...

%\item in the validation need to say the lock-step model is ok b/c interfering traffic are taken into account
%given models
 
\end{itemize}

